Ubi-SleepNet: Advanced Multimodal Fusion Techniques for Three-stage Sleep Classification Using Ubiquitous Sensing

Sleep is a fundamental physiological process that is essential for sustaining a healthy body and mind. The gold standard for clinical sleep monitoring is polysomnography(PSG), based on which sleep can be categorized into five stages, including wake/rapid eye movement sleep (REM sleep)/Non-REM sleep 1 (N1)/Non-REM sleep 2 (N2)/Non-REM sleep 3 (N3). However, PSG is expensive, burdensome, and not suitable for daily use. For long-term sleep monitoring, ubiquitous sensing may be a solution. Most recently, cardiac and movement sensing has become popular in classifying three-stage sleep, since both modalities can be easily acquired from research-grade or consumer-grade devices (e.g., Apple Watch). However, how best to fuse the data for the greatest accuracy remains an open question. In this work, we comprehensively studied deep learning (DL)-based advanced fusion techniques consisting of three fusion strategies alongside three fusion methods for three-stage sleep classification based on two publicly available datasets. Experimental results demonstrate important evidence that three-stage sleep can be reliably classified by fusing cardiac/movement sensing modalities, which may potentially become a practical tool to conduct large-scale sleep stage assessment studies or long-term self-tracking on sleep. To accelerate the progression of sleep research in the ubiquitous/wearable computing community, we made this project open source, and the code can be found at: https://github.com/bzhai/Ubi-SleepNet.

==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/figure_acc_cnn_network_structure.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{Figures/AccCNN_Network_Structure.pdf}
	\caption{An overview of the two subnets used to extract the deep features from the raw accelerometer data. }
    \label{fig:acc_cnn_network_structure}
\end{figure}

==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/figure_backbone_network_hp_tuning_results.tex <==
\begin{figure*}[!ht]
\begin{tabular}{cc}
\rotatebox[origin=c]{90}{} &
\includegraphics[width=15cm,valign=c]{Figures/hp_1.png}\\
    \addlinespace
\rotatebox[origin=c]{90}{} &
\includegraphics[width=15cm,valign=c]{Figures/hp_2.png}\\
    \addlinespace

\end{tabular}
\caption{DeepCNN backbone network hyper-parameters tuning results}
\label{fig:cnn_hp_plot}%
\end{figure*}


==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/figure_bing.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.4\linewidth]{Figures/Bing_LI.jpg}
	\caption{A typical polysomnography(PSG) study in sleep laboratory}
    \label{fig:bing}
\end{figure}

==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/figure_confusion_matrix_2.tex <==
\begin{figure} [h!]
\centering
\begin{tabular}{cccc}
\includegraphics[width=0.3\textwidth]{Figures/mesa_act_hrv_cnn100_cm.png} &
\includegraphics[width=0.3\textwidth]{Figures/mesa_act_hrv_resdeepcnn_att_act_cm.png}  \\
\textbf{(a)}  & \textbf{(b)}  \\[6pt]
\end{tabular}
\begin{tabular}{cccc}
\includegraphics[width=0.3\textwidth]{Figures/apple_mlp_cm.png} &
\includegraphics[width=0.3\textwidth]{Figures/apple_resdeepcnn-2D_addition_cm.png} &
\includegraphics[width=0.3\textwidth]{Figures/apple_raw.png} \\
\textbf{(c)}  & \textbf{(d)}   & \textbf{(e)} \\[6pt]
\end{tabular}
\caption{ \textbf{(a)} The CNN(101)  and early-stage fusion based on the MESA (ACT-HRV) dataset used in~\cite{Zhai2020MakingSensing}.
\textbf{(b)} Hybrid fusion using ResDeepCNN (Attention-on-Act) based on the MESA (ACT-HRV) dataset
\textbf{(c)} Walch et al. using multiple layer perception based on activity counts, HR and circadian time ~\cite{Walch2019SleepDevice} 
\textbf{(d)} Late-stage fusion using ResDeepCNN (Addition) based on the Apple Watch Dataset
\textbf{(e)} Late-stage fusion using ResDeepMixCNN (Concatenation) using raw accelerometer data and HRS based on the Apple Watch dataset.
}
\label{fig:confusion_matrix_2}
\end{figure}



==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/figure_feature_importance.tex <==
\begin{figure}[h]
\centering
\subcaptionbox{Wake}{\includegraphics[width=0.3\textwidth]{Figures/Wake_feature_importance.png}}%
\hfill % <-- Seperation
\subcaptionbox{NREMS}{\includegraphics[width=0.3\textwidth]{Figures/NREM_feature_importance.png}}%
\hfill % <-- Seperation
\subcaptionbox{REMS}{\includegraphics[width=0.3\textwidth]{Figures/REM_feature_importance.png}}%
\caption{The mean of total class activation value for each sleep stage from MESA dataset (ACT-HRV feature) using ResDeepCNN (Addition) in the late-stage fusion. ACT {:} Activity Counts,  MNNI {:} Mean NNI, SDNN{:} Standard Deviation of NNI, SDSD {:} Successive RR Interval Differences,VLF{:} Very-Low-Frequency Band, LF{:} Low-Frequency Band, HF{:} High-Frequency Band, LF/HF{:} The ratio of Low Frequency to High Frequency, SPI{:} The Signal Power Intensity}
\label{fig:featue_importance}
\end{figure}

==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/figure_grad_cam_plot.tex <==
\begin{figure}[t!]
\centering
\subcaptionbox{Wake}{\includegraphics[width=0.333\textwidth]{Figures/2880_wake_1_47.jpeg}}%
\hfill % <-- Seperation
\subcaptionbox{NREMS}{\includegraphics[width=0.333\textwidth]{Figures/712_nrem_2_208.jpeg}}%
\hfill % <-- Seperation
\subcaptionbox{REMS}{\includegraphics[width=0.333\textwidth]{Figures/328_rem_2_861.jpeg}}%
\caption{The Grad-CAM plot of three selected examples from MESA dataset (ACT-HRV feature) using ResDeepCNN (Addition) in the late-stage fusion. Each row is the activation map for the input clinical features. To obtain a clear graph, the highlighted areas are the activation values over the threshold of 0.8 and the light color areas represents the activation values below the threshold of 0.8}
\label{fig:cam_plot}
\end{figure}

==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/figure_inference_time.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=.6\linewidth]{Figures/classifier_module_inference_time.png}
	\caption{An overview of time consumption for each module based on each combination of fusion strategy and fusion method. We counted the running time of each sub-module on the Apple Watch data set for each model. The results are calculated based on 10 runs, and each run we inferred 500 samples.Time is in milliseconds.}
    \label{fig:inference_time_per_module_per_cls}
\end{figure}

==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/figure_raw_intermediate_mix_system_overview.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{Figures/Mixed_Raw_And_Feature_Fusion_Arrchitecture_Combined_v2.pdf}
	\caption{An overview of the three-stage sleep classification system using the raw accelerometer data with HR statistics features. The raw accelerometer data and HR statistic features were extracted for each sleep epoch (30s). The sliding window method divides the sleep data into multiple segments with window length $T$ and stride $S$. In this experiment, we have $T=101$, and $S=1$. We firstly use the AccCNN to learn deep features then fuse them with HR statistic features.  The hypnogram represents the stages of sleep over time. Two fusion strategies and four fusion methods were studied.}
    \label{fig:raw_system_overview}
\end{figure}

==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/figure_system_overview.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/Feature_Fusion_Architecture_Combined.pdf}
	\caption{An overview of the three-stage sleep classification system. Features were extracted for each sleep epoch (30s). The sliding window method divides the sleep data into multiple segments with window length $T$ and stride $S$. In our study, we set $T=101$, and $S =1$. The hypnogram represents the stages of sleep over time in each sleep epoch. Three fusion strategies and three fusion methods were studied. The prediction process was performed for each sleep epoch.}
    \label{fig:system_overview}
\end{figure}

==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/figure_user_study.tex <==
\begin{figure}[h!]
\centering
\subcaptionbox{}{\includegraphics[width=0.3\textwidth]{Figures/user_accuracy_plot.png}}%
\hfill % <-- Seperation
\subcaptionbox{}{\includegraphics[width=0.3\textwidth]{Figures/user_understanding_machine_assisted.png}}%
\hfill % <-- Seperation
\subcaptionbox{}{\includegraphics[width=0.3\textwidth]{Figures/user_accuracy_plot_by_label.png}}%

\caption{ \textbf{(a)} A user study of three-stage classification accuracy calculated per participant-wise for Non-CAM and CAM assisted visualization.
\textbf{(b)} The answer of \textit{The machine-assisted visualization helped me to understand the difference between each sleep stage}.
\textbf{(c)} The breakdown of classification accuracy calculated for each sleep stage.
}
\label{fig:user_study}
\end{figure}
% ** $p<0.01$

==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/section3_v3.tex <==
\section{Advanced Fusion Techniques for Three-stage Sleep Classification}
In this section, we will first discuss the current progress of multimodal fusion strategies and methods and their applications in sleep monitoring. We then present our study structure, followed by a technical description of three fusion strategies (early-stage, late-stage and hybrid fusion) and three methods (simple operation, attention mechanism and tensor-based method) 


\subsection{Overview of Multimodal Fusion}
 Multimodal fusion in machine learning has been extensively studied in pattern recognition applications, such as in image and video captioning\cite{You2016ImageAttention}, visual question answering~\cite{Yang2016StackedAnswering}, audio-visual speech recognition~\cite{Afouras2018DeepRecognition} and affect recognition~\cite{Kapoor2005MultimodalEnvironments}. In the field of ubiquitous computing, multimodal fusion has also been adopted for human activity recognition~\cite{Liu2020GlobalFusion:Fusion}, sleep stage classification~\cite{Zhai2020MakingSensing}, fatigue assessment ~\cite{Bai2020FatigueSensors} and person identification~\cite{Chen2017Rapid}. The simple concatenation method was commonly adopted in these studies to combine the raw inputs or combine the representations obtained from the pre-trained model of each modality~\cite{radu2018multimodal}. Other researchers explored more advanced fusion methods, such as the attention-based fusion scheme for human activity recognition~\cite{Liu2020GlobalFusion:Fusion} 
 
For monitoring sleep, several previous works achieved promising results for sleep stage classification by concatenating multimodal intermediate features and feeding them into DL models~\cite{Zhai2020MakingSensing, Hayano2017SleepSignals}. However, these studies focus on the choice of modalities rather than the fusion techniques. Different modalities may contain complementary information. It is difficult to explicitly identify the best suitable cross-modal fusion architectures.

In terms of the movement sensing and cardiac sensing, they are different in signal-to-noise ratio, data generation process and measurement frequency. Moreover, the activity count is better in sleep/wakefulness classification, but it is difficult to discern different sleep stages~\cite{Ancoli-Israel2003TheRhythms}. For healthy adults, the difference in heart rate variability between REM sleep and wake is less than the difference in  NREM and REM sleep~\cite{Chouchou2014HeartBrain}.


The choice of fusion strategy and fusion method may thus influence the model classification performance. In recent years, the DL-based computational models have outperformed shallow machine learning models for sleep stage classifications, not only on unimodal data, but also on the multimodal data~\cite{Zhai2020MakingSensing,Palotti2019BenchmarkTechniques, Phan2019SeqSleepNet:Staging}. Therefore, this work will only focus on the multimodal fusion techniques based on DL networks.



\subsection{Problem Statement}
Based on the movement sensing and cardiac sensing data, the goal of this work is to comprehensively study how to use the advanced fusion techniques to reliably classify three-stage sleep. As demonstrated in Fig. ~\ref{fig:system_overview}, we adopt a sliding window method with window size $T$ and stride $S$ to segment sleep recordings into frames.  In each frame, we could either extract the handcraft features (e.g. heart rate  features that were deemed to be intermediate / mid-level features) from each sleep epoch that can provide physiologically meaningful features to the model ~\cite{Zhai2020MakingSensing,Fonseca2017CardiorespiratoryFields}, or we could use neural networks to extract the deep features. The time step $t$ represents one sleep epoch (i.e. every 30 seconds). Given that, we aim to map the data in a sliding window to a sleep stage that corresponds to the center point of the window (e.g., the purple point in the hypnogram in Fig. ~\ref{fig:system_overview}).  

Suppose the $i$th frame-wise time-series input data for cardiac sensing can be denoted as $\mathbf{X}_{car}^{(i)} \in \mathbb{R}^{C_{car} \times T}$, where $C_{car}$ denotes the number of features/input channels and $T$ denotes the sliding window length. For movement sensing, the input data can be denoted as $\mathbf{X}_{mov}^{(i)} \in \mathbb{R}^{C_{mov} \times T}$. The details of feature extraction will be introduced in Section ~\ref{sec:methods}. The goal of deep multimodal fusion is to determine a multilayer neural network $f(\cdot)$ whose output $\hat{y}^{(i)}$ is expected to be the same as the target $y^{(i)}$ as much as possible for each sample $(\mathbf{X}_{mov}^{(i)}, \mathbf{X}_{car}^{(i)})$. This can be implemented by minimizing the empirical loss $\mathcal{L}$ for classification denoted as:
\begin{equation} \label{eq: loss_func}
    \min_{f} \frac{1}{N}\sum_{i=1}^{N}\mathcal{L}\left(\hat{y}^{(i)} = f(\mathbf{X}_{mov}^{(i)}, \mathbf{X}_{car}^{(i)}), y^{(i)}\right)
\end{equation}



\subsection{Fusion Strategy}
Traditional fusion strategies include feature level fusion (e.g., ~\cite{Rattani2007FeatureBiometrics,Wang2019MultifocusDomain,Wang2021MedicalTransform}), score-level fusion (e.g., ~\cite{Guan2017EnsemblesWearables}) or decision-level fusion (e.g., ~\cite{Guan2015OnMethod}). In the end-to-end DL era, the boundary between multimodal representation and fusion has been blurred. Representation learning is interlaced with classification (or regression) objectives. Nevertheless, the fusion strategy for DL models may still be carried out in three stages, such as early fusion, late fusion and hybrid fusion~\cite{Zhang2020MultimodalApplications}. 

Fusion at different stages may influence the results of representation learning. For example, the early and late fusion may inhibit intra-modal or inter-modal interaction~\cite{Zhang2020MultimodalApplications}.   Neverova et al. noted that highly correlated modalities should be fused together~\cite{Neverova2016ModDrop:Recognition}. Hazirbas et al. demonstrated that the performance of fusion is highly affected by the choice of which layer to fuse~\cite{Hazirbas2017FuseNet:Architecture}. For sleep stage classification , the way to fuse heterogeneous intermediate features is worthy of exploration. In this study, we want to gain a comprehensive understanding at what stage we should fuse these inputs to achieve the most performance improvements on the three-stage sleep classification task. We adopted three commonly used fusion strategies, including early-stage fusion, late-stage fusion and hybrid fusion, as shown in Figure~\ref{fig:system_overview}.

\subsubsection{Early-stage Fusion}
In the early-stage fusion, data from different modalities (e.g., intermediate features) are concatenated (stacked) in the input stage. It is popular because of its simplicity, yet it is sub-optimal~\cite{Phan2021XSleepNet:Staging}.  Early-stage fusion firstly concatenates the cardiac (denoted as subscript $car$) and movement (denoted as subscript $act$) sensing data then feeds them into neural networks $h$ to make a corresponding prediction.
\begin{equation}
    \hat{y}^{(i)} = h(\text{Concatenate}(\mathbf{X}^{(i)}_{car}, \mathbf{X}^{(i)}_{mov})).
\end{equation}
where Concatenate is the matrix concatenation function.

\subsubsection{Late-stage Fusion}
Late-stage fusion is another prevalent way to fuse (high-level) representation from multiple sources. This fusion strategy allows high-level representations to have better intra-modal coherence. Late-stage fusion processes each modality's $c$th channel input data with a network $q$ and then combines all their high-level representations via an aggregation operation followed by the classification layers. It is denoted as:
\begin{equation}
    \hat{y}^{(i)} = \varphi(\text{Agg}(q(\mathbf{x}_{mov,1}^{(i)}), \cdots, q(\mathbf{x}_{mov, C_{mov}}^{(i)}),  q(\mathbf{x}_{car,1}^{(i)}), \cdots, q(\mathbf{x}_{car,C_{car}}^{(i)})))
\end{equation}
where Agg is the aggregation function and $\varphi$ denotes the classifier (e.g. fully connected layers), and  $\mathbf{x}^{(i)} \in \mathbb{R}^{1 \times T}$ and $T$ is the window length. The cardiac intermediate features are denoted as  $\mathbf{X}_{car}^{(i)} = [\mathbf{x}^{(i)}_{car,1}, \mathbf{x}^{(i)}_{car,2}, \cdots,  \mathbf{x}^{(i)}_{car,C_{car}}]$.  In this study, the aggregation function represents various fusion methods that will be introduced in the next section. $q$ denotes neural networks that learn the latent representation (e.g., for CNNs, it is the feature maps) of the $c$th intermediate feature, where $C_{car}$ and $C_{mov}$ are the numbers of the intermediate features for cardiac sensing and movement sensing respectively.

\subsubsection{Hybrid Fusion}
With hybrid fusion, the fusion may occur at multiple stages/layers of the DL models~\cite{radu2018multimodal,Zeng2021Multi-levelCounting}. It's commonly understood that the DL model hierarchically encodes features at different levels, starting from low-level to higher-level features as the layers go deeper~\cite{Heaton2018IanLearning}. In this study, we would not cover all possible combinations of fusion architecture. Therefore, following previous work ~\cite{radu2018multimodal}, we consider a simple scenario, which is firstly to fuse different input channel data belonging to the same modality (sharing a representation learning network) and then to fuse the high-level features from both modalities at the later stage. Formally, the hybrid-fusion strategy can be written as:
\begin{equation}
    \hat{y}^{(i)} =  \varphi(\text{Agg}(g_{mov}(\mathbf{X}_{mov}^{(i)}), g_{car}(\mathbf{X}_{car}^{(i)})))
\end{equation}
where $\varphi$ is the classifier (e.g., fully connected neural networks) and $g$ denotes the modality-specific networks (e.g., CNNs) that can learn representation from a specific modality such that the $g_{mov}$ does not share network parameters with $g_{car}$. Agg is the aggregation function that can be implemented as concatenation[51],  attention mechanism~\cite{Yang2016StackedAnswering} and tensor-based method~\cite{Fukui2016MultimodalGrounding}.


\subsection{Fusion Method}

Based on their complexity, fusion methods can be divided into three types: simple operations, attention-based methods and tensor-based methods. For feature vectors from different modalities, the concatenation and addition are two commonly used simple operations~\cite{Zhang2020MultimodalApplications}.  The attention mechanism is widely used for multimodal fusion. This usually refers to dynamically calculating a weight vector for each time step (or spatial position) and weighting a set of feature vectors~\cite{Bahdanau2015NeuralTranslate, Duan2020SOFA-Net:Counting}. 
For tensor-based methods, bilinear pooling is a method of fusing two unimodal representations to a joint presentation by calculating their outer product. This method can capture the multiplicative interaction between all elements in two vectors~\cite{Yu2017Multi-modalAnswering}.

For the early-stage fusion, we only adopted the concatenation as the only fusion method in this study. For the late-stage fusion, we selected two commonly used simple methods, which are concatenation and element-wise addition. Hybrid fusion provides aggregated representations for each modality, which facilitates flexible fusion methods. Apart from the simple operation methods, we also evaluated the attention mechanism and the tensor-based method. The choice of fusion method may be influenced by the application context. 
\subsubsection{Concatenation}
For \textbf{early-stage fusion}, the concatenation method concatenates inputs of all modalities into one matrix, which can be denoted as:  
\begin{equation} \label{eq: early_concatenation}
\matr{K}_{early}^{(i)} = \text{Concatenate}(\mathbf{X}_{car}^{(i)}, \mathbf{X}_{mov}^{(i)})
\end{equation}
where $\matr{K}_{early}^{(i)} \in \mathbb{R}^{(C_{mov} + C_{car}) \times T}$ .  $\matr{X}_{car}^{(i)} \in \mathbb{R}^{C_{car} \times T}$ is the intermediate feature matrix of cardiac sensing, $\mathbf{X}_{mov}^{(i)} \in \mathbb{R}^{C_{mov} \times T}$  is the intermediate feature matrix of movement sensing, and the $C_{car}$ represents the number of intermediate feature inputs of cardiac sensing.

%%%% late-stage fusion method %%%%%
For \textbf{late-stage fusion}, suppose we have the cardiac latent representation denoted as $\matr{X}_{car, c}^{\prime (i)} \in \mathbb{R}^{U \times L}$, which is learned from a neural network $g$ via $\matr{X}_{car,c}^{\prime (i)} = g(\mathbf{x}_{car,c}^{(i)})$. The movement representation matrix is computed in the same way, which can be formally denoted as $\matr{X}_{mov}^{\prime (i)} =  g(\mathbf{x}_{mov}^{(i)})$ where the $\matr{X}^{\prime (i)}_{mov} \in \mathbb{R}^{U \times L}$ is the latent representation of movement sensing. $L$ is the temporal length and $U$ is the representation's dimension. For example, in a convolutional neural network, $U$ is the number of feature maps. At the late stage, as the feature maps of each input intermediate feature were kept separately,  the concatenation operation concatenates these representations together, as follows: 
\begin{equation}\label{eq:concatenation}
    \matr{K}^{(i)}_{late} = \text{Concatenate}(\matr{X}^{\prime (i)}_ {mov, 1}, \cdots,\matr{X}^{\prime (i)}_{mov, C_{mov}},  \matr{X}^{\prime (i)}_{car,1},\cdots, \matr{X}^{\prime (i)}_{car,C_{car}})
\end{equation}
In this study, for the activity counts (handcraft feature) and cardiac features, the late-stage fusion's representation is denoted as $\matr{K}^{(i)}_{late} \in \mathbb{R}^{(C_{mov}+C_{car}) \times U \times L}$

%%%%% the hybrid fusion method %%%%%
For the \textbf{hybrid fusion}, the high-level representation of each modality is obtained from their own sub-network. The movement sensing representation is denoted as $\matr{X}_{mov}^{\prime\prime (i)} =  g_{mov}(\matr{X}_{mov}^{(i)})$ and the cardiac sensing is formally denoted as $\matr{X}_{car}^{\prime\prime (i)} =  g_{car}(\matr{X}_{car}^{(i)})$. The concatenation method for the hybrid fusion can be written as:
\begin{equation}
    \matr{K}^{(i)}_{hybrid} = \text{Concatenate}(\matr{X}^{\prime \prime(i)}_{car},\matr{X}^{\prime\prime(i)}_{mov})
\end{equation}
where $\matr{K}^{(i)}_{hybrid} \in \mathbb{R}^{2U \times L}$


\subsubsection{Addition}The second simple operation is the element-wise addition denoted as $\oplus$. For the \textbf{late-stage fusion}, the addition operation is to integrate the high-level representation of each channel from each modality. The method is formally denoted: 
\begin{equation}\label{eq:addition}
\matr{Q}_{late}^{(i)} = \matr{X}_{mov,1}^{\prime (i)} \oplus, \cdots, \matr{X}_{mov,C_{mov}}^{\prime (i)} \oplus \matr{X}_{car,1}^{\prime (i)} ,\cdots, \oplus \matr{X}_{car,C_{car}}^{\prime (i)}
\end{equation}
where $\matr{Q}^{(i)}_{late} \in \mathbb{R}^{U \times L}$.

For the \textbf{hybrid fusion}, the addition method will aggregate the high-level representation of each modality. Formally, it can be denoted as:
\begin{equation}
    \matr{Q}_{hybrid}^{(i)} = \matr{X}_{car}^{\prime\prime (i)} \oplus \matr{X}_{mov}^{\prime \prime(i)}
\end{equation}
where $\matr{Q}^{(i)}_{hybrid} \in \mathbb{R}^{U \times T}$.

\subsubsection{Attention Mechanism}
Attention methods have been broadly adopted in multimodal fusion tasks. For example, in VQA tasks the method used is to fuse the visual representations with the language representation~\cite{Yang2016StackedAnswering}. In our study we derived the attention model that could use the attention vectors to weight one modality based on the context of another modality. The meaning behind this is to filter the most significant information from a unimodal, which is jointly relevant for three-stage sleep classification. Therefore, we designed two attention fusion methods. The first one is Attention-on-Movement (Attention-on-Mov) and the second one is Attention-on-Cardiac (Attention-on-Car). 
Given the cardiac representation matrix $\matr{X}_{car}^{\prime (i)}$ and the movement representation matrix $\matr{X}_{mov}^{\prime (i)}$, we firstly feed them through a single-layer neural network and then apply the softmax function to generate the attention distribution over the temporal dimension, which is denoted as: 
\begin{equation} \label{eq: fused_matrix}
\matr{H}_{att}^{(i)} = \text{tanh}(\matr{W}_{car}\matr{X}_{car}^{\prime {(i)}} \oplus \matr{W}_{mov}\matr{X}_{mov}^{\prime {(i)}} + b_h)
\end{equation}
\begin{equation} \label{eq:attention_weights}
\matr{P}_{att}^{(i)} = \text{softmax}(\matr{W}_{att} \matr{H}_{att}^{(i)} + b_{att} )
\end{equation}
where $\matr{X}_{mov}^{\prime (i)} \in \mathbb{R}^{U \times L}$.  Suppose we have linear transformation matrices that include $\matr{W}_{mov}, \matr{W}_{car} \in \mathbb{R}^{D \times U}$ and $\matr{W}_{att} \in \mathbb{R}^{L \times D}$, then $\matr{H}_{att}^{(i)} \in \mathbb{R}^{D \times L}$ and $\matr{P}_{att}^{(i)} \in \mathbb{R}^{L \times L}$, where $D$ is the dimension of attention embedding space. The attention weight matrix is denoted as  $ \matr{P}_{att}^{(i)} = [\matr{p}_{att,1}^{(i)},\cdots, \matr{p}_{att, L}^{(i)}]$ and each temporal step has an attention vector $\matr{p}_{att,l}^{(i)}$, where $\sum\limits\matr{p}_{att,l}^{(i)} = 1$. The subscript $att$ stands for attention and $l$ is the temporal step index.

We assume that applying attention weights on different modalities will have an impact on the results. Therefore, two scenarios were studied in this work. The first method is to weight cardiac sensing representation based on the attention distribution and concatenate them to build the joint feature representation matrix. It can be written as:
\begin{equation}\label{eq:attention_on_car}
\matr{V}_{car}^{(i)}= \matr{X}_{car}^{\prime(i)}\matr{P}_{att}^{(i)}
\end{equation}
\begin{equation}\label{eq:joint_feature_from_car}
\matr{K}_{car}^{(i)} = \text{Concatenate}(\matr{V}_{car}^{(i)} ,\matr{X}_{mov}^{\prime(i)})
\end{equation}
We refer to this method as Attention-on-Car and $\matr{K}_{car}^{(i)} \in \mathbb{R}^{2U \times L}$

The second method is to weight the latent feature of movement sensing using the attention distribution, then concatenate them to build the joint representation matrix, which can be denoted as:
\begin{equation}
\matr{V}_{mov}^{(i)} = \matr{X}_{mov}^{\prime(i)}\matr{P}_{att}^{(i)}
\end{equation}
\begin{equation}
\matr{K}_{mov}^{(i)} = \text{concatenate}(\matr{V}_{mov}^{(i)} , \matr{X}_{car}^{\prime(i)})
\end{equation}
We refer to this method as Attention-on-Mov and $\matr{K}_{mov}^{(i)} \in \mathbb{R}^{2U \times L}$ is the merged joint representation.

\subsubsection{Bilinear Pooling Method}

Bilinear pooling is a method to compute the matrices outer product that can facilitate multiplication interaction between all elements in both matrices. It's a method often used to fuse visual feature vectors with textual feature vectors to create a joint representation space, even though their distribution may vary dramatically\cite{Lu2016HierarchicalAnswering, Fukui2016MultimodalGrounding}. 
During the NREM sleep period, our cardiac system is co-modulated by peripheral and sympathetic neural systems. The heart rate is generally below the average of wake and REM sleep period and accompanied with tiny tremors in limb movement. We hypothesized that the bilinear model may be able to capture such tiny differences between REM and NREM sleep. Given its superior representation learning capacity, it has achieved remarkable performance in fine-grained image classification tasks~\cite{Lin2015BilinearRecognition}. Bilinear model calculates the outer product of two matrices. In this work, suppose we have two feature representation matrices $\matr{X_{car}^{\prime(i)}}$ and $\matr{X}_{mov}^{\prime(i)}$, and the bilinear representation can be written as: 
\begin{equation} \label{eq:bilinear}
\Vec{k}_{bi}^{(i)} = \text{vec} (\matr{X}_{car}^{\prime(i)} \otimes \matr{X}_{mov}^{\prime(i)})
\end{equation}
The symbol of $\otimes $ denotes Kronecker product of two matrices, and the vec denotes the matrix vectorization. After the vectorization, we then perform an element-wise signed square-root as denoted: 
 \begin{equation}
      \matr{k}_{bi}^{(i)} \leftarrow \text{sign}(k_{bi}^{(i)}) \sqrt{|k_{bi}^{(i)}|}
 \end{equation}
and then apply $l_2$ normalization on the vector $\matr{k}_{bi}^{(i)}$. We pass the normalized vector to a linear function that can reduce the feature dimensions before feeding them to the classifier. 


==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/table_apple_hrs_epoch.tex <==

\begin{table}[H]
  \caption{Three-stage sleep classification prediction results for each fusion strategy and method in the \textit{Apple} dataset using LOOCV method, evaluated on sleep epoch-wise during recording period. }
\centering
\resizebox{0.6\textwidth}{!}{%

\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\multicolumn{3}{c|}{\textbf{Fusion Specifics}} & \multicolumn{3}{c|}{\textbf{Performance Metrics}} & \multicolumn{3}{c}{\textbf{Time Deviation}} \\
\midrule
\textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Accuracy} & \textbf{Cohen} & \textbf{F1} & \textbf{Non-REM sleep} & \textbf{REM sleep} & \textbf{Wake} \\
\midrule
\multicolumn{1}{c|}{\multirow{2}[4]{*}{Early-Stage Fusion}} & DeepCNN & Concatenation & 72.3 $\pm$ 2.5 & 40.0 $\pm$ 5.8 & 59.0 $\pm$ 3.6 & -0.6 $\pm$ 22.3 & 11.8 $\pm$ 22.5 & -11.2 $\pm$ 6.9 \\
\cmidrule{2-9}  & ResDeepCNN & Concatenation & 76.0 $\pm$ 2.4 & 45.7 $\pm$ 6.1 & 63.4 $\pm$ 3.5 & 12.3 $\pm$ 17.2 & -4.0 $\pm$ 17.1 & -8.2 $\pm$ 7.3 \\
\midrule
\multicolumn{1}{c|}{\multirow{4}[4]{*}{Late-Stage Fusion}} & \multirow{2}[2]{*}{DeepCNN} & Concatenation & 76.2 $\pm$ 2.7 & 47.0 $\pm$ 7.1 & 63.7 $\pm$ 4.5 & 8.4 $\pm$ 16.5 & 1.3 $\pm$ 19.4 & -9.7 $\pm$ 7.1 \\
  &   & Addition & 78.2 $\pm$ 2.1 & 49.9 $\pm$ 6.9 & 65.2 $\pm$ 3.8 & 11.4 $\pm$ 10.4 & -0.6 $\pm$ 11.2 & -10.8 $\pm$ 6.6 \\
\cmidrule{2-9}  & \multirow{2}[2]{*}{ResDeepCNN} & Concatenation & 75.5 $\pm$ 2.9 & 47.0 $\pm$ 6.5 & 63.4 $\pm$ 4.2 & 10.4 $\pm$ 18.5 & -2.1 $\pm$ 19.6 & -8.3 $\pm$ 7.0 \\
  &   & Addition & \boldmath{}\textbf{78.2 $\pm$ 2.3}\unboldmath{} & \boldmath{}\textbf{52.0 $\pm$ 5.8}\unboldmath{} & \boldmath{}\textbf{66.5 $\pm$ 3.8}\unboldmath{} & 1.9 $\pm$ 11.7 & 4.7 $\pm$ 12.6 & -6.5 $\pm$ 7.3 \\
\midrule
\multicolumn{1}{c|}{\multirow{10}[4]{*}{Hybrid Fusion}} & \multirow{5}[2]{*}{DeepCNN} & Concatenation & 72.9 $\pm$ 3.0 & 40.1 $\pm$ 6.6 & 60.6 $\pm$ 3.8 & 10.7 $\pm$ 20.1 & 0.6 $\pm$ 19.5 & -11.4 $\pm$ 6.4 \\
  &   & Addition & 72.1 $\pm$ 2.9 & 38.6 $\pm$ 6.5 & 58.9 $\pm$ 3.9 & 8.8 $\pm$ 20.4 & 1.3 $\pm$ 19.9 & -10.2 $\pm$ 7.3 \\
  &   & Attention-On-Mov & 73.5 $\pm$ 2.9 & 41.3 $\pm$ 6.2 & 60.4 $\pm$ 3.9 & 1.2 $\pm$ 18.7 & 5.0 $\pm$ 18.9 & -6.2 $\pm$ 7.7 \\
  &   & Attention-On-Car & 71.1 $\pm$ 3.4 & 37.4 $\pm$ 6.7 & 58.1 $\pm$ 4.1 & 7.5 $\pm$ 24.3 & 0.7 $\pm$ 23.1 & -8.2 $\pm$ 7.5 \\
  &   & Bilinear & 70.4 $\pm$ 3.3 & 34.6 $\pm$ 7.0 & 56.9 $\pm$ 4.0 & 6.4 $\pm$ 21.6 & 4.8 $\pm$ 22.6 & -11.2 $\pm$ 5.5 \\
\cmidrule{2-9}  & \multirow{5}[2]{*}{ResDeepCNN} & Concatenation & 74.6 $\pm$ 2.6 & 44.5 $\pm$ 6.5 & 61.9 $\pm$ 3.5 & 10.2 $\pm$ 13.6 & -1.3 $\pm$ 14.1 & -8.9 $\pm$ 7.0 \\
  &   & Addition & 78.5 $\pm$ 2.4 & 51.5 $\pm$ 5.8 & 66.0 $\pm$ 3.6 & 11.8 $\pm$ 11.5 & -5.6 $\pm$ 12.2 & -6.2 $\pm$ 7.8 \\
  &   & Attention-On-Mov & 75.2 $\pm$ 2.6 & 45.0 $\pm$ 5.6 & 63.1 $\pm$ 3.4 & 10.4 $\pm$ 19.4 & -2.0 $\pm$ 19.5 & -8.4 $\pm$ 7.2 \\
  &   & Attention-On-Car & 72.2 $\pm$ 3.0 & 41.5 $\pm$ 6.8 & 59.7 $\pm$ 3.8 & -2.9 $\pm$ 25.3 & 12.0 $\pm$ 26.4 & -9.1 $\pm$ 6.7 \\
  &   & Bilinear & 70.8 $\pm$ 3.5 & 38.4 $\pm$ 7.5 & 58.1 $\pm$ 4.4 & -2.8 $\pm$ 22.9 & 6.4 $\pm$ 24.8 & -3.5 $\pm$ 8.0 \\
\bottomrule
\end{tabular}%
    
    
    }

  \label{tab:apple_hrs_epoch}%
\end{table}%


==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/table_apple_hrs_rp.tex <==

\begin{table}[hbtp]
  \centering
  \caption{Three-stage sleep classification results (mean ± standard error at 95\% confidence interval) for each combination of fusion strategies and methods with the Apple Watch dataset using ACT-HRS feature based on a window length of 101.}
    \resizebox{0.95\textwidth}{!}{%
% Table generated by Excel2LaTeX from sheet 'Apple_preprocessing_rp'
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\multicolumn{3}{c|}{\textbf{Fusion Specifics}} & \multicolumn{3}{c|}{\textbf{Performance Metrics}} & \multicolumn{3}{c}{\textbf{Time Deviation(min.)}} \\
\midrule
\textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Accuracy(\%)} & \textbf{Cohen's $\kappa$} & \textbf{Mean F1(\%)} & \textbf{Non-REM sleep} & \textbf{REM sleep} & \textbf{Wake} \\
\midrule
\multicolumn{1}{c|}{\multirow{2}[4]{*}{Early-Stage Fusion}} & DeepCNN & Concatenation & 72.3 $\pm$ 2.5 & 40.0 $\pm$ 5.8 & 59.0 $\pm$ 3.6 & -0.6 $\pm$ 22.3 & 11.8 $\pm$ 22.5 & -11.2 $\pm$ 6.9 \\
\cmidrule{2-9}  & ResDeepCNN & Concatenation & 76.0 $\pm$ 2.4 & 45.7 $\pm$ 6.1 & 63.4 $\pm$ 3.5 & 12.3 $\pm$ 17.2 & -4.0 $\pm$ 17.1 & -8.2 $\pm$ 7.3 \\
\midrule
\multicolumn{1}{c|}{\multirow{4}[4]{*}{Late-Stage Fusion}} & \multirow{2}[2]{*}{DeepCNN} & Concatenation & 76.2 $\pm$ 2.7 & 47.0 $\pm$ 7.1 & 63.7 $\pm$ 4.5 & 8.4 $\pm$ 16.5 & 1.3 $\pm$ 19.4 & -9.7 $\pm$ 7.1 \\
  &   & Addition & \boldmath{}\textbf{78.2 $\pm$ 2.1}\unboldmath{} & 49.9 $\pm$ 6.9 & 65.2 $\pm$ 3.8 & 11.4 $\pm$ 10.4 & -0.6 $\pm$ 11.2 & -10.8 $\pm$ 6.6 \\
\cmidrule{2-9}  & \multirow{2}[2]{*}{ResDeepCNN} & Concatenation & 75.5 $\pm$ 2.9 & 47.0 $\pm$ 6.5 & 63.4 $\pm$ 4.2 & 10.4 $\pm$ 18.5 & -2.1 $\pm$ 19.6 & -8.3 $\pm$ 7.0 \\
  &   & Addition & 78.2 $\pm$ 2.3 & \boldmath{}\textbf{52.0 $\pm$ 5.8}\unboldmath{} & \boldmath{}\textbf{66.5 $\pm$ 3.8}\unboldmath{} & 1.9 $\pm$ 11.7 & 4.7 $\pm$ 12.6 & -6.5 $\pm$ 7.3 \\
\midrule
\multicolumn{1}{c|}{\multirow{10}[4]{*}{Hybrid Fusion}} & \multirow{5}[2]{*}{DeepCNN} & Concatenation & 72.9 $\pm$ 3.0 & 40.1 $\pm$ 6.6 & 60.6 $\pm$ 3.8 & 10.7 $\pm$ 20.1 & 0.6 $\pm$ 19.5 & -11.4 $\pm$ 6.4 \\
  &   & Addition & 72.1 $\pm$ 2.9 & 38.6 $\pm$ 6.5 & 58.9 $\pm$ 3.9 & 8.8 $\pm$ 20.4 & 1.3 $\pm$ 19.9 & -10.2 $\pm$ 7.3 \\
  &   & Attention-on-Mov & 73.5 $\pm$ 2.9 & 41.3 $\pm$ 6.2 & 60.4 $\pm$ 3.9 & 1.2 $\pm$ 18.7 & 5.0 $\pm$ 18.9 & -6.2 $\pm$ 7.7 \\
  &   & Attention-on-Car & 71.1 $\pm$ 3.4 & 37.4 $\pm$ 6.7 & 58.1 $\pm$ 4.1 & 7.5 $\pm$ 24.3 & 0.7 $\pm$ 23.1 & -8.2 $\pm$ 7.5 \\
  &   & Bilinear & 69.5 $\pm$ 3.5 & 29.5 $\pm$ 7.5 & 53.0 $\pm$ 4.2 & 1.2 $\pm$ 25.7 & 10.0 $\pm$ 25.0 & -11.3 $\pm$ 8.5 \\
\cmidrule{2-9}  & \multirow{5}[2]{*}{ResDeepCNN} & Concatenation & 74.4 $\pm$ 2.4 & 44.2 $\pm$ 5.7 & 62.0 $\pm$ 3.3 & 2.5 $\pm$ 16.7 & 5.3 $\pm$ 16.9 & -7.8 $\pm$ 7.0 \\
  &   & Addition & 74.9 $\pm$ 2.3 & 44.3 $\pm$ 5.4 & 62.3 $\pm$ 3.7 & 12.8 $\pm$ 14.2 & -7.6 $\pm$ 15.6 & -5.2 $\pm$ 8.2 \\
  &   & Attention-on-Mov & 75.2 $\pm$ 2.6 & 45.0 $\pm$ 5.6 & 63.1 $\pm$ 3.4 & 10.4 $\pm$ 19.4 & -2.0 $\pm$ 19.5 & -8.4 $\pm$ 7.2 \\
  &   & Attention-on-Car & 72.2 $\pm$ 3.0 & 41.5 $\pm$ 6.8 & 59.7 $\pm$ 3.8 & -2.9 $\pm$ 25.3 & 12.0 $\pm$ 26.4 & -9.1 $\pm$ 6.7 \\
  &   & Bilinear & 70.8 $\pm$ 3.5 & 38.4 $\pm$ 7.5 & 58.1 $\pm$ 4.4 & -2.8 $\pm$ 22.9 & 6.4 $\pm$ 24.8 & -3.5 $\pm$ 8.0 \\
\bottomrule
\end{tabular}%



}
\label{tab:apple_hrs_rp}%
\end{table}%


==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/table_class_wise_metrics.tex <==

\begin{table}[h]
  \centering
  \caption{Comparison of three-stage sleep classification metrics between using the intermediate feature and using the raw accelerometer data with the cardiac intermediate feature. Metrics evaluated from the ResDeepCNN and ResDeepMixCNN based on window length of 101 in Apple Watch Dataset.}
  \resizebox{0.9\textwidth}{!}{%

\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\multirow{3}[6]{*}{\textbf{Fusion Strategy}} & \multirow{3}[6]{*}{\textbf{Fusion Method}} & \multicolumn{1}{c|}{\multirow{3}[6]{*}{\textbf{Performance Metrics}}} & \multicolumn{6}{c}{\textbf{Input Type}} \\
\cmidrule{4-9}  &   & \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\textbf{Intermediate Features}} & \multicolumn{3}{c}{\textbf{\shortstack{Raw Accleroemter \\ Cardiac Intermediate Features}}} \\
\cmidrule{4-9}  &   & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\textbf{WAKE}} & \multicolumn{1}{c|}{\textbf{NREM}} & \multicolumn{1}{c|}{\textbf{REM}} & \multicolumn{1}{c|}{\textbf{WAKE}} & \multicolumn{1}{c|}{\textbf{NREM}} & \multicolumn{1}{c}{\textbf{REM}} \\
\midrule
\multicolumn{1}{c|}{\multirow{2}[2]{*}{Early Stage Fusion}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Concatenation }} & Accuracy & 40.5 $\pm$ 6.2 & 72.6 $\pm$ 2.6 & 34.9 $\pm$ 7.0 & 34.9 $\pm$ 5.3 & 75.0 $\pm$ 2.4 & 32.8 $\pm$ 7.6 \\
  &   & F1 & 55.5 $\pm$ 6.4 & 83.9 $\pm$ 1.8 & 48.4 $\pm$ 8.2 & 50.0 $\pm$ 5.5 & 85.6 $\pm$ 1.6 & 45.5 $\pm$ 9.0 \\
\midrule
\multicolumn{1}{c|}{\multirow{10}[10]{*}{Hybrid Fusion}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Concatenation }} & Accuracy & 41.7 $\pm$ 6.1 & 70.5 $\pm$ 3.0 & 33.3 $\pm$ 6.4 & 37.5 $\pm$ 6.2 & 75.3 $\pm$ 2.6 & 36.0 $\pm$ 7.0 \\
  &   & F1 & 56.8 $\pm$ 6.1 & 82.4 $\pm$ 2.2 & 47.0 $\pm$ 7.9 & 52.4 $\pm$ 6.2 & 85.7 $\pm$ 1.7 & 49.7 $\pm$ 7.9 \\
\cmidrule{2-9}  & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Addition }} & Accuracy & 41.7 $\pm$ 6.1 & 70.5 $\pm$ 3.0 & 33.3 $\pm$ 6.4 & 34.9 $\pm$ 6.0 & 75.8 $\pm$ 2.5 & 30.3 $\pm$ 7.7 \\
  &   & F1 & 56.8 $\pm$ 6.1 & 82.4 $\pm$ 2.2 & 47.0 $\pm$ 7.9 & 49.5 $\pm$ 6.4 & 86.0 $\pm$ 1.7 & 42.2 $\pm$ 9.3 \\
\cmidrule{2-9}  & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Attention-On-Mov}} & Accuracy & 40.0 $\pm$ 5.8 & 71.3 $\pm$ 3.2 & 35.4 $\pm$ 7.1 & 36.8 $\pm$ 5.5 & 74.4 $\pm$ 2.8 & 31.4 $\pm$ 7.4 \\
  &   & F1 & 55.3 $\pm$ 5.8 & 82.9 $\pm$ 2.3 & 48.9 $\pm$ 8.4 & 52.1 $\pm$ 5.8 & 85.1 $\pm$ 1.9 & 44.1 $\pm$ 8.6 \\
\cmidrule{2-9}  & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Attention-On-Car}} & Accuracy & 41.0 $\pm$ 5.7 & 67.8 $\pm$ 3.8 & 30.5 $\pm$ 7.9 & 34.3 $\pm$ 5.9 & 73.1 $\pm$ 3.1 & 28.6 $\pm$ 8.2 \\
  &   & F1 & 56.3 $\pm$ 6.0 & 80.3 $\pm$ 3.1 & 42.5 $\pm$ 9.3 & 48.9 $\pm$ 6.6 & 84.2 $\pm$ 2.1 & 39.7 $\pm$ 9.8 \\
\cmidrule{2-9}  & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Bilinear}} & Accuracy & 35.9 $\pm$ 6.7 & 67.0 $\pm$ 4.0 & 29.7 $\pm$ 7.8 & 30.7 $\pm$ 6.8 & 70.7 $\pm$ 2.8 & 15.6 $\pm$ 5.3 \\
  &   & F1 & 50.2 $\pm$ 6.9 & 79.7 $\pm$ 3.0 & 41.6 $\pm$ 9.2 & 44.1 $\pm$ 7.4 & 82.6 $\pm$ 1.9 & 24.3 $\pm$ 7.6 \\
\bottomrule
\end{tabular}%

}
  \label{tab:classi-wise metrics}%
\end{table}%


==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/table_compare_epoch.tex <==

\begin{table}[htbp]
  \centering
  \caption{
  Three stage sleep classification results comparing to previous work based on \textit{sample-wised} evaluation
}
  \resizebox{\textwidth}{!}{%
      \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
    \toprule
    \multicolumn{1}{|c|}{\textbf{Dataset and Feature Set}} & \textbf{Fusion Stage} & \textbf{Model} & \textbf{Accuracy} & \textbf{Cohen Kappa} & \textbf{F1} & \textbf{Precision} & \textbf{Sensitivity} & \textbf{Specificity} \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{MESA (Activity Counts, HRS)}} & Early-stage Fusion & CNN (101) ~\cite{Zhai2020MakingSensing} & 75.9 & 61.0 & 70.4 & 71.5 & 70.0 & 85.6 \\
\cmidrule{2-9}      & Hybrid Fusion & ResDeepCNN, Attention-On-Act & \textbf{79.5} & \textbf{67.2} & \textbf{75.5} & \textbf{74.9} & \textbf{76.2} & \textbf{88.5} \\
    \midrule
    Apple Watch (Activity Counts, HR, Time) & Early-stage Fusion & MLP ~\cite{Walch2019SleepDevice} & 71.6 & 24.4 & 48.4 & 63.8 & 46.0 & 71.2 \\
    \midrule
    Apple Watch (Activity Counts, HRS) & Late-stage Fusion & ResDeepCNN-2D, Addition & \textbf{78.2} & \textbf{52.1} & \textbf{67.1} & \textbf{71.6} & \textbf{64.1} & \textbf{82.0} \\
    \bottomrule
    \end{tabular}%
  
      }
  \label{tab:compare_epoch}%
\end{table}%


==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/table_compare_rp.tex <==
\begin{table}[htbp]
  \centering
  \caption{
  Three-stage sleep classification prediction results compared with previous work evaluated at subject level  (mean $\pm$ standard error at 95\% confidence interval)  during the recording period.
}
  \resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\multicolumn{3}{c|}{\textbf{Fusion Specifics}} & \multicolumn{3}{c|}{\textbf{Performance Metrics}} & \multicolumn{3}{c}{\textbf{Time Deviation (min.)}} \\
\midrule
\textbf{Dataset and Feature Set} & \textbf{Fusion Stage} & \textbf{Model} & \textbf{Accuracy (\%)} & \textbf{Cohen's $\kappa$} & \textbf{Mean F1 (\%)} & \textbf{Non-REM sleep} & \textbf{REM sleep} & {\textbf{Wake}} \\
\midrule
\multirow{2}[2]{*}{MESA (ACT-HRV)} & Early-stage Fusion & CNN (101) (Zhai, 2020) & 76.0 $\pm$ 1.0 & 58.6 $\pm$ 1.9 & 68.1 $\pm$ 1.3 & 14.9 $\pm$ 6.7 & -0.5 $\pm$ 4.3 & -14.4 $\pm$ 5.8 \\
  & Hybrid Fusion & \shortstack{ ResDeepCNN \\( Attention-on-Mov)} & \boldmath{}\textbf{79.8 $\pm$ 0.9}\unboldmath{} & \boldmath{}\textbf{65.5 $\pm$ 1.8}\unboldmath{} & \boldmath{}\textbf{73.3 $\pm$ 1.3}\unboldmath{} & -0.9 $\pm$ 6.4 & 6.1 $\pm$ 3.7 & -5.1 $\pm$ 6.3 \\
\midrule
\shortstack{Apple Watch \\(Activity Counts, HR, Time)} & Early-stage Fusion & MLP (Walch, 2019) & 72.1 $\pm$ 2.4 & 23.7 $\pm$ 4.4 & 47.8 $\pm$ 3.6 & 84.2 $\pm$ 17.2 & -65.4 $\pm$ 15.0 & -18.8 $\pm$ 6.1 \\
\midrule
\shortstack{Apple Watch\\ (Activity Counts, HRS)} & Late-stage Fusion & \shortstack{ResDeepCNN \\ Addition} & \boldmath{}\textbf{78.2 $\pm$ 2.3}\unboldmath{} & \boldmath{}\textbf{52.0 $\pm$ 5.8}\unboldmath{} & \boldmath{}\textbf{66.5 $\pm$ 3.8}\unboldmath{} & 1.9 $\pm$ 11.7 & 4.7 $\pm$ 12.6 & -6.5 $\pm$ 7.3 \\
\bottomrule
\end{tabular}%

}
  \label{tab:compare_rp}%
\end{table}%



==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/table_experiment_setting.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[t!]
\caption{Experiment settings based on input modalities, where $l$ is the window length of the input ($l=\{21, 51 ,101\})$, the inputs are for each sleep epoch}
\label{tab:experiment_seetings}
  \centering
  \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|l|l}
    \toprule
    \textbf{\makecell[l]{\textbf{Algorithm}\\\textbf{Type}}} & \textbf{Modality} & \textbf{Input Dimension} & \textbf{Features Used (Full list on Tables \ref{tab:actigraph_features} and \ref{tab:hr_features})} \\
    \midrule
    \multirow{3}[6]{*}{ML} &  \guy  \hspace{0.1em} \textit{[Actigraphy]} & $x \in \mathbb{R}^{370}$ & 370 features were derived from Activity Counts \\
\cmidrule{2-4}      &  \heart  \hspace{0.1em} \textit{[HR/HRV]} & $x \in \mathbb{R}^{30}$ & 30 features were derived from RR intervals \\
\cmidrule{2-4}      & \specialcell{\heart \hspace{0.1em} \guy \\ \textit{[HR/HRV, Actigraphy]} } & $x \in \mathbb{R}^{400}$ & Concatenation of the two modalities above \\
    \midrule
    \multirow{3}[6]{*}{DL} &  \guy  \hspace{0.1em} \textit{[Actigraphy]} & $x \in \mathbb{R}^{l}$ & Activity Counts  \\
\cmidrule{2-4}      &  \heart  \hspace{0.1em} \textit{[HR/HRV]} & $X \in \mathbb{R}^{l\times8}$  & \makecell[l]{8 features were derived from RR intervals: Mean NNi, \\Standard Derivation of RR interval (SDNN),\\ RR interval differences (SDSD), Very Low Frequency, Low Frequency,\\ High Frequency Bands, Low Frequency to High Frequency Ratio and Total Power.}  \\
\cmidrule{2-4}      & \specialcell{\heart \hspace{0.1em} \guy \\ \textit{[HR/HRV, Actigraphy]} } & $X \in \mathbb{R}^{l\times9}$  & Concatenation of the two modalities above \\
    \bottomrule
    \end{tabular}%
    }
%
\end{table}%


==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/table_hyperparameters.tex <==

\begin{table}[h!]
  \centering
  \caption{Hyper-parameters tuning for backbone networks}
    \label{tab:hyperparameters}
    \centering
    \resizebox{\textwidth}{!}{ %{\color{red} % color red
\begin{tabular}{c|c|c|c|c|c|c|c}
\toprule
\textbf{Block/Group} & \textbf{Layer } & \textbf{Kernel size} & \textbf{Number of Kernels} & \textbf{Padding} & \textbf{ Stride} & \textbf{Hidden Units} & \textbf{Drop out Rate} \\
\midrule
\multirow{2}[4]{*}{Convolutional Block 1} & Convolutional Layer 1 \& 2 & 3 & 128, 256, 512 & 1 & 1 &   &  \\
\cmidrule{2-8}  & Maxpooling & 2 &   &   & 2 &   &  \\
\midrule
\multirow{2}[4]{*}{Convolutional Block 2} & Convolutional Layer 3 \& 4 & 3 & 128, 256, 512 & 1 & 1 &   &  \\
\cmidrule{2-8}  & Maxpooling & 2 &   &   & 2 &   &  \\
\midrule
Convolutional Block 3 & Convolutional Layer 5, 6 \& 7 & 3 & 128, 256, 512 & 1 & 1 &   &  \\
\midrule
  & Maxpooling & 2 &   &   & 2 &   &  \\
\midrule
Convolutional Block 4 & Convolutional Layer 8, 9 \& 10 & 3 & 128, 256, 512 & 1 & 1 &   &  \\
\midrule
  & Maxpooling & 2 &   &   & 2 &   &  \\
\midrule
Convolutional Block 4 & Convolutional Layer 11, 12 \& 13 & 3 & 128, 256, 512 & 1 & 1 &   &  \\
\midrule
  & Maxpooling & 2 &   &   & 2 &   &  \\
\midrule
\multirow{2}[4]{*}{FC Block} & Fully Connected Layer 1, 2 &   &   &   &   & 128, 256, 512 &  \\
\cmidrule{2-8}  & Drop Out &   &   &   &   &   & 0.25, 0.75 \\
\bottomrule
\end{tabular}%


    }
    %} % end of color red
\end{table}%


==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/table_inference_time.tex <==

\begin{table}[htbp]
  \caption{The number of model parameters and inference time of each combination of fusion strategies and methods evaluated in millions of parameters and milliseconds respectively with the  \textit{Apple Watch} dataset, using the \textit{ACT-HRS} feature sets based on a window length of 101.}
\centering
\resizebox{0.7\textwidth}{!}{%
% Table generated by Excel2LaTeX from sheet 'final_exclude_split'
\begin{tabular}{c|c|c|c|c}
\toprule
\textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Total Parameters (M)} & \textbf{Inference Time (ms per sample)} \\
\midrule
\multicolumn{1}{c|}{\multirow{2}[4]{*}{Early-Stage}} & DeepCNN & Concatenation & \textbf{9.44} & \boldmath{}\textbf{3.52$\pm$0.08}\unboldmath{} \\
\cmidrule{2-5}  & ResDeepCNN & Concatenation & 9.44 & 3.54$\pm$0.08 \\
\midrule
\multicolumn{1}{c|}{\multirow{4}[4]{*}{Late-Stage Fusion}} & \multirow{2}[2]{*}{DeepCNN} & Concatenation & 48.75 & 22.9$\pm$0.17 \\
  &   & Addition & 9.43 & 32.25$\pm$5.53 \\
\cmidrule{2-5}  & \multirow{2}[2]{*}{ResDeepCNN} & Concatenation & 48.75 & 31.16$\pm$5.06 \\
  &   & Addition & 9.43 & 22.11$\pm$0.25 \\
\midrule
\multicolumn{1}{c|}{\multirow{8}[4]{*}{Hybrid Fusion}} & \multirow{4}[2]{*}{DeepCNN} & Concatenation & 18.80 & 7.13$\pm$0.12 \\
  &   & Addition & 12.24 & 7.01$\pm$0.12 \\
  &   & Attention-on-Act & 19.07 & 7.32$\pm$0.12 \\
  &   & Bilinear & 274.65 & 10.09$\pm$0.11 \\
\cmidrule{2-5}  & \multirow{4}[2]{*}{ResDeepCNN} & Concatenation & 18.80 & 7.02$\pm$0.16 \\
  &   & Addition & 12.24 & 7.0$\pm$0.14 \\
  &   & Attention-on-Act & 19.07 & 7.27$\pm$0.17 \\
  &   & Bilinear & 274.65 & 10.22$\pm$0.17 \\
\bottomrule
\end{tabular}%

    }

  \label{tab:inference_time}%
\end{table}%


%%%%%%%%%%%%% 2021-05-03 BAK %%%%%%%%%
% \begin{tabular}{c|c|c|c|c}
% \toprule
% \textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Model Parameters (Millions)} & \textbf{Inference Time (ms)} \\
% \midrule
% \multicolumn{1}{c|}{\multirow{2}[4]{*}{Early-Stage}} & DeepCNN & Concatenation & \textbf{4.47} & \boldmath{}\textbf{1.38$\pm$0.04}\unboldmath{} \\
% \cmidrule{2-5}  & ResDeepCNN & Concatenation & \textbf{4.47} & \boldmath{}\textbf{1.46$\pm$0.06}\unboldmath{} \\
% \midrule
% \multicolumn{1}{c|}{\multirow{4}[4]{*}{Late-Stage Fusion}} & \multirow{2}[2]{*}{DeepCNN} & Concatenation & 14.29 & 7.28$\pm$0.2 \\
%   &   & Addition & \textbf{4.46} & \boldmath{}\textbf{7.23$\pm$0.14}\unboldmath{} \\
% \cmidrule{2-5}  & \multirow{2}[2]{*}{ResDeepCNN-2D} & Concatenation & 14.29 & 7.8$\pm$0.89 \\
%   &   & Addition & \textbf{4.46} & \boldmath{}\textbf{7.75$\pm$0.85}\unboldmath{} \\
% \midrule
% \multicolumn{1}{c|}{\multirow{10}[4]{*}{Hybrid Fusion}} & \multirow{5}[2]{*}{DeepCNN} & Concatenation & 18.80 & 2.74$\pm$0.16 \\
%   &   & Addition & \textbf{12.24} & \boldmath{}\textbf{2.58$\pm$0.11}\unboldmath{} \\
%   &   & Attention-On-Act & 19.07 & 2.83$\pm$0.1 \\
%   &   & Attention-On-Car & 19.07 & 2.84$\pm$0.1 \\
%   &   & Bilinear & 274.65 & 7.46$\pm$0.23 \\
% \cmidrule{2-5}  & \multirow{5}[2]{*}{ResDeepCNN} & Concatenation & 18.80 & \boldmath{}\textbf{2.73$\pm$0.14}\unboldmath{} \\
%   &   & Addition & \textbf{12.24} & 3.04$\pm$0.65 \\
%   &   & Attention-On-Act & 19.07 & 2.92$\pm$0.1 \\
%   &   & Attention-On-Car & 19.07 & 2.9$\pm$0.1 \\
%   &   & Bilinear & 274.65 & 8.2$\pm$0.81 \\
% \bottomrule
% \end{tabular}%

% \begin{table}[htbp]
%   \caption{The number of model parameters and inference time for each fusion strategy and method in the \textit{Apple} data set, using Activity Counts and HRS feature sets, evaluated in units of millions of parameters and milliseconds. }
% \centering
% \resizebox{0.7\textwidth}{!}{%
%      \begin{tabular}{|c|c|c|c|c|r}
% \cmidrule{1-5}    \textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Number of Model Parameters} & \textbf{Inference Time} &  \\
% \cmidrule{1-5}    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{Early-Stage}} & DeepCNN & Concatenation & 4.471M & 1.38$\pm$0.04 &  \\
% \cmidrule{2-5}      & ResDeepCNN & Concatenation & 4.471M & 1.46$\pm$0.06 &  \\
% \cmidrule{1-5}    \multicolumn{1}{|c|}{\multirow{6}[12]{*}{Late-Stage}} & \multirow{3}[6]{*}{DeepCNN-2D} & Multiplication & 4.461M & 7.1$\pm$0.18 &  \\
% \cmidrule{3-5}      &   & Concatenation & 14.292M & 7.28$\pm$0.2 &  \\
% \cmidrule{3-5}      &   & Addition & 4.461M & 7.23$\pm$0.14 &  \\
% \cmidrule{2-5}      & \multirow{3}[6]{*}{ResDeepCNN-2D} & Multiplication & 4.461M & 7.52$\pm$0.56 &  \\
% \cmidrule{3-5}      &   & Concatenation & 14.292M & 7.8$\pm$0.89 &  \\
% \cmidrule{3-5}      &   & Addition & 4.461M & 7.75$\pm$0.85 &  \\
% \cmidrule{1-5}    \multicolumn{1}{|c|}{\multirow{12}[24]{*}{Hybrid Fusion}} & \multirow{6}[12]{*}{DeepCNN} & Multiplication & 12.244M & 2.85$\pm$0.1 &  \\
% \cmidrule{3-5}      &   & Concatenation & 18.797M & 2.74$\pm$0.16 &  \\
% \cmidrule{3-5}      &   & Addition & 12.244M & 2.58$\pm$0.11 &  \\
% \cmidrule{3-5}      &   & Attention-On-Act & 19.066M & 2.83$\pm$0.1 &  \\
% \cmidrule{3-5}      &   & Attention-On-Car & 19.066M & 2.84$\pm$0.1 &  \\
% \cmidrule{3-5}      &   & Bilinear & 274.651M & 7.46$\pm$0.23 &  \\
% \cmidrule{2-5}      & \multirow{6}[12]{*}{ResDeepCNN} & Multiplication & 12.244M & 2.62$\pm$0.12 &  \\
% \cmidrule{3-5}      &   & Addition & 12.244M & 3.04$\pm$0.65 &  \\
% \cmidrule{3-5}      &   & Concatenation & 18.797M & 2.73$\pm$0.14 &  \\
% \cmidrule{3-5}      &   & Attention-On-Act & 19.066M & 2.92$\pm$0.1 &  \\
% \cmidrule{3-5}      &   & Attention-On-Car & 19.066M & 2.9$\pm$0.1 &  \\
% \cmidrule{3-5}      &   & Bilinear & 274.651M & 8.2$\pm$0.81 &  \\
% \cmidrule{1-5}    \end{tabular}%
%   \label{tab:addlabel}%
%     }

%   \label{tab:inference_time}%
% \end{table}%


==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/table_mesa_act_hrv_epoch.tex <==

\begin{table}[h!]
  \caption{Three-stage sleep classification prediction results for each fusion strategies and methods in the \textit{MEAS-ACT-HRV test} dataset, using Activity Counts and HRV feature sets, evaluated on sleep epoch-wise. }
\centering
\resizebox{0.6\textwidth}{!}{%
    
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \toprule
    \textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Accuracy} & \textbf{Cohen} & \textbf{F1} & \textbf{Precision} & \textbf{Sensitivity} & \textbf{Specificity} \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{Early-Stage Fusion}} & DeepCNN & Concatenation & \textbf{78.2} & \textbf{64.0} & \textbf{73.3} & \textbf{74.5} & \textbf{72.6} & \textbf{86.9} \\
\cmidrule{2-9}      & ResDeepCNN & Concatenation & \textbf{78.3} & \textbf{64.8} & \textbf{72.9} & \textbf{75.5} & \textbf{71.2} & \textbf{86.8} \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{6}[12]{*}{Late-Stage Fusion}} & \multirow{3}[6]{*}{DeepCNN-2D} & Multiplication & 53.8 & 0.0 & 23.3 & 17.9 & 33.3 & 66.7 \\
\cmidrule{3-9}      &   & Concatenation & \textbf{79.5} & \textbf{65.9} & \textbf{74.5} & \textbf{75.6} & \textbf{73.7} & \textbf{87.7} \\
\cmidrule{3-9}      &   & Addition & 79.2 & \textbf{65.9} & 74.1 & \textbf{75.6} & 72.9 & 87.5 \\
\cmidrule{2-9}      & \multirow{3}[6]{*}{ResDeepCNN-2D} & Multiplication & 78.4 & 65.2 & 73.8 & 73.6 & \textbf{74.1} & 87.6 \\
\cmidrule{3-9}      &   & Concatenation & \textbf{79.6} & \textbf{66.4} & \textbf{74.4} & \textbf{76.1} & 73.1 & \textbf{87.9} \\
\cmidrule{3-9}      &   & Addition & 78.5 & 65.2 & 73.5 & 74.3 & 73.1 & 87.3 \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{12}[24]{*}{Hybrid Fusion}} & \multirow{6}[12]{*}{DeepCNN} & Multiplication & \textbf{78.7} & \textbf{66.0} & \textbf{74.4} & \textbf{74.6} & \textbf{75.1} & \textbf{87.6} \\
\cmidrule{3-9}      &   & Concatenation & 78.2 & 64.0 & 73.3 & 74.5 & 72.6 & 86.9 \\
\cmidrule{3-9}      &   & Addition & 78.4 & 65.4 & 73.0 & 74.2 & 72.0 & 87.1 \\
\cmidrule{3-9}      &   & Attention-On-Act & 78.5 & 65.1 & 73.7 & 74.3 & 73.2 & 87.3 \\
\cmidrule{3-9}      &   & Attention-On-Car & 77.1 & 63.5 & 72.6 & 71.7 & 73.7 & 87.3 \\
\cmidrule{3-9}      &   & Bilinear & 75.4 & 61.3 & 71.1 & 70.3 & 72.8 & 86.2 \\
\cmidrule{2-9}      & \multirow{6}[12]{*}{ResDeepCNN} & Multiplication & 79.2 & 67.0 & 74.5 & 75.6 & 73.6 & 86.2 \\
\cmidrule{3-9}      &   & Addition & 79.3 & 65.9 & 74.7 & 75.0 & 74.9 & 87.9 \\
\cmidrule{3-9}      &   & Concatenation & \textbf{79.6} & 66.7 & 74.2 & \textbf{76.9} & 72.4 & 87.5 \\
\cmidrule{3-9}      &   & Attention-On-Act & 79.5 & \textbf{67.2} & \textbf{75.5} & 74.9 & \textbf{76.2} & \textbf{88.5} \\
\cmidrule{3-9}      &   & Attention-On-Car & 79.1 & 65.0 & 74.0 & 75.7 & 72.8 & 87.4 \\
\cmidrule{3-9}      &   & Bilinear & 75.2 & 60.0 & 69.9 & 70.6 & 69.2 & 85.5 \\
    \bottomrule
    \end{tabular}%
    }

  \label{tab:mesa_act_hrv_epoch}%
\end{table}%


==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/table_mesa_act_hrv_rp.tex <==
\begin{table}[htp]
  \centering
  \caption{
 {Three-stage sleep classification results (mean $\pm$ standard error at 95\% confidence interval) for each combination of fusion strategies and methods with the MESA test dataset using the ACT-HRV feature set based on a window length of 101.}
}
  \resizebox{0.95\textwidth}{!}{%

\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\multicolumn{3}{c|}{\textbf{Fusion Specifics}} & \multicolumn{3}{c|}{\textbf{Performance Metrics}} & \multicolumn{3}{c}{\textbf{Time Deviation(min.)}} \\
\midrule
\textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Accuracy(\%)} & \textbf{Cohen's $\kappa$} & \textbf{Mean F1(\%)} & \textbf{Non-REM sleep} & \textbf{REM sleep} & \textbf{Wake} \\
\midrule
\multicolumn{1}{c|}{\multirow{2}[4]{*}{Early-Stage Fusion}} & DeepCNN & Concatenation & 78.6 $\pm$ 0.9 & 62.8 $\pm$ 1.8 & 71.1 $\pm$ 1.3 & 27.1 $\pm$ 6.9 & -6.5 $\pm$ 3.6 & -20.7 $\pm$ 6.4 \\
\cmidrule{2-9}  & ResDeepCNN & Concatenation & 78.0 $\pm$ 1.1 & 60.2 $\pm$ 2.0 & 71.1 $\pm$ 1.4 & 54.1 $\pm$ 7.0 & 1.2 $\pm$ 3.8 & -55.3 $\pm$ 6.6 \\
\midrule
\multicolumn{1}{c|}{\multirow{4}[4]{*}{Late-Stage Fusion}} & \multirow{2}[2]{*}{DeepCNN} & Concatenation & 79.6 $\pm$ 0.9 & 64.3 $\pm$ 1.8 & 72.5 $\pm$ 1.3 & 12.9 $\pm$ 6.6 & 0.1 $\pm$ 3.5 & -13.0 $\pm$ 6.2 \\
  &   & Addition & 78.5 $\pm$ 0.9 & 62.3 $\pm$ 1.8 & 71.1 $\pm$ 1.3 & 25.7 $\pm$ 6.4 & -6.8 $\pm$ 3.3 & -18.9 $\pm$ 6.4 \\
\cmidrule{2-9}  & \multirow{2}[2]{*}{ResDeepCNN} & Concatenation & 79.3 $\pm$ 0.9 & 64.4 $\pm$ 1.7 & 72.6 $\pm$ 1.2 & 8.9 $\pm$ 6.4 & 4.2 $\pm$ 3.4 & -13.1 $\pm$ 6.1 \\
  &   & Addition & 78.6 $\pm$ 1.0 & 62.8 $\pm$ 1.9 & 71.4 $\pm$ 1.3 & 2.4 $\pm$ 6.9 & -3.0 $\pm$ 3.5 & 0.6 $\pm$ 6.7 \\
\midrule
\multicolumn{1}{c|}{\multirow{10}[4]{*}{Hybrid Fusion}} & \multirow{5}[2]{*}{DeepCNN} & Concatenation & 77.6 $\pm$ 1.1 & 62.7 $\pm$ 1.8 & 71.4 $\pm$ 1.3 & -12.7 $\pm$ 7.3 & 7.2 $\pm$ 3.9 & 5.5 $\pm$ 7.0 \\
  &   & Addition & 79.0 $\pm$ 0.9 & 62.9 $\pm$ 1.7 & 70.7 $\pm$ 1.3 & 53.6 $\pm$ 6.9 & -15.0 $\pm$ 3.3 & -38.6 $\pm$ 6.3 \\
  &   & Attention-on-Mov & 79.0 $\pm$ 1.0 & 63.9 $\pm$ 1.8 & 72.1 $\pm$ 1.3 & 2.3 $\pm$ 7.0 & -4.9 $\pm$ 3.5 & 2.6 $\pm$ 6.9 \\
  &   & Attention-on-Car & 78.1 $\pm$ 1.0 & 63.0 $\pm$ 1.7 & 71.6 $\pm$ 1.3 & -2.1 $\pm$ 6.8 & 6.5 $\pm$ 4.0 & -4.4 $\pm$ 6.3 \\
  &   & Bilinear & 75.7 $\pm$ 0.9 & 58.6 $\pm$ 1.8 & 68.8 $\pm$ 1.2 & 3.7 $\pm$ 6.8 & 16.6 $\pm$ 4.0 & -20.3 $\pm$ 6.3 \\
\cmidrule{2-9}  & \multirow{5}[2]{*}{ResDeepCNN} & Concatenation & 79.7 $\pm$ 0.9 & 65.3 $\pm$ 1.7 & 72.7 $\pm$ 1.3 & 6.4 $\pm$ 6.7 & -7.7 $\pm$ 3.4 & 1.3 $\pm$ 6.7 \\
  &   & Addition & \boldmath{}\textbf{79.8 $\pm$ 0.9}\unboldmath{} & 64.1 $\pm$ 1.7 & 72.7 $\pm$ 1.3 & 24.1 $\pm$ 6.9 & -9.7 $\pm$ 3.2 & -14.4 $\pm$ 6.5 \\
  &   & Attention-on-Mov & 79.6 $\pm$ 1.0 & \boldmath{}\textbf{65.5 $\pm$ 1.8}\unboldmath{} & \boldmath{}\textbf{73.3 $\pm$ 1.3}\unboldmath{} & -0.9 $\pm$ 6.4 & 6.1 $\pm$ 3.7 & -5.1 $\pm$ 6.3 \\
  &   & Attention-on-Car & 78.5 $\pm$ 1.0 & 62.7 $\pm$ 1.7 & 70.5 $\pm$ 1.3 & 37.6 $\pm$ 7.0 & -9.5 $\pm$ 4.0 & -28.1 $\pm$ 6.2 \\
  &   & Bilinear & 75.7 $\pm$ 0.9 & 58.6 $\pm$ 1.8 & 68.8 $\pm$ 1.2 & 3.7 $\pm$ 6.8 & 16.6 $\pm$ 4.0 & -20.3 $\pm$ 6.3 \\
\bottomrule
\end{tabular}%

}

  \label{tab:mesa_act_hrv_rp}%
\end{table}%


==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/table_mesa_hrs_epoch.tex <==

\begin{table}[ht]
  \caption{Three-stage sleep classification prediction results for each fusion strategies and methods in the \textit{MEAS test} dataset, using Activity Counts and HRS feature sets, evaluated on sleep epoch-wise. }
\centering
\resizebox{0.8\textwidth}{!}{%
           \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \toprule
    \textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Accuracy} & \textbf{Cohen} & \textbf{F1} & \textbf{Precision} & \textbf{Sensitivity} & \textbf{Specificity} \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{Early-Stage Fusion}} & DeepCNN & Concatenation & \textbf{77.04} & \textbf{63.78} & \textbf{72.61} & \textbf{71.83} & \textbf{73.62} & \textbf{87.17} \\
\cmidrule{2-9}      & ResDeepCNN & Concatenation & \textbf{79.43} & \textbf{65.66} & \textbf{74.06} & \textbf{76.18} & \textbf{72.58} & \textbf{87.72} \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{6}[12]{*}{Late-Stage Fusion}} & \multirow{3}[6]{*}{DeepCNN-2D} & Multiplication & 53.8 & 0.0 & 23.3 & 17.9 & 33.3 & 66.7 \\
\cmidrule{3-9}      &   & Concatenation & \textbf{79.2} & \textbf{66.7} & \textbf{74.7} & \textbf{74.8} & \textbf{74.6} & \textbf{88.1} \\
\cmidrule{3-9}      &   & Addition & 77.4 & 64.3 & 72.1 & 72.5 & 71.8 & 87.0 \\
\cmidrule{2-9}      & \multirow{3}[6]{*}{ResDeepCNN-2D} & Multiplication & 77.8 & 64.2 & 71.9 & 74.5 & 70.1 & 86.4 \\
\cmidrule{3-9}      &   & Concatenation & \textbf{79.6} & 66.1 & \textbf{73.4} & \textbf{77.9} & 70.8 & \textbf{87.1} \\
\cmidrule{3-9}      &   & Addition & 77.6 & 63.8 & 71.7 & 73.6 & 70.5 & 86.4 \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{12}[24]{*}{Hybrid Fusion}} & \multirow{6}[12]{*}{DeepCNN} & Multiplication & \textbf{79.79} & \textbf{66.51} & \textbf{74.76} & 76.16 & \textbf{73.64} & \textbf{87.94} \\
\cmidrule{3-9}      &   & Concatenation & 79.53 & 66.38 & 74.29 & 76.42 & 72.73 & 87.54 \\
\cmidrule{3-9}      &   & Addition & 78.71 & 64.93 & 73.38 & \textbf{76.53} & 71.68 & 86.62 \\
\cmidrule{3-9}      &   & Attention-On-Act & 79.56 & 66.19 & 74.41 & 76.22 & 73.05 & 87.75 \\
\cmidrule{3-9}      &   & Attention-On-Car & 78.77 & 65.17 & 73.65 & 74.34 & 73.06 & 87.53 \\
\cmidrule{3-9}      &   & Bilinear & 75.35 & 60.34 & 70.28 & 71.42 & 69.98 & 85.23 \\
\cmidrule{2-9}      & \multirow{6}[12]{*}{ResDeepCNN} & Multiplication & 79.42 & \textbf{67.34} & \textbf{75.11} & 74.95 & \textbf{75.26} & \textbf{88.24} \\
\cmidrule{3-9}      &   & Addition & 78.82 & 65.16 & 73.40 & \textbf{77.62} & 71.17 & 86.43 \\
\cmidrule{3-9}      &   & Concatenation & 78.78 & 65.10 & 74.02 & 74.99 & 74.12 & 87.41 \\
\cmidrule{3-9}      &   & Attention-On-Act & \textbf{79.62} & 66.67 & 74.95 & 76.48 & 74.21 & 87.61 \\
\cmidrule{3-9}      &   & Attention-On-Car & \textbf{79.24} & 65.12 & 73.23 & 76.06 & 71.35 & 87.26 \\
\cmidrule{3-9}      &   & Bilinear & 75.48 & 59.96 & 69.99 & 72.04 & 69.40 & 85.07 \\
    \bottomrule
    \end{tabular}%
    }

  \label{tab:mesa_hrs_epoch}%
\end{table}%


==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/table_mesa_hrs_rp.tex <==
\begin{table}[htbp]
  \centering
  \caption{
  Three-stage sleep classification results (mean $\pm$ standard error at 95\% confidence interval) for each combination of fusion strategies and methods with the MESA test dataset using the ACT-HRS feature set based on a window length of 101.
}
  \resizebox{0.95\textwidth}{!}{%

\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\multicolumn{3}{c|}{\textbf{Fusion Specifics}} & \multicolumn{3}{c|}{\textbf{Performance Metrics}} & \multicolumn{3}{c}{\textbf{Time Deviation(min.)}} \\
\midrule
\textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Accuracy(\%)} & \textbf{Cohen's $\kappa$} & \textbf{Mean F1(\%)} & \textbf{Non-REM sleep} & \textbf{REM sleep} & \textbf{Wake} \\
\midrule
\multicolumn{1}{c|}{\multirow{2}[4]{*}{Early-Stage Fusion}} & DeepCNN & Concatenation & 78.0 $\pm$ 1.0 & 63.4 $\pm$ 1.8 & 72.0 $\pm$ 1.2 & 2.7 $\pm$ 7.0 & 15.6 $\pm$ 4.0 & -18.2 $\pm$ 6.4 \\
\cmidrule{2-9}  & ResDeepCNN & Concatenation & 76.9 $\pm$ 1.1 & 61.9 $\pm$ 1.9 & 71.1 $\pm$ 1.3 & -36.7 $\pm$ 7.8 & 12.1 $\pm$ 4.2 & 24.5 $\pm$ 7.5 \\
\midrule
\multicolumn{1}{c|}{\multirow{4}[4]{*}{Late-Stage Fusion}} & \multirow{2}[2]{*}{DeepCNN} & Concatenation & 79.1 $\pm$ 1.0 & 64.7 $\pm$ 1.7 & 72.8 $\pm$ 1.3 & 0.6 $\pm$ 6.9 & 7.5 $\pm$ 3.7 & -8.1 $\pm$ 6.4 \\
  &   & Addition & 78.1 $\pm$ 0.9 & 62.8 $\pm$ 1.6 & 70.6 $\pm$ 1.2 & 23.1 $\pm$ 6.6 & -4.5 $\pm$ 3.7 & -18.5 $\pm$ 6.3 \\
\cmidrule{2-9}  & \multirow{2}[2]{*}{ResDeepCNN} & Concatenation & 77.8 $\pm$ 1.0 & 62.5 $\pm$ 1.7 & 71.0 $\pm$ 1.3 & -1.1 $\pm$ 7.3 & -0.7 $\pm$ 3.5 & 1.8 $\pm$ 6.8 \\
  &   & Addition & 77.7 $\pm$ 1.0 & 62.6 $\pm$ 1.7 & 70.7 $\pm$ 1.2 & 24.3 $\pm$ 7.0 & 3.7 $\pm$ 3.9 & -28.0 $\pm$ 6.4 \\
\midrule
\multicolumn{1}{c|}{\multirow{10}[4]{*}{Hybrid Fusion}} & \multirow{5}[2]{*}{DeepCNN} & Concatenation & 78.2 $\pm$ 0.9 & 64.4 $\pm$ 1.7 & 70.2 $\pm$ 1.2 & 18.5 $\pm$ 7.1 & -14.6 $\pm$ 3.3 & -3.9 $\pm$ 6.5 \\
  &   & Addition & 78.1 $\pm$ 0.9 & 62.2 $\pm$ 1.8 & 71.2 $\pm$ 1.2 & 14.7 $\pm$ 7.4 & 1.4 $\pm$ 3.6 & -16.1 $\pm$ 6.8 \\
  &   & Attention-on-Mov & 79.2 $\pm$ 0.9 & 63.8 $\pm$ 1.8 & 71.8 $\pm$ 1.3 & 28.1 $\pm$ 7.3 & -4.3 $\pm$ 3.5 & -23.9 $\pm$ 6.5 \\
  &   & Attention-on-Car & 76.6 $\pm$ 1.0 & 61.4 $\pm$ 1.7 & 70.4 $\pm$ 1.2 & -7.4 $\pm$ 7.9 & 17.7 $\pm$ 4.7 & -10.3 $\pm$ 6.7 \\
  &   & Bilinear & 75.6 $\pm$ 0.9 & 58.0 $\pm$ 1.8 & 67.7 $\pm$ 1.2 & 6.3 $\pm$ 7.6 & -8.1 $\pm$ 3.7 & 1.8 $\pm$ 7.1 \\
\cmidrule{2-9}  & \multirow{5}[2]{*}{ResDeepCNN} & Concatenation & 79.4 $\pm$ 1.0 & 64.4 $\pm$ 1.7 & 72.7 $\pm$ 1.2 & 31.7 $\pm$ 6.9 & 4.9 $\pm$ 3.6 & -36.6 $\pm$ 6.3 \\
  &   & Addition & 78.9 $\pm$ 0.9 & 63.6 $\pm$ 1.8 & 72.2 $\pm$ 1.2 & 24.6 $\pm$ 7.0 & 4.9 $\pm$ 3.5 & -29.5 $\pm$ 6.5 \\
  &   & Attention-on-Mov & \boldmath{}\textbf{80.3 $\pm$ 0.9}\unboldmath{} & \boldmath{}\textbf{65.6 $\pm$ 1.7}\unboldmath{} & \boldmath{}\textbf{72.9 $\pm$ 1.3}\unboldmath{} & 35.5 $\pm$ 6.9 & 0.8 $\pm$ 3.6 & -36.3 $\pm$ 6.2 \\
  &   & Attention-on-Car & 79.3 $\pm$ 0.9 & 62.8 $\pm$ 1.7 & 71.1 $\pm$ 1.2 & 29.1 $\pm$ 7.1 & -2.4 $\pm$ 3.7 & -26.7 $\pm$ 6.3 \\
  &   & Bilinear & 74.1 $\pm$ 0.9 & 56.8 $\pm$ 1.7 & 66.9 $\pm$ 1.2 & 6.2 $\pm$ 7.1 & 11.7 $\pm$ 4.2 & -17.9 $\pm$ 6.5 \\
\bottomrule
\end{tabular}%

}
  \label{tab:mesa_hrs_rp}%
\end{table}%



==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/table_raw_intermediate_feature.tex <==

\begin{table}[h]
  \centering
  \caption{
  Three-stage sleep classification results (mean $\pm$ standard error at 95\% confidence interval) using raw accelerometer data and HRS features based on DeepMixCNN and ResDeepMixCNN with the Apple Watch Dataset for each combination of fusion strategy and method. The experiments were performed using the same experimental setting as in the main content and evaluated at the subject level during recording period based on window length of 101.
  }
  \resizebox{0.95\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c}
\toprule
\multicolumn{3}{c|}{\textbf{Fusion Specifics}} & \multicolumn{3}{c|}{\textbf{Performance Metrics}} & \multicolumn{2}{c}{\textbf{Deployment Metrics}} \\
\midrule
\textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Accuracy (\%)} & \textbf{Cohen's $\kappa$} & \textbf{Mean F1 (\%)} & \textbf{Model Size (M)} & \textbf{Inference Time (ms)} \\
\midrule
\multicolumn{1}{c|}{\multirow{2}[4]{*}{Early-Stage}} & DeepMixCNN & Concatenation & 74.8 $\pm$ 2.7 & 34.0 $\pm$ 5.9 & 57.2 $\pm$ 3.5 & 11.9 & 18.86$\pm$1.19 \\
\cmidrule{2-8}  & ResDeepMixCNN & Concatenation & 79.8 $\pm$ 3.1 & 48.9 $\pm$ 7.1 & 64.5 $\pm$ 4.5 & 11.9 & 16.45$\pm$0.43 \\
\midrule
\multicolumn{1}{c|}{\multirow{4}[4]{*}{Late-Stage Fusion}} & \multirow{2}[2]{*}{DeepMixCNN} & Concatenation & 79.2 $\pm$ 2.8 & 48.9 $\pm$ 7.6 & 66.0 $\pm$ 4.6 & 50.8 & 37.03$\pm$0.34 \\
  &   & Addition & 76.7 $\pm$ 2.1 & 38.7 $\pm$ 5.9 & 58.0 $\pm$ 3.7 & 11.5 & 32.75$\pm$0.19 \\
\cmidrule{2-8}  & \multirow{2}[2]{*}{ResDeepMixCNN} & Concatenation & \boldmath{}\textbf{79.1 $\pm$ 3.3}\unboldmath{} & \boldmath{}\textbf{51.4 $\pm$ 8.0}\unboldmath{} & \boldmath{}\textbf{66.7 $\pm$ 4.7}\unboldmath{} & 50.8 & 31.19$\pm$0.72 \\
  &   & Addition & 78.9 $\pm$ 2.8 & 48.4 $\pm$ 6.4 & 63.9 $\pm$ 4.0 & 11.5 & 33.11$\pm$0.33 \\
\midrule
\multicolumn{1}{c|}{\multirow{10}[4]{*}{Hybrid}} & \multirow{5}[2]{*}{DeepMixCNN} & Concatenation & 77.3 $\pm$ 3.3 & 43.9 $\pm$ 7.3 & 63.6 $\pm$ 4.3 & 18.0 & 15.94$\pm$0.22 \\
  &   & Addition & 75.8 $\pm$ 2.6 & 36.7 $\pm$ 7.3 & 59.0 $\pm$ 4.0 & 11.5 & 16.28$\pm$0.57 \\
  &   & Attention-on-Mov & 75.8 $\pm$ 3.1 & 39.4 $\pm$ 7.9 & 60.8 $\pm$ 4.8 & 18.3 & 15.7$\pm$0.18 \\
  &   & Attention-on-Car & 71.9 $\pm$ 3.1 & 30.4 $\pm$ 8.1 & 55.7 $\pm$ 4.8 & 18.3 & 15.7$\pm$0.18 \\
  &   & Bilinear & 73.1 $\pm$ 3.4 & 31.4 $\pm$ 8.2 & 52.3 $\pm$ 5.2 & 273.9 & 18.89$\pm$0.43 \\
\cmidrule{2-8}  & \multirow{5}[2]{*}{ResDeepMixCNN} & Concatenation & 77.7 $\pm$ 2.6 & 42.8 $\pm$ 6.0 & 62.6 $\pm$ 3.5 & 18.0 & 15.6$\pm$0.48 \\
  &   & Addition & 80.3 $\pm$ 2.9 & 48.0 $\pm$ 7.3 & 64.4 $\pm$ 4.3 & 11.5 & 15.65$\pm$0.31 \\
  &   & Attention-on-Mov & 77.1 $\pm$ 2.4 & 44.8 $\pm$ 5.9 & 62.7 $\pm$ 3.6 & 18.3 & 16.24$\pm$0.32 \\
  &   & Attention-on-Car & 75.9 $\pm$ 3.0 & 37.0 $\pm$ 7.7 & 57.7 $\pm$ 4.4 & 18.3 & 16.24$\pm$0.32 \\
  &   & Bilinear & 72.8 $\pm$ 3.2 & 29.8 $\pm$ 6.5 & 52.1 $\pm$ 4.4 & 273.9 & 18.88$\pm$0.4 \\
\bottomrule
\end{tabular}%

}
  \label{tab:raw_data_feature_extraction}%
\end{table}%


==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/table_win_20_50.tex <==
% Apple Watch Data Set Win 50'
\begin{table}[htbp]
  \centering
  \caption{Three-stage sleep classification results (mean $\pm$ standard error at 95\% confidence interval) for each combination of the fusion strategy and method with the Apple Watch dataset using the ACT-HRS feature and evaluated at subject level during the recording period based on the window length of 51.}
    \resizebox{0.9\textwidth}{!}{%

\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\multicolumn{3}{c|}{\textbf{Fusion Specifics}} & \multicolumn{3}{c|}{\textbf{Performance Metrics}} & \multicolumn{3}{c}{\textbf{Time Deviation (min.)}} \\
\midrule
\textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Accuracy (\%)} & \textbf{Cohen's $\kappa$} & \textbf{Mean F1 (\%)} & \textbf{Non-REM sleep} & \textbf{REM sleep} & \textbf{Wake} \\
\midrule
\multicolumn{1}{c|}{\multirow{2}[4]{*}{Early-Stage Fusion}} & DeepCNN & Concatenation & 73.1 $\pm$ 3.1 & 40.5 $\pm$ 6.7 & 58.7 $\pm$ 4.4 & 9.1 $\pm$ 22.5 & -0.1 $\pm$ 23.5 & -9.0 $\pm$ 8.8 \\
\cmidrule{2-9}  & ResDeepCNN & Concatenation & 75.4 $\pm$ 2.9 & 43.9 $\pm$ 6.4 & 61.1 $\pm$ 3.9 & 23.0 $\pm$ 24.1 & -12.5 $\pm$ 23.7 & -10.5 $\pm$ 7.2 \\
\midrule
\multicolumn{1}{c|}{\multirow{4}[4]{*}{Late-Stage Fusion}} & \multirow{2}[2]{*}{DeepCNN} & Concatenation & 74.1 $\pm$ 2.7 & 41.9 $\pm$ 6.1 & 59.8 $\pm$ 3.7 & 12.0 $\pm$ 21.6 & -1.1 $\pm$ 22.1 & -10.9 $\pm$ 7.9 \\
  &   & Addition & 78.0 $\pm$ 2.3 & 50.1 $\pm$ 7.0 & 65.5 $\pm$ 3.6 & 1.3 $\pm$ 16.7 & 11.6 $\pm$ 16.8 & -12.9 $\pm$ 6.6 \\
\cmidrule{2-9}  & \multirow{2}[2]{*}{ResDeepCNN} & Concatenation & 76.6 $\pm$ 2.5 & 45.9 $\pm$ 6.9 & 62.6 $\pm$ 4.2 & 20.1 $\pm$ 18.8 & -13.5 $\pm$ 19.6 & -6.7 $\pm$ 7.8 \\
  &   & Addition & \boldmath{}\textbf{77.7 $\pm$ 2.2}\unboldmath{} & \boldmath{}\textbf{48.1 $\pm$ 6.8}\unboldmath{} & \boldmath{}\textbf{64.6 $\pm$ 4.0}\unboldmath{} & 7.6 $\pm$ 19.5 & 3.4 $\pm$ 19.6 & -11.0 $\pm$ 5.8 \\
\midrule
\multicolumn{1}{c|}{\multirow{10}[4]{*}{Hybrid Fusion}} & \multirow{5}[2]{*}{DeepCNN} & Concatenation & 72.5 $\pm$ 3.2 & 39.0 $\pm$ 6.2 & 58.8 $\pm$ 3.9 & 7.5 $\pm$ 24.6 & 5.3 $\pm$ 24.6 & -12.8 $\pm$ 6.8 \\
  &   & Addition & 73.3 $\pm$ 3.0 & 39.2 $\pm$ 6.3 & 58.4 $\pm$ 3.6 & 17.1 $\pm$ 24.1 & -0.8 $\pm$ 24.1 & -16.3 $\pm$ 5.5 \\
  &   & Attention-on-Mov & 72.6 $\pm$ 3.0 & 39.0 $\pm$ 6.0 & 59.4 $\pm$ 3.4 & 15.1 $\pm$ 23.6 & -1.7 $\pm$ 23.6 & -13.4 $\pm$ 6.6 \\
  &   & Attention-on-Car & 72.7 $\pm$ 2.9 & 37.2 $\pm$ 6.4 & 58.3 $\pm$ 3.7 & 23.7 $\pm$ 21.0 & -8.6 $\pm$ 20.3 & -15.2 $\pm$ 6.1 \\
  &   & Bilinear & 72.3 $\pm$ 2.6 & 38.2 $\pm$ 5.5 & 58.5 $\pm$ 3.2 & 1.4 $\pm$ 20.7 & 12.3 $\pm$ 20.7 & -13.7 $\pm$ 6.3 \\
\cmidrule{2-9}  & \multirow{5}[2]{*}{ResDeepCNN} & Concatenation & 73.6 $\pm$ 2.9 & 41.5 $\pm$ 6.5 & 60.7 $\pm$ 4.1 & 8.8 $\pm$ 23.1 & 1.4 $\pm$ 24.9 & -10.2 $\pm$ 7.4 \\
  &   & Addition & 73.1 $\pm$ 3.1 & 40.5 $\pm$ 6.5 & 59.7 $\pm$ 3.9 & 11.5 $\pm$ 23.8 & -0.8 $\pm$ 24.4 & -10.7 $\pm$ 6.8 \\
  &   & Attention-on-Mov & 74.4 $\pm$ 3.3 & 43.8 $\pm$ 6.1 & 61.7 $\pm$ 3.8 & 11.6 $\pm$ 20.9 & -1.5 $\pm$ 21.5 & -10.1 $\pm$ 6.9 \\
  &   & Attention-on-Car & 73.1 $\pm$ 3.0 & 40.6 $\pm$ 7.1 & 60.4 $\pm$ 4.1 & 2.1 $\pm$ 24.0 & 6.9 $\pm$ 24.3 & -9.0 $\pm$ 7.9 \\
  &   & Bilinear & 74.9 $\pm$ 2.6 & 42.2 $\pm$ 6.5 & 60.2 $\pm$ 3.9 & 22.2 $\pm$ 21.9 & -12.2 $\pm$ 22.0 & -9.9 $\pm$ 7.1 \\
\bottomrule
\end{tabular}%

\label{tab:apple_win_50}%
  }
\end{table}%

%%%%%%%%%%%%%%%%%%% Apple Watch Data set window length = 20 %%%%%%%%%%%%

\begin{table}[htbp]
  \centering
  \caption{Three-stage sleep classification results (mean $\pm$ standard error at 95\% confidence interval) for each combination of fusion strategy and method with the Apple Watch dataset using the ACT-HRS feature and evaluated at subject level during the recording period based on the window length of 21.}
    \resizebox{0.9\textwidth}{!}{%

\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\multicolumn{3}{c|}{\textbf{Fusion Specifics}} & \multicolumn{3}{c|}{\textbf{Performance Metrics}} & \multicolumn{3}{c}{\textbf{Time Deviation (min.)}} \\
\midrule
\textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Accuracy (\%)} & \textbf{Cohen's $\kappa$} & \textbf{Mean F1 (\%)} & \textbf{Non-REM sleep} & \textbf{REM sleep} & \textbf{Wake} \\
\midrule
\multicolumn{1}{c|}{\multirow{2}[4]{*}{Early-Stage Fusion}} & DeepCNN & Concatenation & 71.9 $\pm$ 2.1 & 35.2 $\pm$ 5.5 & 54.9 $\pm$ 3.5 & 22.9 $\pm$ 16.6 & -13.9 $\pm$ 16.8 & -9.0 $\pm$ 8.3 \\
\cmidrule{2-9}  & ResDeepCNN & Concatenation & 73.4 $\pm$ 2.4 & 38.7 $\pm$ 5.8 & 58.0 $\pm$ 3.6 & 17.3 $\pm$ 15.2 & -9.6 $\pm$ 16.0 & -7.7 $\pm$ 9.2 \\
\midrule
\multicolumn{1}{c|}{\multirow{4}[4]{*}{Late-Stage Fusion}} & \multirow{2}[2]{*}{DeepCNN} & Concatenation & 72.4 $\pm$ 2.5 & 38.1 $\pm$ 6.1 & 55.9 $\pm$ 3.9 & 21.9 $\pm$ 18.2 & -7.4 $\pm$ 18.0 & -14.6 $\pm$ 8.6 \\
  &   & Addition & \boldmath{}\textbf{75.3 $\pm$ 2.4}\unboldmath{} & \boldmath{}\textbf{39.7 $\pm$ 7.7}\unboldmath{} & \boldmath{}\textbf{59.2 $\pm$ 4.2}\unboldmath{} & 14.6 $\pm$ 13.9 & -1.4 $\pm$ 15.4 & -13.1 $\pm$ 7.2 \\
\cmidrule{2-9}  & \multirow{2}[2]{*}{ResDeepCNN} & Concatenation & 72.7 $\pm$ 2.6 & 38.3 $\pm$ 6.8 & 57.3 $\pm$ 4.2 & 11.9 $\pm$ 20.3 & -4.5 $\pm$ 21.0 & -7.4 $\pm$ 8.8 \\
  &   & Addition & 74.3 $\pm$ 2.7 & 38.9 $\pm$ 7.5 & 58.9 $\pm$ 4.2 & 6.2 $\pm$ 16.6 & 4.5 $\pm$ 17.6 & -10.7 $\pm$ 7.9 \\
\midrule
\multicolumn{1}{c|}{\multirow{10}[4]{*}{Hybrid Fusion}} & \multirow{5}[2]{*}{DeepCNN} & Concatenation & 71.6 $\pm$ 2.5 & 35.8 $\pm$ 6.2 & 55.6 $\pm$ 4.0 & 17.7 $\pm$ 23.5 & -0.0 $\pm$ 23.4 & -17.7 $\pm$ 6.4 \\
  &   & Addition & 71.6 $\pm$ 2.6 & 35.0 $\pm$ 5.7 & 55.8 $\pm$ 3.6 & 22.9 $\pm$ 19.7 & -5.9 $\pm$ 19.7 & -17.0 $\pm$ 6.7 \\
  &   & Attention-on-Mov & 72.2 $\pm$ 2.6 & 37.3 $\pm$ 5.4 & 56.6 $\pm$ 3.4 & 20.5 $\pm$ 19.6 & -3.6 $\pm$ 20.8 & -16.9 $\pm$ 6.3 \\
  &   & Attention-on-Car & 73.2 $\pm$ 2.3 & 35.4 $\pm$ 5.9 & 56.6 $\pm$ 3.6 & 31.1 $\pm$ 20.6 & -13.3 $\pm$ 20.1 & -17.8 $\pm$ 6.4 \\
  &   & Bilinear & 71.5 $\pm$ 2.9 & 37.3 $\pm$ 6.0 & 57.2 $\pm$ 3.7 & 5.0 $\pm$ 19.1 & 6.9 $\pm$ 17.7 & -11.9 $\pm$ 7.7 \\
\cmidrule{2-9}  & \multirow{5}[2]{*}{ResDeepCNN} & Concatenation & 72.3 $\pm$ 2.7 & 36.6 $\pm$ 6.5 & 57.3 $\pm$ 4.0 & 21.3 $\pm$ 23.8 & -5.3 $\pm$ 23.3 & -15.9 $\pm$ 6.5 \\
  &   & Addition & 71.6 $\pm$ 2.2 & 35.2 $\pm$ 5.2 & 55.5 $\pm$ 3.4 & 24.7 $\pm$ 18.2 & -11.6 $\pm$ 19.1 & -13.2 $\pm$ 6.9 \\
  &   & Attention-on-Mov & 73.3 $\pm$ 2.3 & 38.0 $\pm$ 5.4 & 57.9 $\pm$ 3.3 & 33.5 $\pm$ 17.3 & -19.3 $\pm$ 17.7 & -14.2 $\pm$ 6.4 \\
  &   & Attention-on-Car & 72.1 $\pm$ 2.7 & 37.8 $\pm$ 5.5 & 57.8 $\pm$ 3.6 & 17.5 $\pm$ 19.2 & -5.8 $\pm$ 18.8 & -11.7 $\pm$ 7.9 \\
  &   & Bilinear & 70.5 $\pm$ 2.7 & 35.7 $\pm$ 5.8 & 55.9 $\pm$ 3.6 & 3.1 $\pm$ 19.2 & 1.2 $\pm$ 19.5 & -4.3 $\pm$ 9.8 \\
\bottomrule
\end{tabular}%

  \label{tab:apple_win_20}%
  }
\end{table}%

%%%%%%%%%%%%%%%%%%%%%  MESA HRS Window Length 50 %%%%%%%%%%%%%%%

% Table generated by Excel2LaTeX from sheet 'MESA_HR_stat_subject_rp'
\begin{table}[htbp]
  \centering
  \caption{Three-stage sleep classification results (mean $\pm$ standard error at 95\% confidence interval) for each combination of fusion strategy and method with the MESA test dataset using the ACT-HRS evaluated at subject level during the recording period based on the window length of 51.}
   \resizebox{0.9\textwidth}{!}{%

\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\multicolumn{3}{c|}{\textbf{Fusion Specifics}} & \multicolumn{3}{c|}{\textbf{Performance Metrics}} & \multicolumn{3}{c}{\textbf{Time Deviation (min.)}} \\
\midrule
\textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Accuracy (\%)} & \textbf{Cohen's $\kappa$} & \textbf{Mean F1 (\%)} & \textbf{Non-REM sleep} & \textbf{REM sleep} & \textbf{Wake} \\
\midrule
\multicolumn{1}{c|}{\multirow{2}[4]{*}{Early-Stage Fusion}} & DeepCNN & Concatenation & 78.1 $\pm$ 0.9 & 60.1 $\pm$ 1.8 & 69.3 $\pm$ 1.3 & 14.6 $\pm$ 7.3 & -18.7 $\pm$ 3.6 & 4.1 $\pm$ 6.9 \\
\cmidrule{2-9}  & ResDeepCNN & Concatenation & 76.7 $\pm$ 1.0 & 60.2 $\pm$ 1.9 & 70.3 $\pm$ 1.3 & -15.6 $\pm$ 7.4 & 12.6 $\pm$ 5.0 & 3.0 $\pm$ 6.8 \\
\midrule
\multicolumn{1}{c|}{\multirow{4}[4]{*}{Late-Stage Fusion}} & \multirow{2}[2]{*}{DeepCNN} & Concatenation & \boldmath{}\textbf{78.4 $\pm$ 1.0}\unboldmath{} & \boldmath{}\textbf{62.5 $\pm$ 1.8}\unboldmath{} & \boldmath{}\textbf{71.4 $\pm$ 1.3}\unboldmath{} & 9.9 $\pm$ 7.3 & 0.2 $\pm$ 4.1 & -10.0 $\pm$ 6.4 \\
  &   & Addition & 76.5 $\pm$ 0.9 & 58.8 $\pm$ 1.7 & 66.7 $\pm$ 1.2 & 62.3 $\pm$ 7.4 & -21.7 $\pm$ 3.7 & -40.6 $\pm$ 6.9 \\
\cmidrule{2-9}  & \multirow{2}[2]{*}{ResDeepCNN} & Concatenation & 77.7 $\pm$ 0.9 & 61.0 $\pm$ 1.8 & 69.9 $\pm$ 1.2 & 17.3 $\pm$ 7.6 & -4.6 $\pm$ 4.2 & -12.6 $\pm$ 6.6 \\
  &   & Addition & 74.8 $\pm$ 1.0 & 55.7 $\pm$ 1.8 & 66.2 $\pm$ 1.3 & -21.0 $\pm$ 7.7 & -16.0 $\pm$ 4.2 & 37.0 $\pm$ 7.5 \\
\midrule
\multicolumn{1}{c|}{\multirow{10}[4]{*}{Hybrid Fusion}} & \multirow{5}[2]{*}{DeepCNN} & Concatenation & 76.4 $\pm$ 1.1 & 61.1 $\pm$ 1.8 & 70.0 $\pm$ 1.3 & -9.4 $\pm$ 8.0 & 17.9 $\pm$ 5.0 & -8.5 $\pm$ 6.9 \\
  &   & Addition & 77.2 $\pm$ 1.0 & 61.3 $\pm$ 1.7 & 70.6 $\pm$ 1.2 & -17.9 $\pm$ 7.5 & 2.5 $\pm$ 4.3 & 15.4 $\pm$ 7.0 \\
  &   & Attention-on-Mov & 74.6 $\pm$ 1.1 & 59.1 $\pm$ 1.8 & 69.0 $\pm$ 1.2 & -24.0 $\pm$ 8.1 & 39.2 $\pm$ 5.7 & -15.3 $\pm$ 6.6 \\
  &   & Attention-on-Car & 77.8 $\pm$ 0.9 & 60.7 $\pm$ 1.8 & 69.8 $\pm$ 1.2 & 5.4 $\pm$ 7.4 & -9.2 $\pm$ 4.1 & 3.8 $\pm$ 6.7 \\
  &   & Bilinear & 77.1 $\pm$ 0.9 & 60.1 $\pm$ 1.8 & 70.2 $\pm$ 1.2 & 6.8 $\pm$ 8.0 & 13.9 $\pm$ 5.0 & -20.8 $\pm$ 6.5 \\
\cmidrule{2-9}  & \multirow{5}[2]{*}{ResDeepCNN} & Concatenation & 77.7 $\pm$ 1.0 & 62.4 $\pm$ 1.7 & 71.0 $\pm$ 1.2 & 8.3 $\pm$ 7.7 & 15.5 $\pm$ 5.0 & -23.8 $\pm$ 6.3 \\
  &   & Addition & 78.5 $\pm$ 0.9 & 62.0 $\pm$ 1.7 & 71.3 $\pm$ 1.2 & 30.4 $\pm$ 7.3 & 4.1 $\pm$ 4.3 & -34.5 $\pm$ 6.5 \\
  &   & Attention-on-Mov & 76.1 $\pm$ 1.1 & 60.7 $\pm$ 1.8 & 70.4 $\pm$ 1.3 & -9.9 $\pm$ 8.2 & 31.3 $\pm$ 5.7 & -21.4 $\pm$ 6.8 \\
  &   & Attention-on-Car & 76.6 $\pm$ 1.1 & 61.2 $\pm$ 1.8 & 70.7 $\pm$ 1.2 & -0.3 $\pm$ 7.6 & 25.8 $\pm$ 5.1 & -25.6 $\pm$ 6.2 \\
  &   & Bilinear & 76.7 $\pm$ 0.9 & 60.2 $\pm$ 1.7 & 69.7 $\pm$ 1.2 & -9.5 $\pm$ 7.6 & 9.4 $\pm$ 4.6 & 0.1 $\pm$ 6.6 \\
\bottomrule
\end{tabular}%

    }
  \label{tab:mesa_hrs_win_50}%
\end{table}%

%%%%%%%%%%%%%%%%%%%%%  MESA HRS Window Length 20 %%%%%%%%%%%%%%%

% Table generated by Excel2LaTeX from sheet 'MESA_HR_stat_subject_rp'
\begin{table}[htbp]
  \centering
  \caption{Three-stage sleep classification results (mean $\pm$ standard error at 95\% confidence interval) for each combination of fusion strategy and method with the MESA test dataset using the ACT-HRS evaluated at subject level during the recording period based on the window length of 21.}
     \resizebox{0.9\textwidth}{!}{%
% Table generated by Excel2LaTeX from sheet 'MESA_HR_stat_subject_rp'
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\multicolumn{3}{c|}{\textbf{Fusion Specifics}} & \multicolumn{3}{c|}{\textbf{Performance Metrics}} & \multicolumn{3}{c}{\textbf{Time Deviation (min.)}} \\
\midrule
\textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Accuracy (\%)} & \textbf{Cohen's $\kappa$} & \textbf{Mean F1 (\%)} & \textbf{Non-REM sleep} & \textbf{REM sleep} & \textbf{Wake} \\
\midrule
\multirow{2}[4]{*}{Early-Stage Fusion} & DeepCNN & Concatenation & 75.3 $\pm$ 1.0 & 55.2 $\pm$ 1.8 & 66.7 $\pm$ 1.2 & 61.4 $\pm$ 7.7 & -4.3 $\pm$ 4.2 & -57.0 $\pm$ 6.8 \\
\cmidrule{2-9}  & ResDeepCNN & Concatenation & 75.0 $\pm$ 0.9 & 56.6 $\pm$ 1.7 & 68.3 $\pm$ 1.1 & 13.3 $\pm$ 7.4 & 16.7 $\pm$ 4.6 & -30.0 $\pm$ 6.5 \\
\midrule
\multicolumn{1}{c|}{\multirow{4}[4]{*}{Late-Stage Fusion}} & \multirow{2}[2]{*}{DeepCNN} & Concatenation & 76.6 $\pm$ 0.9 & 57.8 $\pm$ 1.6 & 68.0 $\pm$ 1.2 & 29.8 $\pm$ 7.0 & -13.9 $\pm$ 3.7 & -15.9 $\pm$ 6.4 \\
  &   & Addition & 74.4 $\pm$ 0.9 & 56.9 $\pm$ 1.6 & 66.8 $\pm$ 1.1 & 13.7 $\pm$ 7.5 & 6.9 $\pm$ 4.8 & -20.7 $\pm$ 6.4 \\
\cmidrule{2-9}  & \multirow{2}[2]{*}{ResDeepCNN} & Concatenation & 75.9 $\pm$ 0.9 & 58.1 $\pm$ 1.6 & 68.8 $\pm$ 1.1 & 7.8 $\pm$ 7.1 & 6.8 $\pm$ 4.1 & -14.7 $\pm$ 6.4 \\
  &   & Addition & 74.7 $\pm$ 0.9 & 56.6 $\pm$ 1.6 & 66.6 $\pm$ 1.1 & 33.4 $\pm$ 7.4 & 2.7 $\pm$ 4.7 & -36.1 $\pm$ 6.4 \\
\midrule
\multicolumn{1}{c|}{\multirow{10}[4]{*}{Hybrid Fusion}} & \multirow{5}[2]{*}{DeepCNN} & Concatenation & 76.0 $\pm$ 0.9 & 57.1 $\pm$ 1.7 & 68.6 $\pm$ 1.2 & 33.8 $\pm$ 7.6 & 8.2 $\pm$ 4.4 & -42.0 $\pm$ 6.7 \\
  &   & Addition & 74.8 $\pm$ 1.0 & 55.7 $\pm$ 1.8 & 67.9 $\pm$ 1.2 & 22.6 $\pm$ 7.8 & 21.7 $\pm$ 4.9 & -44.3 $\pm$ 6.6 \\
  &   & Attention-on-Mov & 74.2 $\pm$ 1.0 & 56.8 $\pm$ 1.7 & 67.9 $\pm$ 1.2 & -25.4 $\pm$ 7.9 & 18.4 $\pm$ 4.7 & 7.0 $\pm$ 7.0 \\
  &   & Attention-on-Car & 76.1 $\pm$ 0.9 & 57.4 $\pm$ 1.6 & 68.3 $\pm$ 1.1 & 13.1 $\pm$ 7.5 & -1.0 $\pm$ 4.3 & -12.1 $\pm$ 6.7 \\
  &   & Bilinear & 76.9 $\pm$ 0.9 & 57.6 $\pm$ 1.7 & 68.0 $\pm$ 1.2 & 26.4 $\pm$ 7.2 & -20.1 $\pm$ 3.6 & -6.3 $\pm$ 6.8 \\
\cmidrule{2-9}  & \multirow{5}[2]{*}{ResDeepCNN} & Concatenation & 76.5 $\pm$ 0.9 & 57.6 $\pm$ 1.7 & 68.6 $\pm$ 1.2 & 47.2 $\pm$ 7.4 & -0.2 $\pm$ 4.1 & -47.0 $\pm$ 6.6 \\
  &   & Addition & 76.2 $\pm$ 0.9 & 57.7 $\pm$ 1.7 & 68.8 $\pm$ 1.2 & 25.0 $\pm$ 7.4 & 7.6 $\pm$ 4.3 & -32.6 $\pm$ 6.6 \\
  &   & Attention-on-Mov & 75.9 $\pm$ 0.9 & 58.1 $\pm$ 1.7 & \boldmath{}\textbf{69.0 $\pm$ 1.1}\unboldmath{} & -0.2 $\pm$ 7.5 & 10.0 $\pm$ 4.3 & -9.8 $\pm$ 6.7 \\
  &   & Attention-on-Car & 75.5 $\pm$ 0.9 & 58.2 $\pm$ 1.7 & 68.8 $\pm$ 1.2 & -5.1 $\pm$ 7.5 & 13.2 $\pm$ 4.6 & -8.2 $\pm$ 6.6 \\
  &   & Bilinear & \boldmath{}\textbf{77.0 $\pm$ 0.9}\unboldmath{} & \boldmath{}\textbf{58.7 $\pm$ 1.6}\unboldmath{} & 68.6 $\pm$ 1.1 & 39.9 $\pm$ 7.1 & -13.1 $\pm$ 3.9 & -26.8 $\pm$ 6.5 \\
\bottomrule
\end{tabular}%

}
  \label{tab:mesa_hrs_win_20}%
\end{table}%


%%%%%%%%%%%%% MESA HRV Window length 50 %%%%%%%%%%%%%%%%%%%%%%
% Table generated by Excel2LaTeX from sheet 'MESA_Subject_rp'
\begin{table}[htbp]
  \centering
  \caption{Three-stage sleep classification results (mean $\pm$ standard error at 95\% confidence interval) for each combination of fusion strategy and method in the MESA test dataset using the ACT-HRV feature set evaluated at subject level during the recording period based on the window length of 51.}
  \resizebox{0.9\textwidth}{!}{%
    % Table generated by Excel2LaTeX from sheet 'MESA_Subject_rp'
% Table generated by Excel2LaTeX from sheet 'MESA_Subject_rp'
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\multicolumn{3}{c|}{\textbf{Fusion Specifics}} & \multicolumn{3}{c|}{\textbf{Performance Metrics}} & \multicolumn{3}{c}{\textbf{Time Deviation (min.)}} \\
\midrule
\textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Accuracy (\%)} & \textbf{Cohen's $\kappa$} & \textbf{Mean F1 (\%)} & \textbf{Non-REM sleep} & \textbf{REM sleep} & \textbf{Wake} \\
\midrule
\multirow{2}[4]{*}{Early-Stage Fusion} & DeepCNN & Concatenation & 75.7 $\pm$ 1.0 & 56.7 $\pm$ 1.8 & 67.2 $\pm$ 1.3 & 40.0 $\pm$ 6.9 & -11.1 $\pm$ 3.9 & -28.9 $\pm$ 6.5 \\
\cmidrule{2-9}  & ResDeepCNN & Concatenation & 76.0 $\pm$ 0.9 & 56.9 $\pm$ 1.8 & 66.8 $\pm$ 1.3 & 63.1 $\pm$ 7.3 & -17.3 $\pm$ 3.6 & -45.9 $\pm$ 6.8 \\
\midrule
\multicolumn{1}{c|}{\multirow{4}[4]{*}{Late-Stage Fusion}} & \multirow{2}[2]{*}{DeepCNN} & Concatenation & 78.4 $\pm$ 0.9 & 61.7 $\pm$ 1.8 & 70.2 $\pm$ 1.3 & 20.8 $\pm$ 6.9 & -10.9 $\pm$ 3.7 & -9.8 $\pm$ 6.4 \\
  &   & Addition & 77.6 $\pm$ 0.9 & 60.5 $\pm$ 1.8 & 69.2 $\pm$ 1.2 & 34.3 $\pm$ 6.9 & -8.6 $\pm$ 3.9 & -25.7 $\pm$ 6.5 \\
\cmidrule{2-9}  & \multirow{2}[2]{*}{ResDeepCNN} & Concatenation & 78.0 $\pm$ 1.0 & \boldmath{}\textbf{62.4 $\pm$ 1.7}\unboldmath{} & \boldmath{}\textbf{71.1 $\pm$ 1.2}\unboldmath{} & 2.8 $\pm$ 7.2 & 3.3 $\pm$ 4.1 & -6.1 $\pm$ 6.4 \\
  &   & Addition & 77.5 $\pm$ 0.9 & 61.1 $\pm$ 1.8 & 70.3 $\pm$ 1.2 & 16.8 $\pm$ 6.9 & 2.4 $\pm$ 4.0 & -19.2 $\pm$ 6.5 \\
\midrule
\multicolumn{1}{c|}{\multirow{10}[4]{*}{Hybrid Fusion}} & \multirow{5}[2]{*}{DeepCNN} & Concatenation & 77.2 $\pm$ 1.0 & 60.3 $\pm$ 1.7 & 69.7 $\pm$ 1.3 & 12.5 $\pm$ 7.5 & -0.5 $\pm$ 4.4 & -12.0 $\pm$ 6.5 \\
  &   & Addition & 76.6 $\pm$ 1.0 & 59.7 $\pm$ 1.8 & 69.7 $\pm$ 1.3 & 14.2 $\pm$ 7.4 & 13.4 $\pm$ 4.6 & -27.6 $\pm$ 6.5 \\
  &   & Attention-on-Mov & 77.5 $\pm$ 1.0 & 61.2 $\pm$ 1.7 & 70.5 $\pm$ 1.3 & 35.3 $\pm$ 7.3 & 5.7 $\pm$ 4.8 & -40.9 $\pm$ 6.4 \\
  &   & Attention-on-Car & 77.8 $\pm$ 0.9 & 60.4 $\pm$ 1.7 & 68.5 $\pm$ 1.3 & 45.2 $\pm$ 7.1 & -20.6 $\pm$ 3.8 & -24.7 $\pm$ 6.4 \\
  &   & Bilinear & 77.1 $\pm$ 1.0 & 60.8 $\pm$ 1.7 & 70.6 $\pm$ 1.2 & 5.4 $\pm$ 6.9 & 12.2 $\pm$ 4.4 & -17.7 $\pm$ 6.2 \\
\cmidrule{2-9}  & \multirow{5}[2]{*}{ResDeepCNN} & Concatenation & 76.7 $\pm$ 1.1 & 60.7 $\pm$ 1.9 & 70.6 $\pm$ 1.3 & 6.2 $\pm$ 7.9 & 23.4 $\pm$ 5.4 & -29.6 $\pm$ 6.3 \\
  &   & Addition & 76.7 $\pm$ 1.1 & 61.3 $\pm$ 1.8 & 70.9 $\pm$ 1.3 & -27.4 $\pm$ 7.2 & 23.5 $\pm$ 4.8 & 3.8 $\pm$ 6.6 \\
  &   & Attention-on-Mov & \boldmath{}\textbf{78.7 $\pm$ 0.9}\unboldmath{} & 62.2 $\pm$ 1.7 & 70.0 $\pm$ 1.3 & 43.9 $\pm$ 6.9 & -17.6 $\pm$ 3.8 & -26.3 $\pm$ 6.4 \\
  &   & Attention-on-Car & 78.3 $\pm$ 0.9 & 62.2 $\pm$ 1.7 & 70.6 $\pm$ 1.3 & 37.7 $\pm$ 7.1 & -4.7 $\pm$ 4.4 & -33.0 $\pm$ 6.2 \\
  &   & Bilinear & 76.8 $\pm$ 1.0 & 59.1 $\pm$ 1.8 & 69.6 $\pm$ 1.2 & 24.0 $\pm$ 7.0 & 6.7 $\pm$ 4.2 & -30.6 $\pm$ 6.2 \\
\bottomrule
\end{tabular}%


    }
  \label{tab:mesa_hrv_win_50}%

\end{table}%

%%%%%%%%%%%%%%%%%%% MESA HRV Window length 20 %%%%%%%%%%%%%%%%%
% Table generated by Excel2LaTeX from sheet 'MESA_Subject_rp'
\begin{table}[htbp]
  \centering
  \caption{Three-stage sleep classification results (mean $\pm$ standard error at 95\% confidence interval) for each combination of fusion strategy and method with the MESA test dataset using the ACT-HRV evaluated at subject level during the recording period based on the window length of 21.}
  \resizebox{0.9\textwidth}{!}{%
 % Table generated by Excel2LaTeX from sheet 'MESA_Subject_rp'
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\multicolumn{3}{c|}{\textbf{Fusion Specifics}} & \multicolumn{3}{c|}{\textbf{Performance Metrics}} & \multicolumn{3}{c}{\textbf{Time Deviation (min.)}} \\
\midrule
\textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Accuracy (\%)} & \textbf{Cohen's $\kappa$} & \textbf{Mean F1 (\%)} & \textbf{Non-REM sleep} & \textbf{REM sleep} & \textbf{Wake} \\
\midrule
\multirow{2}[4]{*}{Early-Stage Fusion} & DeepCNN & Concatenation & 75.9 $\pm$ 0.9 & 57.0 $\pm$ 1.7 & 67.5 $\pm$ 1.2 & 34.7 $\pm$ 7.0 & -10.2 $\pm$ 3.7 & -24.6 $\pm$ 6.6 \\
\cmidrule{2-9}  & ResDeepCNN & Concatenation & 75.4 $\pm$ 0.9 & 56.0 $\pm$ 1.7 & 67.2 $\pm$ 1.2 & 8.5 $\pm$ 7.1 & -10.9 $\pm$ 3.7 & 2.4 $\pm$ 6.7 \\
\midrule
\multicolumn{1}{c|}{\multirow{4}[4]{*}{Late-Stage Fusion}} & \multirow{2}[2]{*}{DeepCNN} & Concatenation & 76.0 $\pm$ 0.9 & 57.5 $\pm$ 1.7 & 68.0 $\pm$ 1.1 & 12.1 $\pm$ 7.1 & -4.5 $\pm$ 3.9 & -7.6 $\pm$ 6.5 \\
  &   & Addition & 74.4 $\pm$ 0.9 & 54.4 $\pm$ 1.7 & 64.0 $\pm$ 1.2 & 26.7 $\pm$ 7.7 & -21.6 $\pm$ 3.8 & -5.1 $\pm$ 7.2 \\
\cmidrule{2-9}  & \multirow{2}[2]{*}{ResDeepCNN} & Concatenation & 76.2 $\pm$ 0.9 & 58.2 $\pm$ 1.7 & 68.0 $\pm$ 1.2 & 16.7 $\pm$ 6.9 & -7.1 $\pm$ 3.8 & -9.6 $\pm$ 6.5 \\
  &   & Addition & 75.3 $\pm$ 0.9 & 56.0 $\pm$ 1.7 & 65.4 $\pm$ 1.2 & 38.7 $\pm$ 7.6 & -19.2 $\pm$ 3.8 & -19.5 $\pm$ 7.0 \\
\midrule
\multicolumn{1}{c|}{\multirow{10}[4]{*}{Hybrid Fusion}} & \multirow{5}[2]{*}{DeepCNN} & Concatenation & 75.8 $\pm$ 1.0 & 57.5 $\pm$ 1.7 & 68.5 $\pm$ 1.2 & 21.2 $\pm$ 7.7 & 3.6 $\pm$ 4.4 & -24.8 $\pm$ 7.0 \\
  &   & Addition & 75.2 $\pm$ 1.0 & 57.0 $\pm$ 1.8 & 68.5 $\pm$ 1.2 & 11.3 $\pm$ 7.4 & 21.4 $\pm$ 5.2 & -32.7 $\pm$ 6.7 \\
  &   & Attention-on-Mov & 75.4 $\pm$ 1.0 & 56.7 $\pm$ 1.7 & 67.7 $\pm$ 1.2 & 15.3 $\pm$ 7.5 & 3.9 $\pm$ 4.9 & -19.3 $\pm$ 6.7 \\
  &   & Attention-on-Car & 74.3 $\pm$ 1.0 & 56.6 $\pm$ 1.7 & 67.8 $\pm$ 1.2 & -14.6 $\pm$ 7.5 & 14.7 $\pm$ 4.6 & -0.1 $\pm$ 6.5 \\
  &   & Bilinear & 74.9 $\pm$ 1.0 & 57.4 $\pm$ 1.8 & 68.3 $\pm$ 1.2 & -13.4 $\pm$ 7.9 & 8.6 $\pm$ 4.3 & 4.7 $\pm$ 7.2 \\
\cmidrule{2-9}  & \multirow{5}[2]{*}{ResDeepCNN} & Concatenation & 75.5 $\pm$ 1.0 & 57.1 $\pm$ 1.8 & 68.7 $\pm$ 1.2 & 19.8 $\pm$ 7.4 & 20.8 $\pm$ 5.0 & -40.6 $\pm$ 6.6 \\
  &   & Addition & 76.2 $\pm$ 0.9 & 58.4 $\pm$ 1.7 & 69.0 $\pm$ 1.2 & 19.6 $\pm$ 7.1 & -0.9 $\pm$ 4.1 & -18.7 $\pm$ 6.6 \\
  &   & Attention-on-Mov & 76.0 $\pm$ 1.0 & \boldmath{}\textbf{58.7 $\pm$ 1.8}\unboldmath{} & \boldmath{}\textbf{69.0 $\pm$ 1.2}\unboldmath{} & 18.5 $\pm$ 7.4 & 10.3 $\pm$ 4.9 & -28.8 $\pm$ 6.4 \\
  &   & Attention-on-Car & 75.4 $\pm$ 1.0 & 58.0 $\pm$ 1.7 & 68.6 $\pm$ 1.2 & 1.5 $\pm$ 7.5 & 12.9 $\pm$ 4.8 & -14.4 $\pm$ 6.5 \\
  &   & Bilinear & \boldmath{}\textbf{76.4 $\pm$ 0.9}\unboldmath{} & 58.7 $\pm$ 1.8 & 68.8 $\pm$ 1.2 & 37.8 $\pm$ 7.1 & -0.8 $\pm$ 4.1 & -36.9 $\pm$ 6.5 \\
\bottomrule
\end{tabular}%


    }
  \label{tab:mesa_hrv_win_20}%
\end{table}%



==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/test_table.tex <==

\begin{table}[htbp]
  \centering
  \caption{
  Three-stage sleep classification prediction results comparing to previous work evaluated on subject level during recording period; (*Average time deviation measured in \textbf{Minutes} from ground truth across all subjects $\pm$ standard error )
}
  \resizebox{\textwidth}{!}{%
      % Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\toprule
\textbf{Dataset and Feature Set} & \textbf{Fusion Stage} & \textbf{Model} & \textbf{Accuracy} & \textbf{Cohen} & \textbf{F1} & \textbf{Precision} & \textbf{Sensitivity} & \textbf{Specificity} & \textbf{Non-REM sleep} & \textbf{REM sleep} & \textbf{Wake} \\
\midrule
\multirow{2}[4]{*}{ \shortstack{MESA \\ (Activity Counts, HRV)}} & Early-stage Fusion & CNN (101) (Zhai, 2020) & \shortstack{ 76.0 \\ (75.0, 77.0) } & \shortstack{ 58.6 \\ (56.7, 60.5) } & \shortstack{ 68.1 \\ (66.8, 69.4) } & \shortstack{ 72.2 \\ (71.0, 73.4) } & \shortstack{ 69.7 \\ (68.4, 71.0) } & \shortstack{ 85.6 \\ (85.0, 86.2) } & \shortstack{ 14.9 \\ (8.2, 21.6) } & \shortstack{ -0.5 \\ (-4.8, 3.8) } & \shortstack{ -14.4 \\ (-20.2, -8.6) } \\
\cmidrule{2-12}  & Hybrid Fusion & ResDeepCNN, Attention-On-Act & \textbf{\shortstack{ 79.5 \\ (78.5, 80.5) }} & \textbf{\shortstack{ 65.1 \\ (63.3, 66.9) }} & \textbf{\shortstack{ 73.4 \\ (72.2, 74.6) }} & \textbf{\shortstack{ 75.1 \\ (73.9, 76.3) }} & \textbf{\shortstack{ 75.7 \\ (74.5, 76.9) }} & \textbf{\shortstack{ 88.4 \\ (87.9, 88.9) }} & \textbf{\shortstack{ -5.4 \\ (-12.1, 1.3) }} & \textbf{\shortstack{ 6.7 \\ (3.1, 10.3) }} & \textbf{\shortstack{ -1.3 \\ (-7.8, 5.2) }} \\
\midrule
 \shortstack{Apple Watch \\ (Activity Counts, HR, Time)} & Early-stage Fusion & MLP (Walch, 2019) & \shortstack{ 72.1 \\ (69.7, 74.5) } & \shortstack{ 23.7 \\ (19.3, 28.1) } & \shortstack{ 47.8 \\ (44.2, 51.4) } & \shortstack{ 57.4 \\ (52.9, 61.9) } & \shortstack{ 49.0 \\ (45.4, 52.6) } & \shortstack{ 71.3 \\ (70.1, 72.5) } & \shortstack{ 84.2 \\ (67.0, 101.4) } & \shortstack{ -65.4 \\ (-80.4, -50.4) } & \shortstack{ -18.8 \\ (-24.9, -12.7) } \\
\midrule
 \shortstack{Apple Watch \\ (Activity Counts, HRS)}& Late-stage Fusion & ResDeepCNN-2D, Addition & \textbf{\shortstack{ 78.4 \\ (76.3, 80.5) }} & \textbf{\shortstack{ 50.1 \\ (43.7, 56.5) }} & \textbf{\shortstack{ 64.5 \\ (60.6, 68.4) }} & \textbf{\shortstack{ 71.6 \\ (67.3, 75.9) }} & \textbf{\shortstack{ 64.2 \\ (60.4, 68.0) }} & \textbf{\shortstack{ 82.2 \\ (80.4, 84.0) }} & \textbf{\shortstack{ 21.3 \\ (6.0, 36.6) }} & \textbf{\shortstack{ -10.5 \\ (-25.9, 4.9) }} & \textbf{\shortstack{ -10.8 \\ (-17.4, -4.2) }} \\
\bottomrule
\end{tabular}%
}
  \label{tab:test}%
\end{table}%


==> Fusion Methods for Sleep Stage Classification (Overleaf-Arxiv)/unused.tex <==

% \begin{enumerate}
%     \item To the best of our knowledge, we are the first study that explore the advanced modality fusion strategies and methods and the influence of features to the performance of modality fusion for the three-stage sleep classification which is a viable task based on movement sensing and cardiac sensing data .
%     \item For ubiquitous practitioners, we compared the data that may generate from commercial or clinical grade research wearables. Or the data that may collected from the consumer devices, for the health study, we may not need this level’s grade of the rigorous. 
%     \item Our study design that facilitate the multimodal fusion for sleep stages monitoring. We found these following insights. Our study provided several guidelines for considering to adopt DL fusion methods for sensing three sleep stages for health ubiquitous computing to solve real world sleep health problem. We also provided some useful insides towards strength model prediction reliability by adopting multimodal fusion methods on health related research that using ubiquitous methods on physiological signals. For non-machine learning application researchers in Ubicomp, we could understand how does the advanced ML model might influence the sleep health research. 

% \end{enumerate}


% \begin{itemize}
%     \item \textbf{Simple operation-based method} For Simple operation-based method, we have concatenation, weighted sums and multiplication.
%     \item \textbf{Attention-based fusion} Attention mechanisms are widely used for fusion physiological signals. It often refers to the weighted sum of set of vectors with scalar weights that are dynamically generated by a small “attention” model at each time-step. Multiple glimpses are often used to generate multiple sets of dynamic weights for summation, which can preserve additional information by concatenating the results derived from each glimpse.
%     \begin{itemize}
%         \item \textbf{GlobalFusion} method is proposed by Liu and Yao et.al. which is an effective multimodal fusion method for human activity recognition. 
%         \item \textbf{Gated multimodal attention} is Blah Blah.
%     \end{itemize}
%     \item \textbf{Bilinear Pooling-based attention} Second-order statistic pooling is an example of it

% \end{itemize}


% \begin{table}[ht!]
%   \centering
%   \caption{Models and Experiments Plan}
%   \resizebox{0.99\textwidth}{!}{
%     \begin{tabular}{|p{19.39em}|p{26em}|p{9.335em}|}
%     \toprule
%     \textbf{Fusion Strategies} & \textbf{Models, Methods and Networks} & \textbf{Status} \\
%     \midrule
%     \multicolumn{3}{|p{54.725em}|}{\textbf{Early Fusion}} \\
%     \midrule
%     Joint representation & Concatenation of modalities on network & Done, it is the baseline \\
%     \midrule
%     Split representation & Separate representation learning for each modality then adopt simple operation based fusion method & Done \\
%     \midrule
%     Sharing representation & Sharing weights over modalities ?? & To Do \\
%     \midrule
%     Residual connection with intra-modality fusion & Concatenation of modalities & Done \\
%     \midrule
%     Residual connection with inter-modality fusion & Fusion on each level of representations and then adopt simple operation-based method & Done \\
%     \midrule
%     \multicolumn{3}{|p{54.725em}|}{\textbf{Attention-based Fusion }} \\
%     \midrule
%     \multirow{2}[2]{*}{GlobalFusion} & Multimodality multi-level of representation attention & \multirow{2}[2]{*}{TODO} \\
%     \multicolumn{1}{|r|}{} & Bing: One or two? & \multicolumn{1}{r|}{} \\
%     \midrule
%     \multicolumn{3}{|p{54.725em}|}{\textbf{Tensor-based Fusion}} \\
%     \midrule
%     Bilinear Pooling-based Attention & Second-order statistics pooling, & Done \\
%     \midrule
%     \multicolumn{3}{|p{54.725em}|}{\textbf{Late Fusion}} \\
%     \midrule
%     Score level fusion & Select top 5 classifiers and do mean, max posterior fusion & TODO \\
%     \midrule
%     Decision level fusion & Select top 5 networks to do weighted voting (inverse overfitting scores) & TODO \\
%     \bottomrule
%     \end{tabular}}%
%   \label{tab:addlabel}%
% \end{table}%


% \begin{table}[htbp]
%   \centering
%   \caption{Add caption}
%     \resizebox{0.99\textwidth}{!}
%     {\begin{tabular}{|p{25.72em}|r|p{23.835em}|}
%     \toprule
%     \textbf{Paper} & \multicolumn{1}{p{3.335em}|}{\textbf{Citation}} & \textbf{Potential for Sleep Takss} \\
%     \midrule
%     \textbf{Decision-level fusion in fingerprint verification} & \multirow{5}[2]{*}{521} & Multiple samples different window lengths, \\
%     Abstract: &   & Multiple representations (feature sets) from different modality \\
%     We propose to use a combination of four different fingerprint-based biometric systems where each system uses different feature extraction and/or matching algorithms to generate a matching score which can be interpreted as the confidence level of the matcher. These different matching scores are combined to obtain the lowest possible FRR for a given FAR. &   & Multiple loss functions (optimization diversity) \\
%     \multicolumn{1}{|r|}{} &   & Multiple network architectures (classifier diversity) \\
%     We also compare the performance of our integration strategy with the sum and the product rules [2]. Even though we propose and report results in scenarios (iii)–(v), our combination strategy could be used for scenarios (i) and (ii) as we &   & \multicolumn{1}{r|}{} \\
%     \midrule
%     \textbf{Feature-level and decision-level fusion of noncoincidently sampled sensors for land mine detection} & 161 & It’s a likelihood-ratio based decision fusion from various sensors. \\
%     \midrule
%     \multirow{2}[2]{*}{\textbf{Multimodal decision-level fusion for person authentication}} & \multirow{2}[2]{*}{204} & k-Means Algorithm \\
%     \multicolumn{1}{|r|}{} &   & do the k-means on the layer before FC \\
%     \midrule
%     \textbf{Threshold-optimized decision-level fusion and its application to biometrics} & 89 & Threshold based decision fusion \\
%     \midrule
%     \textbf{Decision-level fusion strategies for correlated biometric classifiers} & 49 & likelihood ratio test(LRT) and particle swarm optimization (PSO) \\
%     \midrule
%     \textbf{A comparison of decision-level sensor-fusion methods for anti-personnel landmine detection} & 111 & Dempster–Shafer theory not sure \\
%     \bottomrule
%     \end{tabular}}%
%   \label{tab:addlabel}%
% \end{table}%

% Taking into account the class imbalance in the data set, the mean F1 score used in this study is the average mean F1 score of each class  ($ \text{mean }F_1 = \frac{1}{C} \sum\limits_{c=1}^{C}\frac{2P_cR_c}{P_c+R_c}$, $P_c$ and $R_c$ denotes the class-wise precision and recall respectfully).  

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{Figures/mesa_deepcnn_baseline_intensity_area_sum_abs_per_stage_v1.png}
% 	\caption{Ensemble model. The model starts by taking inputs from different window lengths ($l$) from the multi-modal sensors. A total of six different classifiers are used, combining a mixture of CNNs and LSTMs and exploiting their individual strengths. This results on posterior probability confusion matrix that is then combined through concatenation as part of the ensemble architecture. Finally, the decision making layer takes place by either (a) using a maximum operator approach or (b) a mean operator across all classifiers}
%     \label{fig:fig1}
% \end{figure}

% \begin{figure}
% \centering
% \subfloat[legend]{\label{a}\includegraphics[width=.45\linewidth]{nrem_pid_4294_idx_342_thres_0.8.jpeg}}\hfill
% \subfloat[legend]{\label{b}\includegraphics[width=.45\linewidth]{nrem_pid_4294_idx_342_thres_0.8.jpeg}}\hfill
% \subfloat[legend]{\label{c}\includegraphics[width=.45\linewidth]{nrem_pid_4294_idx_342_thres_0.8.jpeg}}\hfill
% \caption{my fig}
% \label{fig}
% \end{figure}


%further define the sleep label as 
%we aim to output the sleep stage label corresponding to centre point of the sliding window, as shown in Fig. ~\ref{fig:system_overview}.
%Sliding window with size $T$ and stride $S$ were used.
%(i.e.,with $T=101$ sleep epoches, equivalent to $101\times 30s/60s=50.5$ minutes)
%demonstrates the pipeline of our system.
%Based on each epoch (30 seconds), cardiac features and movement features can be extracted, serving as a sample (i.e., multivariate signal at a timestamp) in the feature streams.  %time series data. 
%Sliding window with size $T$  was employed and the stride $S$ was set to $S=1$ such that there will be a prediction at each sleep epoch.



%we focus on studying how to better utilize advanced fusion techniques
%strategies and methods to produce a reliable mode that can better classifying three sleep stages using movement sensing and cardiac sensing. 
%For each modality, we may extract one or more medical features that can be used for multimodal fusion and deep learning networks.

%Before diving into the details, we first introduce the notations used for the rest of this paper. 
%All vectors are denoted by bold lower-case letters (e.g., $\matr{x}$ and $\matr{y}$). 
%All matrices and tensors are represented by bold upper-case letters(e.g. $\matr{X}$ and $\matr{Y}$). 
%For a vector $\matr{x}$, the $j^{th}$ element is denoted by $x_j$.
%For each modality, we use the superscript to denote the modality where it came from. 
%For example, $\matr{X^{car}}$ means the feature matrix for cardiac sensing. 

%After 

% \begin{itemize}
% % 	\item \textbf{Accuracy} counts the number of correctly classified sleep epochs, normalized over the total number of sleep epochs ($\text{Acc} =\frac{TP+TN}{TP+TN+FP+FN}$).
	
% % 	\item \textbf{Recall} measures the proportion of positives that are correctly identified as the given stage ($R = \frac{TP}{TP+FN}$).
	
% % 	\item \textbf{Specificity}, also known as true negative rate, measures the proportion of negatives that are correctly identified as the given stage ($S = \frac{TN}{FP+TN}$).
	
% % 	\item \textbf{Precision} is the fraction of correct classified instances among the overall positive predictions ($P=\frac{TP}{TP+FP}$).
	
% % 	\item \textbf{$\mathbf{F_1}$ score (Macro $\mathbf{F_1}$)} is the harmonic mean between precision and recall, where the average is calculated per label and then averaged across all labels ($macro F_1 = \frac{1}{C} \sum\limits_{c=1}^{C}\frac{2P_cR_c}{P_c+R_c}$, $P_c$ and $R_c$ denotes the class-wise precision and recall respectfully).
	
% % 	\item \textbf{Cohen's Kappa ($\kappa$)} measures inter-rater reliability/agreement, comparing observed accuracy with an expected accuracy 
% % 	($\kappa = \frac{P_o - P_e}{1 - P_e}$,
% % 	where $P_o$ the observed proportional agreement and and $P_e$ the
% % 	expected proportion of agreement). In this context, Cohen's $\kappa$ factors out agreement by chance arising from the class imbalance of different sleep stages throughout the night. 
	
% 	\item \textbf{Time Deviation} We also evaluated 
% 	\item \textbf{Model Parameters and Inference Time} We count the number of model parameters to compare the size of the model which is a consideration to deploy the model in a real world mobile or edge computer equipment. We also evaluated the model inference time which is also a key consideration to the user experience and power consumption.
% \end{itemize}


% \section{Limitation and Future Work}
% The strength of this work derives from the study of the advanced fusion strategies and methods on two sleep data scenarios and the systematic design and in-depth analysis. This makes an important contribution to the literature with potential applications for clinicians, ubiquitous practitioners and the wellness industry engineers as we can achieve a reasonable performance on three-stage sleep classification without using EEG or adding extra modalities. Especially, the Apple Watch data set scenario proves that we can achieve a good result through fusion. 
% Given the fact that, the demographic factors, device, signal processing and sample size differences between these two datasets. Another limitation is that we did not explore the impact of model results trained on MESA and tested on the Apple dataset or the reverse process. It is a well know problem of data driven approach does not generalise well on different dataset or domain. We plan to address the domain adaption issues in our future work, such as how to use limited labelled data or unlabelled data to better fit to the target domain.

% In this study, we only explored the most commonly used fusion methods on convolutional neural network architecture. We did not explore tens and hundreds of fusion methods. Such as fusing over multiple convolutional layers or fusing with heterogeneous network structures such as LSTM. All our experiments are performed on a fixed windows length (101 sleep epochs) and we concentrate on multimodal fusion rather than the multiple window lengths fusion, although previous work showed that different window sizes carry different discriminative information. Future research may consider the best way to fuse information from various or dynamic window lengths.

% Given the scope of our work and objective, we did not perform the analysis to show how different models perform in diseased versus healthy population or highlight the differences between them.  We also did not consider the use of ultradian periodicity~\cite{Hobson1975SleepGroups}, the approximately 90-min sleep cycle, we tested several mixed models such as CNN + LSTM and did not observe improvement on the prediction of each sleep epoch. 

% For visualisation, we did not perform the quantitative studies the previous sleep physiological journal. Since Grad-CAM is applied to the last convolutional layer, it does not incorporate the computation performed by the last layer (the fully-connected hidden layer), and thus may not be entirely representative of the features supporting the network's decision~\cite{Jonas2019EEG-basedFeatures}.  The visualisation is only used to see whether these post-threshold filtering features highlighted by the model are similar to those mentioned in the sleep physiology study. The physiological significance behind the dynamic changes of these features in the time dimension is beyond the scope of existing medical knowledge and also not all samples are the same. 

% Finally, the use of multimodal fusion methods will inevitably increase the size of the model, which is still a concern for ubiquitous computing applications and deserves attention in future work. For example, how to reduce the size of parameters and maintain the performance of the model through knowledge distillation methods.

%This means that representation learning using early fusion tends to be less affected by noisy modalities, which may disregard the noisy signals, that hinders the learning of inter-modal relationship. 
%This means that representation learning using early fusion will not make full use of the relationship between modalities, and in most cases may not be able to learn useful information from modalities with a lot of noise.

%multimodalities because many studies use the unimodal features derived from pre-trained backbone models and use fusion methods to combine them. 


%  Firstly, the measurement methods are not standardised. Secondly, the lack of precise understanding of the physiological origins that influences the signal waveform. Thirdly, these signals' reliability and specificity are relatively low compared to the existing clinical methods

%Being able to access raw data provides medical and sleep health researchers with the opportunities to develop transparent sleep stage classification algorithms, which facilitates comparative studies. 
% The performance of using neural network models in three-stage sleep classification is much better than traditional models. But we do not know the decision-making process of these models, in this work, we will also explore the decision-making process to gain a better understand by visualising the deep neural networks.

%we focus on studying how to better utilize advanced fusion techniques
%strategies and methods to produce a reliable mode that can better classifying three sleep stages using movement sensing and cardiac sensing. 
% Clinical sleep monitoring and assessment have long been recognised as a manual multimodal classification task using various types of sensors in the PSG study.
%Fusion can be invoked at different levels in the traditional machine learning pipeline. 
%The most significant modules to complete recognition or classification tasks are sensor modules, segmentation modules, feature extraction modules and the classification or decision-making modules~\cite{Ross2001InformationBiometrics}.  Based on the operations that occur after different modules, 


%from other research fields to study the three-stage sleep classification, , namely early-stage fusion, late-stage fus1ion or hybrid fusion. 
%We select five commonly used methods in our study which can be divided into three categories, the simple operation, attention mechanism based method, and tensor-based method. 

%We only performed the inference process on the CPU and do not use the GPU resources as the GPU hardware may vary greatly in real world scenarios.

% Table ~\ref{tab:inference_time} shows the inference time, in early-fusion strategy, the total number of parameters of two backbone networks are the second lowest and the inference time is the lowest. Their F1 score and accuracy remains in the middle level.The model with the highest F1 score among all fusion strategies is ResDeepCNN-2D using the addition method in late-fusion strategy. It also has the least model parameters, but its inference time is the slowest. In Hybrid Fusion, the bilinear model has the highest parameters and the longest inference time, and the worst F1 score and accuracy. In the same category, the best performance mode is ResDeepCNN using the Attention-On-Mov method. Although its number of model parameters is 4.3 times greater than the best model (ResDeepCNN-2D using Addition method) in late-stage, the average time of forward propagation is about 2.6 times faster than that model. In addition, there is no significant difference in their F1 scores.

%In summary, if the application scenario has limitations on running time and power consumption, hybrid-fusion can improve prediction performance without increasing the running time that much. If the application scenario has restrictions on model size (a.k.a memory restriction), then late-stage fusion may provide an alternative option.


%In this work, based on two dataset scenarios,  we systematically studied three fusion strategies and four fusion methods. The data in the first scenario was collected from a group of young and healthy adults using the Apple Watch, which has gold ground truth labels annotated from PSG recordings.The second scenario is the MESA dataset, which is collected from a large diverse population of both healthy and sleep disordered participants from an aged population. The main purpose of this work is to understand how different fusion strategies and fusion methods can improve robustness of the three-stage classification model. Through this research, we have confirmed that the three-stage sleep classification is a practical task, and the model obtained using multimodal fusion techniques can achieve state-of-the-art performance. In addition, this work highlights the strengths and limitations of the different techniques. It provides a guideline to use multimodal fusion approaches to develop the state-of-the-art models that may be able to deploy on research/consumer-grade wearable devices in a transparent way.

%From Grad-CAM plot we observed that, the activity counts, mean NNI and the ratio of LF to HF for that sample are the top three most important features for classifying Wake. For NREMS classification, the activity counts, VLF, LF, and the ratio of LF to HF are showed as the important feature for the classifier. For the REMS classification, we can see all the highlighted areas are the features derived from HRV. These phenomena have some similarities with HRV characters that have been confirmed 

% Visualisation

% To better understand the decision making process of multimodal fusion, we use the gradient class activation map(Grad-Cam)~\cite{SelvarajuGrad-CAM:Localization} to visualise the important areas that matter to a specific class prediction from a qualitative perspective. The darker the colour in Figure ~\ref{fig:cam_plot}, the more important that parts and the corresponding features are for the specified class.As the late-stage fusion individually retain the feature map of each input intermediate feature.  We only selected the best model from the late-stage fusion to visualise three examples. 
%The Grad-CAM allows us to roughly understand the importance of input features for a certain sleep stage in a sliding window.
% To obtain a clear graph, we only retain activation weights greater than 0.8.  

% The Figure 5(a) shows an activation map and a sliding window of each input feature, the input windows labelled as “Wake”. From the activation map, we can see that some temporal areas of activity counts, mean NNI and ratio of LF and HF have the darkest colour areas. This indicates that these three features contain the most important temporal areas for WAKE classification.

% Figure ~\ref{fig:cam_plot}(b) and (c) shows a NREMS and a REMS that  occurred in the first sleep cycle. We can see  more and more HRV features have been highlighted. Compared to Wake, figure ~\ref{fig:cam_plot}(b) shows that the entire sequence of activity counts is highlighted, which may indicate that the limb inactivity is important for NREMS classification. Compared with the previous two sleep stages, figure ~\ref{fig:cam_plot}(c) shows that except for SDNN, the HRV features have various highlighted areas at different time points. This may indicate that changes in HRV over time are of greater importance to classify REMS other than NREMS and Wake. And the activation weights of the entire activity counts series are below 0.8, which means the temporal changes for this feature is less importance to REMS classification in the early-stage sleep cycle. 


% the activation map and input signal of each feature of the window labelled "NREMS". This window is located in the first sleep cycle. We can see the activity counts, mean NNI, the ratio of LF to HF ratio, VLF and LF are all the highlighted features over temporal sequence that are important for NREMS. Compare to Wake, the entire sequence of activity counts have been highlighted, which may indicate that the limb inactivity is important to NREMS classification. And HRV features become more and more important.
% Figure ~\ref{fig:cam_plot} (C) shows the REMS activation map and the window labelled as REMS for input features. This inputs in this window is a REMS epoch in the first sleep cycle. 



%%%%%%%% discussion %%%%%%%%%%%%%%


%%%%%% old visualization section %%%%%%%%%%%%%
% \subsection{The Comparison of the Performance Difference between Apple Watch Dataset and MESA Dataset}
% the classification results of using HRS features performed better on MESA dataset than the Apple Watch dataset. First, the number of subjects in the MESA data set is approximately 56 times that of the Apple Watch data set. The size of the data set affects the performance of the data-driven model. Not only is the classification metrics of the MESA data set higher than that of the Apple Watch data set, but the standard error on the MESA data set is smaller than that of the Apple Watch data set. The second reason is due to differences in data acquisition equipment and data preprocessing methods. The HR sensing module of Apple Watch dynamically returns the calculated HR data within 2-5 seconds, whereas the MESA dataset provides IHR. When calculating statistical characteristics, differences in distribution lead to differences in features. 

% \subsection{Interpretation and sleep physiological underpinnings of features}
% Physiologically, sleep stages are different. One objective of this work is to better understand the features that may be important to the decision making process of neural network using the late-stage fusion. We think the features from different modalities may have different effects in predicting specific sleep stages. This is of high importance when considering the development of transparent technologies for health research settings in population-based research.
% The feature importance based on Grad-CAM showed some phenomena of HRV features and limb movement changes over time which have some similarities with the changes of HRV characters that have been confirmed in sleep physiological studies.

% For example, when we enter NREM sleep, the heart rate, breathing and eye movement slowing down, and muscle twitches occasionally occur during N1  sleep ~\cite{Berry2017AASM2.4}. 
% %When our heart rate, breathing and muscles relax further, we enter the third stage of NREMS~\cite{Berry2017AASM2.4}. The ANS balance of cardiac control during NREMS could be due to homeostatic control of the cardiovascular system by ascending visceral information rather than descending cortical information~\cite{Chouchou2014HeartBrain}.
% The corresponding HRV response is the decreased LF to HF ratios, HR and LF power~\cite{Montano2009HeartBehavior, Chouchou2014HeartBrain}. During the REMS, for healthy adults, the breathing is faster, the heart rate is increased and the body is in a state of temporary paralysis that prevent limb movements~\cite{Tobaldini2013HeartSleep}. The corresponding HRV response is the increased HR, LF power and LF to HF ratio~\cite{Montano2009HeartBehavior, Chouchou2014HeartBrain}. The presented results showed that the HF and the ratio of LF to HF in Figure ~\ref{fig:featue_importance} corroborates to the those mentioned in sleep physiological studies to some extent. These findings emphasise the importance of combining HRV features with movement sensing for three-stage sleep classification tasks.More interestingly, the activity count is also important to classify REMS and NREMS.




% In Apple Watch dataset, the concatenation method in the late-stage fusion numerically improved the prediction performance of all metrics for ResDeepCNN compared with the early-stage fusion and statistically improved the prediction performance of DeepCNN. But, the parameter size and inference time are increased by five times and six times, respectively.
% The performance improvement does not increase as much as the cost increases. 
% For the addition method in the late-stage fusion. It achieved the significantly improvement on the Apple Watch dataset with respect to the early-stage fusion. This indicates the benefit of keeping feature maps separately and fuse them at higher level of representation can produce better results. 

% For the hybrid fusion, the concatenation method produced the same or better results compared with the early-stage fusion. Although these sub-nets do not share the parameters in convolutional layers, the sub-net structure used to learn the representation is the same for both modalities. This may result in a high-level representation of movement sensing contains a large amount of information that may not be useful to the three-stage sleep classification. Since the movement sensing is effective for classifying sleep/wake rather than three sleep stages.

% In the hybrid fusion, we fused all cardiac intermediate features at early-stage and before fusing them with the movement sensing representation at the late stage. The latent representation of cardiac sensing learned using the sub-net may be similar to the concatenation method used in early-stage fusion.  The concatenation in hybrid fusion has increased many parameters and inference time, but the classification performance has hardly improved for both. The addition method aggregates the high-level representations of all modalities before the classifier layers. From the results, we can see that using a simple fusion method to summarise the feature representation of each modality may not always be effective in improving performance.


% We visualized the important time areas of each input channel (i.e. movement or cardiac feature channels) that matter to different sleep stages. We also calculated the feature importance score for each input using the gradient class activation map value~\cite{SelvarajuGrad-CAM:Localization}. The highlighted intermediate features demonstrated that for different sleep stages, the relative importance scores are also different. Especially, we found that the movement sensing was deemed as one of the important modalities for all sleep stages via the late-stage fusion strategy. This highlights the benefits of using the late-stage fusion strategy, which not only improves the reliability of the three-sleep stage classification model, but also capable to highlight which features are more important.

% We also visualised the important time areas of each input channel (i.e. movement or cardiac feature channels) that matter to different sleep stages. We also calculated the feature importance score for each input using the gradient class activation map value ~\cite{SelvarajuGrad-CAM:Localization}. %Some highlighted Heart Rate Variability(HRV) features from the feature importance plot were corroborated to previous sleep researches to some extent. 
% The highlighted movement sensing was deemed as one of the important modalities to achieve reliable three-sleep stage classification.


% that may be suitable for the large-scale population-based sleep and health studies

%we also reported the computational overhead
%while MESA includes 
%We evaluated these advanced fusion techniques using movement sensing and cardiac sensing data collected from two datasets using wearable devices. 
%The MESA data set contains the sleep records of 1743 people with movement sensing and cardiac sensing data derived from research-grade equipment in the ageing population. The second data set contains 31 subjects' sleep data collected from a cohort of healthy adults using consumer-grade Apple Watches with PSG sleep stage annotations. 
%A system level overview of our design pipeline can be seen in figure ~\ref{fig:system_overview}. 

%Our results show that through advanced modal fusion strategies and methods, we can improve classification performance and achieve the state-of-art results without adding additional modalities, which are usually limited by engineering challenges. 

%The results also demonstrated the three-stage sleep classification is a practical task using movement and cardiac sensing that are available on current available ubiquitous sensing products and would address a major gap in the existing literature. 

%We also thoughtfully analyse the feasibility of the discovered models with respect to the overhead imposed by each multimodal fusion combination. 

%In this work, we used a visualisation method to explore the importance of features on the deep learning model by highlighting the important time regions for each input element. This improves our understanding of the model decision process.


%We expect this study to dramatically accelerate the progression of sleep and health research in the ubiquitous computing community, and  


%given the open access of datasets, transparency of pipeline/algorithms. 

%as well as  open-access data, pre-processing pipelines along with the model development and validation.  

%We also discussed possible extensions to the presented approach which will help establish a more precise sleep stage classification model. Our code used for study can be found: https://github.com/placeholder


%We not only need to extract discriminative information from individual modalities, but we also have to discover at what stage the integration of these features can better serve the advantages of multimodal representation learning. 
%The discovered models provide promising sleep time estimate for each sleep stage that will have a substantial impact on real-world deployment.

==> figure_bing.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.4\linewidth]{Figures/Bing_LI.jpg}
	\caption{A typical polysomnography(PSG) study in sleep laboratory}
    \label{fig:bing}
\end{figure}

==> figure_inference_time.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=.6\linewidth]{Figures/classifier_module_inference_time.png}
	\caption{An overview of time consumption for each module based on each combination of fusion strategy and fusion method. We counted the running time of each sub-module on the Apple Watch data set for each model. The results are calculated based on 10 runs, and each run we inferred 500 samples.Time is in milliseconds.}
    \label{fig:inference_time_per_module_per_cls}
\end{figure}

==> table_apple_hrs_epoch.tex <==

\begin{table}[H]
  \caption{Three-stage sleep classification prediction results for each fusion strategy and method in the \textit{Apple} dataset using LOOCV method, evaluated on sleep epoch-wise during recording period. }
\centering
\resizebox{0.6\textwidth}{!}{%

\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\multicolumn{3}{c|}{\textbf{Fusion Specifics}} & \multicolumn{3}{c|}{\textbf{Performance Metrics}} & \multicolumn{3}{c}{\textbf{Time Deviation}} \\
\midrule
\textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Accuracy} & \textbf{Cohen} & \textbf{F1} & \textbf{Non-REM sleep} & \textbf{REM sleep} & \textbf{Wake} \\
\midrule
\multicolumn{1}{c|}{\multirow{2}[4]{*}{Early-Stage Fusion}} & DeepCNN & Concatenation & 72.3 $\pm$ 2.5 & 40.0 $\pm$ 5.8 & 59.0 $\pm$ 3.6 & -0.6 $\pm$ 22.3 & 11.8 $\pm$ 22.5 & -11.2 $\pm$ 6.9 \\
\cmidrule{2-9}  & ResDeepCNN & Concatenation & 76.0 $\pm$ 2.4 & 45.7 $\pm$ 6.1 & 63.4 $\pm$ 3.5 & 12.3 $\pm$ 17.2 & -4.0 $\pm$ 17.1 & -8.2 $\pm$ 7.3 \\
\midrule
\multicolumn{1}{c|}{\multirow{4}[4]{*}{Late-Stage Fusion}} & \multirow{2}[2]{*}{DeepCNN} & Concatenation & 76.2 $\pm$ 2.7 & 47.0 $\pm$ 7.1 & 63.7 $\pm$ 4.5 & 8.4 $\pm$ 16.5 & 1.3 $\pm$ 19.4 & -9.7 $\pm$ 7.1 \\
  &   & Addition & 78.2 $\pm$ 2.1 & 49.9 $\pm$ 6.9 & 65.2 $\pm$ 3.8 & 11.4 $\pm$ 10.4 & -0.6 $\pm$ 11.2 & -10.8 $\pm$ 6.6 \\
\cmidrule{2-9}  & \multirow{2}[2]{*}{ResDeepCNN} & Concatenation & 75.5 $\pm$ 2.9 & 47.0 $\pm$ 6.5 & 63.4 $\pm$ 4.2 & 10.4 $\pm$ 18.5 & -2.1 $\pm$ 19.6 & -8.3 $\pm$ 7.0 \\
  &   & Addition & \boldmath{}\textbf{78.2 $\pm$ 2.3}\unboldmath{} & \boldmath{}\textbf{52.0 $\pm$ 5.8}\unboldmath{} & \boldmath{}\textbf{66.5 $\pm$ 3.8}\unboldmath{} & 1.9 $\pm$ 11.7 & 4.7 $\pm$ 12.6 & -6.5 $\pm$ 7.3 \\
\midrule
\multicolumn{1}{c|}{\multirow{10}[4]{*}{Hybrid Fusion}} & \multirow{5}[2]{*}{DeepCNN} & Concatenation & 72.9 $\pm$ 3.0 & 40.1 $\pm$ 6.6 & 60.6 $\pm$ 3.8 & 10.7 $\pm$ 20.1 & 0.6 $\pm$ 19.5 & -11.4 $\pm$ 6.4 \\
  &   & Addition & 72.1 $\pm$ 2.9 & 38.6 $\pm$ 6.5 & 58.9 $\pm$ 3.9 & 8.8 $\pm$ 20.4 & 1.3 $\pm$ 19.9 & -10.2 $\pm$ 7.3 \\
  &   & Attention-On-Mov & 73.5 $\pm$ 2.9 & 41.3 $\pm$ 6.2 & 60.4 $\pm$ 3.9 & 1.2 $\pm$ 18.7 & 5.0 $\pm$ 18.9 & -6.2 $\pm$ 7.7 \\
  &   & Attention-On-Car & 71.1 $\pm$ 3.4 & 37.4 $\pm$ 6.7 & 58.1 $\pm$ 4.1 & 7.5 $\pm$ 24.3 & 0.7 $\pm$ 23.1 & -8.2 $\pm$ 7.5 \\
  &   & Bilinear & 70.4 $\pm$ 3.3 & 34.6 $\pm$ 7.0 & 56.9 $\pm$ 4.0 & 6.4 $\pm$ 21.6 & 4.8 $\pm$ 22.6 & -11.2 $\pm$ 5.5 \\
\cmidrule{2-9}  & \multirow{5}[2]{*}{ResDeepCNN} & Concatenation & 74.6 $\pm$ 2.6 & 44.5 $\pm$ 6.5 & 61.9 $\pm$ 3.5 & 10.2 $\pm$ 13.6 & -1.3 $\pm$ 14.1 & -8.9 $\pm$ 7.0 \\
  &   & Addition & 78.5 $\pm$ 2.4 & 51.5 $\pm$ 5.8 & 66.0 $\pm$ 3.6 & 11.8 $\pm$ 11.5 & -5.6 $\pm$ 12.2 & -6.2 $\pm$ 7.8 \\
  &   & Attention-On-Mov & 75.2 $\pm$ 2.6 & 45.0 $\pm$ 5.6 & 63.1 $\pm$ 3.4 & 10.4 $\pm$ 19.4 & -2.0 $\pm$ 19.5 & -8.4 $\pm$ 7.2 \\
  &   & Attention-On-Car & 72.2 $\pm$ 3.0 & 41.5 $\pm$ 6.8 & 59.7 $\pm$ 3.8 & -2.9 $\pm$ 25.3 & 12.0 $\pm$ 26.4 & -9.1 $\pm$ 6.7 \\
  &   & Bilinear & 70.8 $\pm$ 3.5 & 38.4 $\pm$ 7.5 & 58.1 $\pm$ 4.4 & -2.8 $\pm$ 22.9 & 6.4 $\pm$ 24.8 & -3.5 $\pm$ 8.0 \\
\bottomrule
\end{tabular}%
    
    
    }

  \label{tab:apple_hrs_epoch}%
\end{table}%


==> table_class_wise_metrics.tex <==

\begin{table}[h]
  \centering
  \caption{Comparison of three-stage sleep classification metrics between using the intermediate feature and using the raw accelerometer data with the cardiac intermediate feature. Metrics evaluated from the ResDeepCNN and ResDeepMixCNN based on window length of 101 in Apple Watch Dataset.}
  \resizebox{0.9\textwidth}{!}{%

\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\multirow{3}[6]{*}{\textbf{Fusion Strategy}} & \multirow{3}[6]{*}{\textbf{Fusion Method}} & \multicolumn{1}{c|}{\multirow{3}[6]{*}{\textbf{Performance Metrics}}} & \multicolumn{6}{c}{\textbf{Input Type}} \\
\cmidrule{4-9}  &   & \multicolumn{1}{c|}{} & \multicolumn{3}{c|}{\textbf{Intermediate Features}} & \multicolumn{3}{c}{\textbf{\shortstack{Raw Accleroemter \\ Cardiac Intermediate Features}}} \\
\cmidrule{4-9}  &   & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\textbf{WAKE}} & \multicolumn{1}{c|}{\textbf{NREM}} & \multicolumn{1}{c|}{\textbf{REM}} & \multicolumn{1}{c|}{\textbf{WAKE}} & \multicolumn{1}{c|}{\textbf{NREM}} & \multicolumn{1}{c}{\textbf{REM}} \\
\midrule
\multicolumn{1}{c|}{\multirow{2}[2]{*}{Early Stage Fusion}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Concatenation }} & Accuracy & 40.5 $\pm$ 6.2 & 72.6 $\pm$ 2.6 & 34.9 $\pm$ 7.0 & 34.9 $\pm$ 5.3 & 75.0 $\pm$ 2.4 & 32.8 $\pm$ 7.6 \\
  &   & F1 & 55.5 $\pm$ 6.4 & 83.9 $\pm$ 1.8 & 48.4 $\pm$ 8.2 & 50.0 $\pm$ 5.5 & 85.6 $\pm$ 1.6 & 45.5 $\pm$ 9.0 \\
\midrule
\multicolumn{1}{c|}{\multirow{10}[10]{*}{Hybrid Fusion}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Concatenation }} & Accuracy & 41.7 $\pm$ 6.1 & 70.5 $\pm$ 3.0 & 33.3 $\pm$ 6.4 & 37.5 $\pm$ 6.2 & 75.3 $\pm$ 2.6 & 36.0 $\pm$ 7.0 \\
  &   & F1 & 56.8 $\pm$ 6.1 & 82.4 $\pm$ 2.2 & 47.0 $\pm$ 7.9 & 52.4 $\pm$ 6.2 & 85.7 $\pm$ 1.7 & 49.7 $\pm$ 7.9 \\
\cmidrule{2-9}  & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Addition }} & Accuracy & 41.7 $\pm$ 6.1 & 70.5 $\pm$ 3.0 & 33.3 $\pm$ 6.4 & 34.9 $\pm$ 6.0 & 75.8 $\pm$ 2.5 & 30.3 $\pm$ 7.7 \\
  &   & F1 & 56.8 $\pm$ 6.1 & 82.4 $\pm$ 2.2 & 47.0 $\pm$ 7.9 & 49.5 $\pm$ 6.4 & 86.0 $\pm$ 1.7 & 42.2 $\pm$ 9.3 \\
\cmidrule{2-9}  & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Attention-On-Mov}} & Accuracy & 40.0 $\pm$ 5.8 & 71.3 $\pm$ 3.2 & 35.4 $\pm$ 7.1 & 36.8 $\pm$ 5.5 & 74.4 $\pm$ 2.8 & 31.4 $\pm$ 7.4 \\
  &   & F1 & 55.3 $\pm$ 5.8 & 82.9 $\pm$ 2.3 & 48.9 $\pm$ 8.4 & 52.1 $\pm$ 5.8 & 85.1 $\pm$ 1.9 & 44.1 $\pm$ 8.6 \\
\cmidrule{2-9}  & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Attention-On-Car}} & Accuracy & 41.0 $\pm$ 5.7 & 67.8 $\pm$ 3.8 & 30.5 $\pm$ 7.9 & 34.3 $\pm$ 5.9 & 73.1 $\pm$ 3.1 & 28.6 $\pm$ 8.2 \\
  &   & F1 & 56.3 $\pm$ 6.0 & 80.3 $\pm$ 3.1 & 42.5 $\pm$ 9.3 & 48.9 $\pm$ 6.6 & 84.2 $\pm$ 2.1 & 39.7 $\pm$ 9.8 \\
\cmidrule{2-9}  & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Bilinear}} & Accuracy & 35.9 $\pm$ 6.7 & 67.0 $\pm$ 4.0 & 29.7 $\pm$ 7.8 & 30.7 $\pm$ 6.8 & 70.7 $\pm$ 2.8 & 15.6 $\pm$ 5.3 \\
  &   & F1 & 50.2 $\pm$ 6.9 & 79.7 $\pm$ 3.0 & 41.6 $\pm$ 9.2 & 44.1 $\pm$ 7.4 & 82.6 $\pm$ 1.9 & 24.3 $\pm$ 7.6 \\
\bottomrule
\end{tabular}%

}
  \label{tab:classi-wise metrics}%
\end{table}%


==> table_compare_epoch.tex <==

\begin{table}[htbp]
  \centering
  \caption{
  Three stage sleep classification results comparing to previous work based on \textit{sample-wised} evaluation
}
  \resizebox{\textwidth}{!}{%
      \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
    \toprule
    \multicolumn{1}{|c|}{\textbf{Dataset and Feature Set}} & \textbf{Fusion Stage} & \textbf{Model} & \textbf{Accuracy} & \textbf{Cohen Kappa} & \textbf{F1} & \textbf{Precision} & \textbf{Sensitivity} & \textbf{Specificity} \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{MESA (Activity Counts, HRS)}} & Early-stage Fusion & CNN (101) ~\cite{Zhai2020MakingSensing} & 75.9 & 61.0 & 70.4 & 71.5 & 70.0 & 85.6 \\
\cmidrule{2-9}      & Hybrid Fusion & ResDeepCNN, Attention-On-Act & \textbf{79.5} & \textbf{67.2} & \textbf{75.5} & \textbf{74.9} & \textbf{76.2} & \textbf{88.5} \\
    \midrule
    Apple Watch (Activity Counts, HR, Time) & Early-stage Fusion & MLP ~\cite{Walch2019SleepDevice} & 71.6 & 24.4 & 48.4 & 63.8 & 46.0 & 71.2 \\
    \midrule
    Apple Watch (Activity Counts, HRS) & Late-stage Fusion & ResDeepCNN-2D, Addition & \textbf{78.2} & \textbf{52.1} & \textbf{67.1} & \textbf{71.6} & \textbf{64.1} & \textbf{82.0} \\
    \bottomrule
    \end{tabular}%
  
      }
  \label{tab:compare_epoch}%
\end{table}%


==> table_experiment_setting.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[t!]
\caption{Experiment settings based on input modalities, where $l$ is the window length of the input ($l=\{21, 51 ,101\})$, the inputs are for each sleep epoch}
\label{tab:experiment_seetings}
  \centering
  \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|l|l}
    \toprule
    \textbf{\makecell[l]{\textbf{Algorithm}\\\textbf{Type}}} & \textbf{Modality} & \textbf{Input Dimension} & \textbf{Features Used (Full list on Tables \ref{tab:actigraph_features} and \ref{tab:hr_features})} \\
    \midrule
    \multirow{3}[6]{*}{ML} &  \guy  \hspace{0.1em} \textit{[Actigraphy]} & $x \in \mathbb{R}^{370}$ & 370 features were derived from Activity Counts \\
\cmidrule{2-4}      &  \heart  \hspace{0.1em} \textit{[HR/HRV]} & $x \in \mathbb{R}^{30}$ & 30 features were derived from RR intervals \\
\cmidrule{2-4}      & \specialcell{\heart \hspace{0.1em} \guy \\ \textit{[HR/HRV, Actigraphy]} } & $x \in \mathbb{R}^{400}$ & Concatenation of the two modalities above \\
    \midrule
    \multirow{3}[6]{*}{DL} &  \guy  \hspace{0.1em} \textit{[Actigraphy]} & $x \in \mathbb{R}^{l}$ & Activity Counts  \\
\cmidrule{2-4}      &  \heart  \hspace{0.1em} \textit{[HR/HRV]} & $X \in \mathbb{R}^{l\times8}$  & \makecell[l]{8 features were derived from RR intervals: Mean NNi, \\Standard Derivation of RR interval (SDNN),\\ RR interval differences (SDSD), Very Low Frequency, Low Frequency,\\ High Frequency Bands, Low Frequency to High Frequency Ratio and Total Power.}  \\
\cmidrule{2-4}      & \specialcell{\heart \hspace{0.1em} \guy \\ \textit{[HR/HRV, Actigraphy]} } & $X \in \mathbb{R}^{l\times9}$  & Concatenation of the two modalities above \\
    \bottomrule
    \end{tabular}%
    }
%
\end{table}%


==> table_mesa_act_hrv_epoch.tex <==

\begin{table}[h!]
  \caption{Three-stage sleep classification prediction results for each fusion strategies and methods in the \textit{MEAS-ACT-HRV test} dataset, using Activity Counts and HRV feature sets, evaluated on sleep epoch-wise. }
\centering
\resizebox{0.6\textwidth}{!}{%
    
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \toprule
    \textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Accuracy} & \textbf{Cohen} & \textbf{F1} & \textbf{Precision} & \textbf{Sensitivity} & \textbf{Specificity} \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{Early-Stage Fusion}} & DeepCNN & Concatenation & \textbf{78.2} & \textbf{64.0} & \textbf{73.3} & \textbf{74.5} & \textbf{72.6} & \textbf{86.9} \\
\cmidrule{2-9}      & ResDeepCNN & Concatenation & \textbf{78.3} & \textbf{64.8} & \textbf{72.9} & \textbf{75.5} & \textbf{71.2} & \textbf{86.8} \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{6}[12]{*}{Late-Stage Fusion}} & \multirow{3}[6]{*}{DeepCNN-2D} & Multiplication & 53.8 & 0.0 & 23.3 & 17.9 & 33.3 & 66.7 \\
\cmidrule{3-9}      &   & Concatenation & \textbf{79.5} & \textbf{65.9} & \textbf{74.5} & \textbf{75.6} & \textbf{73.7} & \textbf{87.7} \\
\cmidrule{3-9}      &   & Addition & 79.2 & \textbf{65.9} & 74.1 & \textbf{75.6} & 72.9 & 87.5 \\
\cmidrule{2-9}      & \multirow{3}[6]{*}{ResDeepCNN-2D} & Multiplication & 78.4 & 65.2 & 73.8 & 73.6 & \textbf{74.1} & 87.6 \\
\cmidrule{3-9}      &   & Concatenation & \textbf{79.6} & \textbf{66.4} & \textbf{74.4} & \textbf{76.1} & 73.1 & \textbf{87.9} \\
\cmidrule{3-9}      &   & Addition & 78.5 & 65.2 & 73.5 & 74.3 & 73.1 & 87.3 \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{12}[24]{*}{Hybrid Fusion}} & \multirow{6}[12]{*}{DeepCNN} & Multiplication & \textbf{78.7} & \textbf{66.0} & \textbf{74.4} & \textbf{74.6} & \textbf{75.1} & \textbf{87.6} \\
\cmidrule{3-9}      &   & Concatenation & 78.2 & 64.0 & 73.3 & 74.5 & 72.6 & 86.9 \\
\cmidrule{3-9}      &   & Addition & 78.4 & 65.4 & 73.0 & 74.2 & 72.0 & 87.1 \\
\cmidrule{3-9}      &   & Attention-On-Act & 78.5 & 65.1 & 73.7 & 74.3 & 73.2 & 87.3 \\
\cmidrule{3-9}      &   & Attention-On-Car & 77.1 & 63.5 & 72.6 & 71.7 & 73.7 & 87.3 \\
\cmidrule{3-9}      &   & Bilinear & 75.4 & 61.3 & 71.1 & 70.3 & 72.8 & 86.2 \\
\cmidrule{2-9}      & \multirow{6}[12]{*}{ResDeepCNN} & Multiplication & 79.2 & 67.0 & 74.5 & 75.6 & 73.6 & 86.2 \\
\cmidrule{3-9}      &   & Addition & 79.3 & 65.9 & 74.7 & 75.0 & 74.9 & 87.9 \\
\cmidrule{3-9}      &   & Concatenation & \textbf{79.6} & 66.7 & 74.2 & \textbf{76.9} & 72.4 & 87.5 \\
\cmidrule{3-9}      &   & Attention-On-Act & 79.5 & \textbf{67.2} & \textbf{75.5} & 74.9 & \textbf{76.2} & \textbf{88.5} \\
\cmidrule{3-9}      &   & Attention-On-Car & 79.1 & 65.0 & 74.0 & 75.7 & 72.8 & 87.4 \\
\cmidrule{3-9}      &   & Bilinear & 75.2 & 60.0 & 69.9 & 70.6 & 69.2 & 85.5 \\
    \bottomrule
    \end{tabular}%
    }

  \label{tab:mesa_act_hrv_epoch}%
\end{table}%


==> table_mesa_hrs_epoch.tex <==

\begin{table}[ht]
  \caption{Three-stage sleep classification prediction results for each fusion strategies and methods in the \textit{MEAS test} dataset, using Activity Counts and HRS feature sets, evaluated on sleep epoch-wise. }
\centering
\resizebox{0.8\textwidth}{!}{%
           \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \toprule
    \textbf{Fusion Strategy} & \textbf{Network} & \textbf{Fusion Method} & \textbf{Accuracy} & \textbf{Cohen} & \textbf{F1} & \textbf{Precision} & \textbf{Sensitivity} & \textbf{Specificity} \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{2}[4]{*}{Early-Stage Fusion}} & DeepCNN & Concatenation & \textbf{77.04} & \textbf{63.78} & \textbf{72.61} & \textbf{71.83} & \textbf{73.62} & \textbf{87.17} \\
\cmidrule{2-9}      & ResDeepCNN & Concatenation & \textbf{79.43} & \textbf{65.66} & \textbf{74.06} & \textbf{76.18} & \textbf{72.58} & \textbf{87.72} \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{6}[12]{*}{Late-Stage Fusion}} & \multirow{3}[6]{*}{DeepCNN-2D} & Multiplication & 53.8 & 0.0 & 23.3 & 17.9 & 33.3 & 66.7 \\
\cmidrule{3-9}      &   & Concatenation & \textbf{79.2} & \textbf{66.7} & \textbf{74.7} & \textbf{74.8} & \textbf{74.6} & \textbf{88.1} \\
\cmidrule{3-9}      &   & Addition & 77.4 & 64.3 & 72.1 & 72.5 & 71.8 & 87.0 \\
\cmidrule{2-9}      & \multirow{3}[6]{*}{ResDeepCNN-2D} & Multiplication & 77.8 & 64.2 & 71.9 & 74.5 & 70.1 & 86.4 \\
\cmidrule{3-9}      &   & Concatenation & \textbf{79.6} & 66.1 & \textbf{73.4} & \textbf{77.9} & 70.8 & \textbf{87.1} \\
\cmidrule{3-9}      &   & Addition & 77.6 & 63.8 & 71.7 & 73.6 & 70.5 & 86.4 \\
    \midrule
    \multicolumn{1}{|c|}{\multirow{12}[24]{*}{Hybrid Fusion}} & \multirow{6}[12]{*}{DeepCNN} & Multiplication & \textbf{79.79} & \textbf{66.51} & \textbf{74.76} & 76.16 & \textbf{73.64} & \textbf{87.94} \\
\cmidrule{3-9}      &   & Concatenation & 79.53 & 66.38 & 74.29 & 76.42 & 72.73 & 87.54 \\
\cmidrule{3-9}      &   & Addition & 78.71 & 64.93 & 73.38 & \textbf{76.53} & 71.68 & 86.62 \\
\cmidrule{3-9}      &   & Attention-On-Act & 79.56 & 66.19 & 74.41 & 76.22 & 73.05 & 87.75 \\
\cmidrule{3-9}      &   & Attention-On-Car & 78.77 & 65.17 & 73.65 & 74.34 & 73.06 & 87.53 \\
\cmidrule{3-9}      &   & Bilinear & 75.35 & 60.34 & 70.28 & 71.42 & 69.98 & 85.23 \\
\cmidrule{2-9}      & \multirow{6}[12]{*}{ResDeepCNN} & Multiplication & 79.42 & \textbf{67.34} & \textbf{75.11} & 74.95 & \textbf{75.26} & \textbf{88.24} \\
\cmidrule{3-9}      &   & Addition & 78.82 & 65.16 & 73.40 & \textbf{77.62} & 71.17 & 86.43 \\
\cmidrule{3-9}      &   & Concatenation & 78.78 & 65.10 & 74.02 & 74.99 & 74.12 & 87.41 \\
\cmidrule{3-9}      &   & Attention-On-Act & \textbf{79.62} & 66.67 & 74.95 & 76.48 & 74.21 & 87.61 \\
\cmidrule{3-9}      &   & Attention-On-Car & \textbf{79.24} & 65.12 & 73.23 & 76.06 & 71.35 & 87.26 \\
\cmidrule{3-9}      &   & Bilinear & 75.48 & 59.96 & 69.99 & 72.04 & 69.40 & 85.07 \\
    \bottomrule
    \end{tabular}%
    }

  \label{tab:mesa_hrs_epoch}%
\end{table}%


==> test_table.tex <==

\begin{table}[htbp]
  \centering
  \caption{
  Three-stage sleep classification prediction results comparing to previous work evaluated on subject level during recording period; (*Average time deviation measured in \textbf{Minutes} from ground truth across all subjects $\pm$ standard error )
}
  \resizebox{\textwidth}{!}{%
      % Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\toprule
\textbf{Dataset and Feature Set} & \textbf{Fusion Stage} & \textbf{Model} & \textbf{Accuracy} & \textbf{Cohen} & \textbf{F1} & \textbf{Precision} & \textbf{Sensitivity} & \textbf{Specificity} & \textbf{Non-REM sleep} & \textbf{REM sleep} & \textbf{Wake} \\
\midrule
\multirow{2}[4]{*}{ \shortstack{MESA \\ (Activity Counts, HRV)}} & Early-stage Fusion & CNN (101) (Zhai, 2020) & \shortstack{ 76.0 \\ (75.0, 77.0) } & \shortstack{ 58.6 \\ (56.7, 60.5) } & \shortstack{ 68.1 \\ (66.8, 69.4) } & \shortstack{ 72.2 \\ (71.0, 73.4) } & \shortstack{ 69.7 \\ (68.4, 71.0) } & \shortstack{ 85.6 \\ (85.0, 86.2) } & \shortstack{ 14.9 \\ (8.2, 21.6) } & \shortstack{ -0.5 \\ (-4.8, 3.8) } & \shortstack{ -14.4 \\ (-20.2, -8.6) } \\
\cmidrule{2-12}  & Hybrid Fusion & ResDeepCNN, Attention-On-Act & \textbf{\shortstack{ 79.5 \\ (78.5, 80.5) }} & \textbf{\shortstack{ 65.1 \\ (63.3, 66.9) }} & \textbf{\shortstack{ 73.4 \\ (72.2, 74.6) }} & \textbf{\shortstack{ 75.1 \\ (73.9, 76.3) }} & \textbf{\shortstack{ 75.7 \\ (74.5, 76.9) }} & \textbf{\shortstack{ 88.4 \\ (87.9, 88.9) }} & \textbf{\shortstack{ -5.4 \\ (-12.1, 1.3) }} & \textbf{\shortstack{ 6.7 \\ (3.1, 10.3) }} & \textbf{\shortstack{ -1.3 \\ (-7.8, 5.2) }} \\
\midrule
 \shortstack{Apple Watch \\ (Activity Counts, HR, Time)} & Early-stage Fusion & MLP (Walch, 2019) & \shortstack{ 72.1 \\ (69.7, 74.5) } & \shortstack{ 23.7 \\ (19.3, 28.1) } & \shortstack{ 47.8 \\ (44.2, 51.4) } & \shortstack{ 57.4 \\ (52.9, 61.9) } & \shortstack{ 49.0 \\ (45.4, 52.6) } & \shortstack{ 71.3 \\ (70.1, 72.5) } & \shortstack{ 84.2 \\ (67.0, 101.4) } & \shortstack{ -65.4 \\ (-80.4, -50.4) } & \shortstack{ -18.8 \\ (-24.9, -12.7) } \\
\midrule
 \shortstack{Apple Watch \\ (Activity Counts, HRS)}& Late-stage Fusion & ResDeepCNN-2D, Addition & \textbf{\shortstack{ 78.4 \\ (76.3, 80.5) }} & \textbf{\shortstack{ 50.1 \\ (43.7, 56.5) }} & \textbf{\shortstack{ 64.5 \\ (60.6, 68.4) }} & \textbf{\shortstack{ 71.6 \\ (67.3, 75.9) }} & \textbf{\shortstack{ 64.2 \\ (60.4, 68.0) }} & \textbf{\shortstack{ 82.2 \\ (80.4, 84.0) }} & \textbf{\shortstack{ 21.3 \\ (6.0, 36.6) }} & \textbf{\shortstack{ -10.5 \\ (-25.9, 4.9) }} & \textbf{\shortstack{ -10.8 \\ (-17.4, -4.2) }} \\
\bottomrule
\end{tabular}%
}
  \label{tab:test}%
\end{table}%


==> unused.tex <==

% \begin{enumerate}
%     \item To the best of our knowledge, we are the first study that explore the advanced modality fusion strategies and methods and the influence of features to the performance of modality fusion for the three-stage sleep classification which is a viable task based on movement sensing and cardiac sensing data .
%     \item For ubiquitous practitioners, we compared the data that may generate from commercial or clinical grade research wearables. Or the data that may collected from the consumer devices, for the health study, we may not need this level’s grade of the rigorous. 
%     \item Our study design that facilitate the multimodal fusion for sleep stages monitoring. We found these following insights. Our study provided several guidelines for considering to adopt DL fusion methods for sensing three sleep stages for health ubiquitous computing to solve real world sleep health problem. We also provided some useful insides towards strength model prediction reliability by adopting multimodal fusion methods on health related research that using ubiquitous methods on physiological signals. For non-machine learning application researchers in Ubicomp, we could understand how does the advanced ML model might influence the sleep health research. 

% \end{enumerate}


% \begin{itemize}
%     \item \textbf{Simple operation-based method} For Simple operation-based method, we have concatenation, weighted sums and multiplication.
%     \item \textbf{Attention-based fusion} Attention mechanisms are widely used for fusion physiological signals. It often refers to the weighted sum of set of vectors with scalar weights that are dynamically generated by a small “attention” model at each time-step. Multiple glimpses are often used to generate multiple sets of dynamic weights for summation, which can preserve additional information by concatenating the results derived from each glimpse.
%     \begin{itemize}
%         \item \textbf{GlobalFusion} method is proposed by Liu and Yao et.al. which is an effective multimodal fusion method for human activity recognition. 
%         \item \textbf{Gated multimodal attention} is Blah Blah.
%     \end{itemize}
%     \item \textbf{Bilinear Pooling-based attention} Second-order statistic pooling is an example of it

% \end{itemize}


% \begin{table}[ht!]
%   \centering
%   \caption{Models and Experiments Plan}
%   \resizebox{0.99\textwidth}{!}{
%     \begin{tabular}{|p{19.39em}|p{26em}|p{9.335em}|}
%     \toprule
%     \textbf{Fusion Strategies} & \textbf{Models, Methods and Networks} & \textbf{Status} \\
%     \midrule
%     \multicolumn{3}{|p{54.725em}|}{\textbf{Early Fusion}} \\
%     \midrule
%     Joint representation & Concatenation of modalities on network & Done, it is the baseline \\
%     \midrule
%     Split representation & Separate representation learning for each modality then adopt simple operation based fusion method & Done \\
%     \midrule
%     Sharing representation & Sharing weights over modalities ?? & To Do \\
%     \midrule
%     Residual connection with intra-modality fusion & Concatenation of modalities & Done \\
%     \midrule
%     Residual connection with inter-modality fusion & Fusion on each level of representations and then adopt simple operation-based method & Done \\
%     \midrule
%     \multicolumn{3}{|p{54.725em}|}{\textbf{Attention-based Fusion }} \\
%     \midrule
%     \multirow{2}[2]{*}{GlobalFusion} & Multimodality multi-level of representation attention & \multirow{2}[2]{*}{TODO} \\
%     \multicolumn{1}{|r|}{} & Bing: One or two? & \multicolumn{1}{r|}{} \\
%     \midrule
%     \multicolumn{3}{|p{54.725em}|}{\textbf{Tensor-based Fusion}} \\
%     \midrule
%     Bilinear Pooling-based Attention & Second-order statistics pooling, & Done \\
%     \midrule
%     \multicolumn{3}{|p{54.725em}|}{\textbf{Late Fusion}} \\
%     \midrule
%     Score level fusion & Select top 5 classifiers and do mean, max posterior fusion & TODO \\
%     \midrule
%     Decision level fusion & Select top 5 networks to do weighted voting (inverse overfitting scores) & TODO \\
%     \bottomrule
%     \end{tabular}}%
%   \label{tab:addlabel}%
% \end{table}%


% \begin{table}[htbp]
%   \centering
%   \caption{Add caption}
%     \resizebox{0.99\textwidth}{!}
%     {\begin{tabular}{|p{25.72em}|r|p{23.835em}|}
%     \toprule
%     \textbf{Paper} & \multicolumn{1}{p{3.335em}|}{\textbf{Citation}} & \textbf{Potential for Sleep Takss} \\
%     \midrule
%     \textbf{Decision-level fusion in fingerprint verification} & \multirow{5}[2]{*}{521} & Multiple samples different window lengths, \\
%     Abstract: &   & Multiple representations (feature sets) from different modality \\
%     We propose to use a combination of four different fingerprint-based biometric systems where each system uses different feature extraction and/or matching algorithms to generate a matching score which can be interpreted as the confidence level of the matcher. These different matching scores are combined to obtain the lowest possible FRR for a given FAR. &   & Multiple loss functions (optimization diversity) \\
%     \multicolumn{1}{|r|}{} &   & Multiple network architectures (classifier diversity) \\
%     We also compare the performance of our integration strategy with the sum and the product rules [2]. Even though we propose and report results in scenarios (iii)–(v), our combination strategy could be used for scenarios (i) and (ii) as we &   & \multicolumn{1}{r|}{} \\
%     \midrule
%     \textbf{Feature-level and decision-level fusion of noncoincidently sampled sensors for land mine detection} & 161 & It’s a likelihood-ratio based decision fusion from various sensors. \\
%     \midrule
%     \multirow{2}[2]{*}{\textbf{Multimodal decision-level fusion for person authentication}} & \multirow{2}[2]{*}{204} & k-Means Algorithm \\
%     \multicolumn{1}{|r|}{} &   & do the k-means on the layer before FC \\
%     \midrule
%     \textbf{Threshold-optimized decision-level fusion and its application to biometrics} & 89 & Threshold based decision fusion \\
%     \midrule
%     \textbf{Decision-level fusion strategies for correlated biometric classifiers} & 49 & likelihood ratio test(LRT) and particle swarm optimization (PSO) \\
%     \midrule
%     \textbf{A comparison of decision-level sensor-fusion methods for anti-personnel landmine detection} & 111 & Dempster–Shafer theory not sure \\
%     \bottomrule
%     \end{tabular}}%
%   \label{tab:addlabel}%
% \end{table}%

% Taking into account the class imbalance in the data set, the mean F1 score used in this study is the average mean F1 score of each class  ($ \text{mean }F_1 = \frac{1}{C} \sum\limits_{c=1}^{C}\frac{2P_cR_c}{P_c+R_c}$, $P_c$ and $R_c$ denotes the class-wise precision and recall respectfully).  

% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{Figures/mesa_deepcnn_baseline_intensity_area_sum_abs_per_stage_v1.png}
% 	\caption{Ensemble model. The model starts by taking inputs from different window lengths ($l$) from the multi-modal sensors. A total of six different classifiers are used, combining a mixture of CNNs and LSTMs and exploiting their individual strengths. This results on posterior probability confusion matrix that is then combined through concatenation as part of the ensemble architecture. Finally, the decision making layer takes place by either (a) using a maximum operator approach or (b) a mean operator across all classifiers}
%     \label{fig:fig1}
% \end{figure}

% \begin{figure}
% \centering
% \subfloat[legend]{\label{a}\includegraphics[width=.45\linewidth]{nrem_pid_4294_idx_342_thres_0.8.jpeg}}\hfill
% \subfloat[legend]{\label{b}\includegraphics[width=.45\linewidth]{nrem_pid_4294_idx_342_thres_0.8.jpeg}}\hfill
% \subfloat[legend]{\label{c}\includegraphics[width=.45\linewidth]{nrem_pid_4294_idx_342_thres_0.8.jpeg}}\hfill
% \caption{my fig}
% \label{fig}
% \end{figure}


%further define the sleep label as 
%we aim to output the sleep stage label corresponding to centre point of the sliding window, as shown in Fig. ~\ref{fig:system_overview}.
%Sliding window with size $T$ and stride $S$ were used.
%(i.e.,with $T=101$ sleep epoches, equivalent to $101\times 30s/60s=50.5$ minutes)
%demonstrates the pipeline of our system.
%Based on each epoch (30 seconds), cardiac features and movement features can be extracted, serving as a sample (i.e., multivariate signal at a timestamp) in the feature streams.  %time series data. 
%Sliding window with size $T$  was employed and the stride $S$ was set to $S=1$ such that there will be a prediction at each sleep epoch.



%we focus on studying how to better utilize advanced fusion techniques
%strategies and methods to produce a reliable mode that can better classifying three sleep stages using movement sensing and cardiac sensing. 
%For each modality, we may extract one or more medical features that can be used for multimodal fusion and deep learning networks.

%Before diving into the details, we first introduce the notations used for the rest of this paper. 
%All vectors are denoted by bold lower-case letters (e.g., $\matr{x}$ and $\matr{y}$). 
%All matrices and tensors are represented by bold upper-case letters(e.g. $\matr{X}$ and $\matr{Y}$). 
%For a vector $\matr{x}$, the $j^{th}$ element is denoted by $x_j$.
%For each modality, we use the superscript to denote the modality where it came from. 
%For example, $\matr{X^{car}}$ means the feature matrix for cardiac sensing. 

%After 

% \begin{itemize}
% % 	\item \textbf{Accuracy} counts the number of correctly classified sleep epochs, normalized over the total number of sleep epochs ($\text{Acc} =\frac{TP+TN}{TP+TN+FP+FN}$).
	
% % 	\item \textbf{Recall} measures the proportion of positives that are correctly identified as the given stage ($R = \frac{TP}{TP+FN}$).
	
% % 	\item \textbf{Specificity}, also known as true negative rate, measures the proportion of negatives that are correctly identified as the given stage ($S = \frac{TN}{FP+TN}$).
	
% % 	\item \textbf{Precision} is the fraction of correct classified instances among the overall positive predictions ($P=\frac{TP}{TP+FP}$).
	
% % 	\item \textbf{$\mathbf{F_1}$ score (Macro $\mathbf{F_1}$)} is the harmonic mean between precision and recall, where the average is calculated per label and then averaged across all labels ($macro F_1 = \frac{1}{C} \sum\limits_{c=1}^{C}\frac{2P_cR_c}{P_c+R_c}$, $P_c$ and $R_c$ denotes the class-wise precision and recall respectfully).
	
% % 	\item \textbf{Cohen's Kappa ($\kappa$)} measures inter-rater reliability/agreement, comparing observed accuracy with an expected accuracy 
% % 	($\kappa = \frac{P_o - P_e}{1 - P_e}$,
% % 	where $P_o$ the observed proportional agreement and and $P_e$ the
% % 	expected proportion of agreement). In this context, Cohen's $\kappa$ factors out agreement by chance arising from the class imbalance of different sleep stages throughout the night. 
	
% 	\item \textbf{Time Deviation} We also evaluated 
% 	\item \textbf{Model Parameters and Inference Time} We count the number of model parameters to compare the size of the model which is a consideration to deploy the model in a real world mobile or edge computer equipment. We also evaluated the model inference time which is also a key consideration to the user experience and power consumption.
% \end{itemize}


% \section{Limitation and Future Work}
% The strength of this work derives from the study of the advanced fusion strategies and methods on two sleep data scenarios and the systematic design and in-depth analysis. This makes an important contribution to the literature with potential applications for clinicians, ubiquitous practitioners and the wellness industry engineers as we can achieve a reasonable performance on three-stage sleep classification without using EEG or adding extra modalities. Especially, the Apple Watch data set scenario proves that we can achieve a good result through fusion. 
% Given the fact that, the demographic factors, device, signal processing and sample size differences between these two datasets. Another limitation is that we did not explore the impact of model results trained on MESA and tested on the Apple dataset or the reverse process. It is a well know problem of data driven approach does not generalise well on different dataset or domain. We plan to address the domain adaption issues in our future work, such as how to use limited labelled data or unlabelled data to better fit to the target domain.

% In this study, we only explored the most commonly used fusion methods on convolutional neural network architecture. We did not explore tens and hundreds of fusion methods. Such as fusing over multiple convolutional layers or fusing with heterogeneous network structures such as LSTM. All our experiments are performed on a fixed windows length (101 sleep epochs) and we concentrate on multimodal fusion rather than the multiple window lengths fusion, although previous work showed that different window sizes carry different discriminative information. Future research may consider the best way to fuse information from various or dynamic window lengths.

% Given the scope of our work and objective, we did not perform the analysis to show how different models perform in diseased versus healthy population or highlight the differences between them.  We also did not consider the use of ultradian periodicity~\cite{Hobson1975SleepGroups}, the approximately 90-min sleep cycle, we tested several mixed models such as CNN + LSTM and did not observe improvement on the prediction of each sleep epoch. 

% For visualisation, we did not perform the quantitative studies the previous sleep physiological journal. Since Grad-CAM is applied to the last convolutional layer, it does not incorporate the computation performed by the last layer (the fully-connected hidden layer), and thus may not be entirely representative of the features supporting the network's decision~\cite{Jonas2019EEG-basedFeatures}.  The visualisation is only used to see whether these post-threshold filtering features highlighted by the model are similar to those mentioned in the sleep physiology study. The physiological significance behind the dynamic changes of these features in the time dimension is beyond the scope of existing medical knowledge and also not all samples are the same. 

% Finally, the use of multimodal fusion methods will inevitably increase the size of the model, which is still a concern for ubiquitous computing applications and deserves attention in future work. For example, how to reduce the size of parameters and maintain the performance of the model through knowledge distillation methods.

%This means that representation learning using early fusion tends to be less affected by noisy modalities, which may disregard the noisy signals, that hinders the learning of inter-modal relationship. 
%This means that representation learning using early fusion will not make full use of the relationship between modalities, and in most cases may not be able to learn useful information from modalities with a lot of noise.

%multimodalities because many studies use the unimodal features derived from pre-trained backbone models and use fusion methods to combine them. 


%  Firstly, the measurement methods are not standardised. Secondly, the lack of precise understanding of the physiological origins that influences the signal waveform. Thirdly, these signals' reliability and specificity are relatively low compared to the existing clinical methods

%Being able to access raw data provides medical and sleep health researchers with the opportunities to develop transparent sleep stage classification algorithms, which facilitates comparative studies. 
% The performance of using neural network models in three-stage sleep classification is much better than traditional models. But we do not know the decision-making process of these models, in this work, we will also explore the decision-making process to gain a better understand by visualising the deep neural networks.

%we focus on studying how to better utilize advanced fusion techniques
%strategies and methods to produce a reliable mode that can better classifying three sleep stages using movement sensing and cardiac sensing. 
% Clinical sleep monitoring and assessment have long been recognised as a manual multimodal classification task using various types of sensors in the PSG study.
%Fusion can be invoked at different levels in the traditional machine learning pipeline. 
%The most significant modules to complete recognition or classification tasks are sensor modules, segmentation modules, feature extraction modules and the classification or decision-making modules~\cite{Ross2001InformationBiometrics}.  Based on the operations that occur after different modules, 


%from other research fields to study the three-stage sleep classification, , namely early-stage fusion, late-stage fus1ion or hybrid fusion. 
%We select five commonly used methods in our study which can be divided into three categories, the simple operation, attention mechanism based method, and tensor-based method. 

%We only performed the inference process on the CPU and do not use the GPU resources as the GPU hardware may vary greatly in real world scenarios.

% Table ~\ref{tab:inference_time} shows the inference time, in early-fusion strategy, the total number of parameters of two backbone networks are the second lowest and the inference time is the lowest. Their F1 score and accuracy remains in the middle level.The model with the highest F1 score among all fusion strategies is ResDeepCNN-2D using the addition method in late-fusion strategy. It also has the least model parameters, but its inference time is the slowest. In Hybrid Fusion, the bilinear model has the highest parameters and the longest inference time, and the worst F1 score and accuracy. In the same category, the best performance mode is ResDeepCNN using the Attention-On-Mov method. Although its number of model parameters is 4.3 times greater than the best model (ResDeepCNN-2D using Addition method) in late-stage, the average time of forward propagation is about 2.6 times faster than that model. In addition, there is no significant difference in their F1 scores.

%In summary, if the application scenario has limitations on running time and power consumption, hybrid-fusion can improve prediction performance without increasing the running time that much. If the application scenario has restrictions on model size (a.k.a memory restriction), then late-stage fusion may provide an alternative option.


%In this work, based on two dataset scenarios,  we systematically studied three fusion strategies and four fusion methods. The data in the first scenario was collected from a group of young and healthy adults using the Apple Watch, which has gold ground truth labels annotated from PSG recordings.The second scenario is the MESA dataset, which is collected from a large diverse population of both healthy and sleep disordered participants from an aged population. The main purpose of this work is to understand how different fusion strategies and fusion methods can improve robustness of the three-stage classification model. Through this research, we have confirmed that the three-stage sleep classification is a practical task, and the model obtained using multimodal fusion techniques can achieve state-of-the-art performance. In addition, this work highlights the strengths and limitations of the different techniques. It provides a guideline to use multimodal fusion approaches to develop the state-of-the-art models that may be able to deploy on research/consumer-grade wearable devices in a transparent way.

%From Grad-CAM plot we observed that, the activity counts, mean NNI and the ratio of LF to HF for that sample are the top three most important features for classifying Wake. For NREMS classification, the activity counts, VLF, LF, and the ratio of LF to HF are showed as the important feature for the classifier. For the REMS classification, we can see all the highlighted areas are the features derived from HRV. These phenomena have some similarities with HRV characters that have been confirmed 

% Visualisation

% To better understand the decision making process of multimodal fusion, we use the gradient class activation map(Grad-Cam)~\cite{SelvarajuGrad-CAM:Localization} to visualise the important areas that matter to a specific class prediction from a qualitative perspective. The darker the colour in Figure ~\ref{fig:cam_plot}, the more important that parts and the corresponding features are for the specified class.As the late-stage fusion individually retain the feature map of each input intermediate feature.  We only selected the best model from the late-stage fusion to visualise three examples. 
%The Grad-CAM allows us to roughly understand the importance of input features for a certain sleep stage in a sliding window.
% To obtain a clear graph, we only retain activation weights greater than 0.8.  

% The Figure 5(a) shows an activation map and a sliding window of each input feature, the input windows labelled as “Wake”. From the activation map, we can see that some temporal areas of activity counts, mean NNI and ratio of LF and HF have the darkest colour areas. This indicates that these three features contain the most important temporal areas for WAKE classification.

% Figure ~\ref{fig:cam_plot}(b) and (c) shows a NREMS and a REMS that  occurred in the first sleep cycle. We can see  more and more HRV features have been highlighted. Compared to Wake, figure ~\ref{fig:cam_plot}(b) shows that the entire sequence of activity counts is highlighted, which may indicate that the limb inactivity is important for NREMS classification. Compared with the previous two sleep stages, figure ~\ref{fig:cam_plot}(c) shows that except for SDNN, the HRV features have various highlighted areas at different time points. This may indicate that changes in HRV over time are of greater importance to classify REMS other than NREMS and Wake. And the activation weights of the entire activity counts series are below 0.8, which means the temporal changes for this feature is less importance to REMS classification in the early-stage sleep cycle. 


% the activation map and input signal of each feature of the window labelled "NREMS". This window is located in the first sleep cycle. We can see the activity counts, mean NNI, the ratio of LF to HF ratio, VLF and LF are all the highlighted features over temporal sequence that are important for NREMS. Compare to Wake, the entire sequence of activity counts have been highlighted, which may indicate that the limb inactivity is important to NREMS classification. And HRV features become more and more important.
% Figure ~\ref{fig:cam_plot} (C) shows the REMS activation map and the window labelled as REMS for input features. This inputs in this window is a REMS epoch in the first sleep cycle. 



%%%%%%%% discussion %%%%%%%%%%%%%%


%%%%%% old visualization section %%%%%%%%%%%%%
% \subsection{The Comparison of the Performance Difference between Apple Watch Dataset and MESA Dataset}
% the classification results of using HRS features performed better on MESA dataset than the Apple Watch dataset. First, the number of subjects in the MESA data set is approximately 56 times that of the Apple Watch data set. The size of the data set affects the performance of the data-driven model. Not only is the classification metrics of the MESA data set higher than that of the Apple Watch data set, but the standard error on the MESA data set is smaller than that of the Apple Watch data set. The second reason is due to differences in data acquisition equipment and data preprocessing methods. The HR sensing module of Apple Watch dynamically returns the calculated HR data within 2-5 seconds, whereas the MESA dataset provides IHR. When calculating statistical characteristics, differences in distribution lead to differences in features. 

% \subsection{Interpretation and sleep physiological underpinnings of features}
% Physiologically, sleep stages are different. One objective of this work is to better understand the features that may be important to the decision making process of neural network using the late-stage fusion. We think the features from different modalities may have different effects in predicting specific sleep stages. This is of high importance when considering the development of transparent technologies for health research settings in population-based research.
% The feature importance based on Grad-CAM showed some phenomena of HRV features and limb movement changes over time which have some similarities with the changes of HRV characters that have been confirmed in sleep physiological studies.

% For example, when we enter NREM sleep, the heart rate, breathing and eye movement slowing down, and muscle twitches occasionally occur during N1  sleep ~\cite{Berry2017AASM2.4}. 
% %When our heart rate, breathing and muscles relax further, we enter the third stage of NREMS~\cite{Berry2017AASM2.4}. The ANS balance of cardiac control during NREMS could be due to homeostatic control of the cardiovascular system by ascending visceral information rather than descending cortical information~\cite{Chouchou2014HeartBrain}.
% The corresponding HRV response is the decreased LF to HF ratios, HR and LF power~\cite{Montano2009HeartBehavior, Chouchou2014HeartBrain}. During the REMS, for healthy adults, the breathing is faster, the heart rate is increased and the body is in a state of temporary paralysis that prevent limb movements~\cite{Tobaldini2013HeartSleep}. The corresponding HRV response is the increased HR, LF power and LF to HF ratio~\cite{Montano2009HeartBehavior, Chouchou2014HeartBrain}. The presented results showed that the HF and the ratio of LF to HF in Figure ~\ref{fig:featue_importance} corroborates to the those mentioned in sleep physiological studies to some extent. These findings emphasise the importance of combining HRV features with movement sensing for three-stage sleep classification tasks.More interestingly, the activity count is also important to classify REMS and NREMS.




% In Apple Watch dataset, the concatenation method in the late-stage fusion numerically improved the prediction performance of all metrics for ResDeepCNN compared with the early-stage fusion and statistically improved the prediction performance of DeepCNN. But, the parameter size and inference time are increased by five times and six times, respectively.
% The performance improvement does not increase as much as the cost increases. 
% For the addition method in the late-stage fusion. It achieved the significantly improvement on the Apple Watch dataset with respect to the early-stage fusion. This indicates the benefit of keeping feature maps separately and fuse them at higher level of representation can produce better results. 

% For the hybrid fusion, the concatenation method produced the same or better results compared with the early-stage fusion. Although these sub-nets do not share the parameters in convolutional layers, the sub-net structure used to learn the representation is the same for both modalities. This may result in a high-level representation of movement sensing contains a large amount of information that may not be useful to the three-stage sleep classification. Since the movement sensing is effective for classifying sleep/wake rather than three sleep stages.

% In the hybrid fusion, we fused all cardiac intermediate features at early-stage and before fusing them with the movement sensing representation at the late stage. The latent representation of cardiac sensing learned using the sub-net may be similar to the concatenation method used in early-stage fusion.  The concatenation in hybrid fusion has increased many parameters and inference time, but the classification performance has hardly improved for both. The addition method aggregates the high-level representations of all modalities before the classifier layers. From the results, we can see that using a simple fusion method to summarise the feature representation of each modality may not always be effective in improving performance.


% We visualized the important time areas of each input channel (i.e. movement or cardiac feature channels) that matter to different sleep stages. We also calculated the feature importance score for each input using the gradient class activation map value~\cite{SelvarajuGrad-CAM:Localization}. The highlighted intermediate features demonstrated that for different sleep stages, the relative importance scores are also different. Especially, we found that the movement sensing was deemed as one of the important modalities for all sleep stages via the late-stage fusion strategy. This highlights the benefits of using the late-stage fusion strategy, which not only improves the reliability of the three-sleep stage classification model, but also capable to highlight which features are more important.

% We also visualised the important time areas of each input channel (i.e. movement or cardiac feature channels) that matter to different sleep stages. We also calculated the feature importance score for each input using the gradient class activation map value ~\cite{SelvarajuGrad-CAM:Localization}. %Some highlighted Heart Rate Variability(HRV) features from the feature importance plot were corroborated to previous sleep researches to some extent. 
% The highlighted movement sensing was deemed as one of the important modalities to achieve reliable three-sleep stage classification.


% that may be suitable for the large-scale population-based sleep and health studies

%we also reported the computational overhead
%while MESA includes 
%We evaluated these advanced fusion techniques using movement sensing and cardiac sensing data collected from two datasets using wearable devices. 
%The MESA data set contains the sleep records of 1743 people with movement sensing and cardiac sensing data derived from research-grade equipment in the ageing population. The second data set contains 31 subjects' sleep data collected from a cohort of healthy adults using consumer-grade Apple Watches with PSG sleep stage annotations. 
%A system level overview of our design pipeline can be seen in figure ~\ref{fig:system_overview}. 

%Our results show that through advanced modal fusion strategies and methods, we can improve classification performance and achieve the state-of-art results without adding additional modalities, which are usually limited by engineering challenges. 

%The results also demonstrated the three-stage sleep classification is a practical task using movement and cardiac sensing that are available on current available ubiquitous sensing products and would address a major gap in the existing literature. 

%We also thoughtfully analyse the feasibility of the discovered models with respect to the overhead imposed by each multimodal fusion combination. 

%In this work, we used a visualisation method to explore the importance of features on the deep learning model by highlighting the important time regions for each input element. This improves our understanding of the model decision process.


%We expect this study to dramatically accelerate the progression of sleep and health research in the ubiquitous computing community, and  


%given the open access of datasets, transparency of pipeline/algorithms. 

%as well as  open-access data, pre-processing pipelines along with the model development and validation.  

%We also discussed possible extensions to the presented approach which will help establish a more precise sleep stage classification model. Our code used for study can be found: https://github.com/placeholder


%We not only need to extract discriminative information from individual modalities, but we also have to discover at what stage the integration of these features can better serve the advantages of multimodal representation learning. 
%The discovered models provide promising sleep time estimate for each sleep stage that will have a substantial impact on real-world deployment.
